Cross-Domain Acceleration of Open Modification Search: From Commodity Platforms to Emerging Memory and Storage Devices

Open modification search (OMS) in mass spectrometry (MS) is a data-intensive workload whose performance is dominantly limited by reference data movement rather than computation. Prior OMS accelerators have largely been evaluated in isolation, making it difficult to understand system-level trade-offs across platforms. This paper presents the first workload-driven, cross-platform survey of accelerators for MS search by studying not only commodity platforms, but also emerging memory- and storage-centric architectures, including GPUs, near-storage FPGAs, DRAM near-memory processing, ReRAM/PCM in-memory processing, and 3D NAND/FeNAND in-storage processing, under consistent algorithmic and accuracy assumptions. Leveraging a binary hyperdimensional computing (HDC)-based OMS formulation that reduces similarity evaluation to lightweight bitwise primitives and tolerates device-level non-idealities, we enable a robust execution on memory-centric architectures despite device-level non-idealities and limited computing capability. Overall, this study identifies memory- and storage-centric architectures as a key architectural breakthrough for large-scale, high-speed search acceleration, delivering up to >100x speedup and >40,000x improvement in energy efficiency.

==> BACKUP/6.Evaluation.tex <==


\definecolor{resultpurple}{HTML}{7B1FA2}
\newcommand{\result}[1]{\textcolor{resultpurple}{\bfseries #1}}

\section{Results}


% \subsection{Experimental Setup}

% We evaluate OMS accelerators under a common methodology that (i) holds the OMS workload and scoring objective fixed across substrates and (ii) uses a unified reporting convention that cleanly separates steady-state kernel execution from the one-time cost of making the staged working set resident. Table~\ref{tab:hw_summary} summarizes the evaluated platforms, per-package capacities, and the search primitives used in each mapping.


% \textbf{Reporting convention.}
% We report throughput and energy as \emph{search-only} and \emph{search + $1\times$ load}. \emph{Search-only} assumes the staged working set for a batch is already resident in the executing substrate (e.g., HBM/GDDR, device-side DRAM, or a pre-programmed non-volatile array). \emph{Search + $1\times$ load} adds the one-time cost to make that working set resident: DMA staging into GPU memory, NAND$\rightarrow$DRAM refills on near-storage FPGA systems, or host$\rightarrow$DRAM provisioning for volatile memory-centric designs. This separation isolates kernel efficiency from the staging overhead that dominates in the transient regime defined in Section~\ref{sec:oms-scaling}.


% \textbf{GPUs.}
% We measure throughput and energy on an NVIDIA RTX~4090 (GDDR6X, 24\,GB, $\sim$1\,TB/s) using three kernels: \textit{ANN-SoLo} (FP32 cosine), \textit{HOMS-TC} (INT8 tensor-core HDC), and \textit{HyperOMS} (binary HDC). Representative results are then scaled to an NVIDIA H100 (HBM3, 80\,GB, $\sim$3.35\,TB/s) using bandwidth and effective compute normalization. When the staged footprint $S$ exceeds the resident capacity $C_{\mathrm{res}}$, the GPU operates in the transient regime by streaming shards over the external interface; otherwise, the working set remains resident and is reused across batches.


% \textbf{Near-storage FPGAs.}
% For the FPGA path, we anchor search latency and power using a Samsung/Xilinx SmartSSD CSD (Kintex UltraScale+) and scale to a Xilinx Versal VP1902-class design co-located with NVMe storage and attached to board DRAM. RapidOMS~\cite{pinge2024rapidoms} implements XOR+popcount engines with parametric lane parallelism and supports metadata-driven pruning to reduce unnecessary comparisons. We report both search-only and search + $1\times$ load, where the load term captures NAND$\rightarrow$DRAM refills when the hot working set exceeds the device-side buffer.


% \textbf{DRAM-NMP.}
% For DRAM near-memory processing, we assume commodity DDR4 modules and model near-bank primitives and scan timing following Kang~et~al.~\cite{kang2024dram}. Write energy follows Kim~et~al.~\cite{kim2013memory}. We scale capacity and controller timing to 64\,GB modules for parity with our mid-scale regime and treat the provisioned set of modules as the executing substrate, with their aggregate capacity defining $C_{\mathrm{res}}$ in our workload model.


% \textbf{ReRAM/PCM IMP.}
% For ReRAM and PCM IMP designs, we adopt an in-array storage scenario in which reference hypervectors are programmed into crossbar arrays and reused across searches. We model 0.2\,TB per chip as a conservative capacity-normalized target comparable to high-density flash packages. ReRAM OMS follows~\cite{fan2024mlcrram}; write energy is taken from Chen~et~al.~\cite{chen2016design}, and latency/energy parameters are grounded in 40\,nm prototypes. For PCM, we use \textit{SpecPCM}~\cite{fan2024specpcm} for bandwidth and write energy and scale peripheral circuitry (drivers, sense/readout, and control) to the same 0.2\,TB target. Unless otherwise noted, we model both ReRAM and PCM with TLC (3\,bits/cell) and default \emph{no write-verify}; because the reference library is written once and then read repeatedly, we treat verify overhead as a sensitivity rather than a mainline term.


% \textbf{3D NAND / 3D FeNAND ISP.}
% For 3D NAND and FeNAND ISP designs, we adopt device parameters, latency/energy models, and the ISP flow from Hsu~et~al.~\cite{hsu2025fenand}. Across all memory- and storage-centric designs (DRAM-NMP, ReRAM, PCM, 3D NAND, FeNAND), references are resident within the substrate (arrays or provisioned memory modules), queries are broadcast, and only compact indices and scores are returned. Unless otherwise noted, we assume a conservative 64-bit, 200\,MHz host/control interface sufficient for query broadcast and top-$k$ egress, and we include peripheral overheads (sense paths, mixed-signal where applicable, and controller logic) in both latency and energy. Technology nodes are normalized to representative processes (GPU 5\,nm, FPGA 7\,nm, DRAM 22--28\,nm, ReRAM/PCM 40\,nm, and NAND/FeNAND with 14\,nm arrays and 7\,nm CMOS periphery).
 



  
 


% \subsection{Accuracy Preservation}
% \label{sec:acc_preservation}
% % HDC-based methods achieve consistent identifications under device-level bit errors.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1\columnwidth]{fig/final_identifications_comparison_ber_withdrops.pdf}
%   \caption{Impact of injected bit error rate (BER) on HyperOMS identifications for datasets b1906--b1931.}
%   \label{fig:hyperoms-ber}
% \end{figure}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\textwidth]{fig/upset.pdf}%
%   \caption{Identification consistency across BER levels (UpSet overlaps, b1906).}
%   \label{fig:UPSET}
% \end{figure*}



% Before comparing performance, we first establish that HyperOMS preserves identification accuracy under the device-level errors expected in memory-centric deployments. Concretely, we inject random bit flips into the binary hypervectors at a controlled bit error rate (BER), modeling readout uncertainty under tight sensing margins in multi-level non-volatile memories. The BER levels we sweep are aligned with regimes reported for higher bits-per-cell operation in ReRAM/PCM arrays, and therefore represent a realistic operating stress rather than an adversarial corruption model~\cite{fan2024mlcrram,fan2024specpcm}.


% We evaluate robustness along two complementary axes. First, we measure \emph{coverage} via total identifications at a fixed FDR (Fig.~\ref{fig:hyperoms-ber}). Across datasets b1906--b1931, HyperOMS-BIN tracks the INT8 baseline closely for BER $\le 10\%$. At 15\% BER, the reduction in total identifications remains modest and dataset dependent (approximately 9--14\%), indicating that discovery coverage degrades smoothly as the error rate increases.

% Total identifications alone cannot determine whether the same peptides are being recovered. We therefore evaluate identification \emph{consistency} using UpSet overlaps (Fig.~\ref{fig:UPSET}), which quantify agreement in high-confidence identifications across BER settings. In effect, totals summarize coverage, while overlaps test whether the reported set is stable under device noise. The measured resilience is consistent with hyperdimensional computing: binary encodings with Hamming-style similarity distribute information across many dimensions, so random bit flips tend to average out rather than induce catastrophic rank changes.


% To operationalize this notion of consistency, we summarize UpSet overlaps for dataset b1906 across BER $\in \{0,5,10,15\%\}$. Because ground truth is not available for HEK293, we treat the \emph{consensus} between ANN-SoLo and HOMS-TC (INT8) as a proxy reference set: this intersection captures identifications that are supported by both a conventional scoring baseline and an 8-bit HDC baseline, and is therefore a conservative approximation of ``high-confidence'' peptides for comparing robustness. We then quantify \emph{recovery} as the fraction of this proxy consensus that is also identified by HyperOMS-BIN:

% {\footnotesize
% \begin{equation}
% \mathrm{Recovery} \;=\; 
% \frac{|\mathrm{ANN}\_\mathrm{SoLo} \cap \mathrm{HOMS\text{-}TC} \cap \mathrm{HyperOMS}\_\mathrm{BIN}|}
% {|\mathrm{ANN}\_\mathrm{SoLo} \cap \mathrm{HOMS\text{-}TC}|}
% \end{equation}
% }

% Using the verified counts, recovery is $96.78\%$ at $0\%$ BER, $95.73\%$ at $5\%$ BER, $94.47\%$ at $10\%$ BER, and $91.41\%$ at $15\%$ BER. Thus, agreement with the proxy consensus remains high through $10\%$ BER and shrinks moderately at $15\%$ BER, with most differences concentrated near the reporting threshold rather than reflecting wholesale rank shifts. Taken together, total identifications and UpSet overlaps indicate that HyperOMS maintains substantial discovery coverage and preserves a large fraction of high-confidence peptides under realistic device-level BER, supporting its suitability for memory-centric deployments.



% \sumukh{fixed until here}




% % ================== TABLE: HEK DATASET (MANAGEABLE) ==================
% \begin{table*}[t]
%   \centering
%   \caption{HEK293 (Human Embryonic Kidney 293) dataset: Algorithmic comparisions with normalized energy efficiency and speedup across platforms (normalized to RTX~4090 FP32 ANN-SoLo = 1.0). We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
%   \label{tab:hek-managed}
%   \adjustbox{max width=\textwidth}{
%   \begin{tabularx}{\textwidth}{l *{6}{Y}}
%     \toprule
%     Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
%     Memory & {GDDR6X} & {GDDR6X} & {GDDR6X} & {HBM3} & {HBM3} & {HBM3} \\
%     Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
%     Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
%     \midrule
%     Energy efficiency (search-only) &
%     \result{1.000} & \result{9.696} & \result{18.814} &
%     \result{1.931} & \result{18.715} & \result{37.258} \\
%     Energy efficiency (search + 1$\times$ write/load) &
%     \result{1.000} & \result{9.671} & \result{18.804} &
%     \result{1.931} & \result{18.613} & \result{37.211} \\
%     \midrule
%     Speedup (search-only) &
%     \result{1.000} & \result{23.712} & \result{33.781} &
%     \result{2.996} & \result{71.033} & \result{101.198} \\
%     Speedup (search + 1$\times$ write/load) &
%     \result{1.000} & \result{20.517} & \result{32.944} &
%     \result{2.979} & \result{48.402} & \result{93.621} \\
%     \bottomrule
%   \end{tabularx}}
% \end{table*}

% % ================== TABLE: HEK DATASET (PART B: HyperOMS-only) ==================
% \begin{table*}[t]
%   \centering
%   \caption{HEK293 (Human Embryonic Kidney 293) dataset (Part B): HyperOMS (BIN) across platforms for an equitable comparison. We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
%   \label{tab:hek-hyperoms-only}
%   \adjustbox{max width=\textwidth}{
%   \begin{tabularx}{\textwidth}{l *{8}{Y}}
%     \toprule
%     Platform / Device & {RTX 4090} & {H100} & {VP1902} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
%     Memory / Tech. & {GDDR6X} & {HBM3} & {FPGA} & {NMP} & {40\,nm} & {\textcolor{red}{TBD}} & {ISP} & {ISP} \\
%     Method / Type & {GPU HDC} & {GPU HDC} & {NSP} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
%     Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
%     \midrule
%     Energy efficiency (search-only) &
%     \result{1.000} & \result{1.980} & \result{2.841} & \result{65.543} &
%     \result{6,737.430} & \result{16,187.919} & \result{4,912.424} & \result{40,743.243} \\
%     Energy efficiency (search + 1$\times$ write/load) &
%     \result{1.000} & \result{1.979} & \result{2.840} & \result{63.926} &
%     \result{6,741.883} & \result{16,198.617} & \result{4,915.670} & \result{40,770.169} \\
%     \midrule
%     Speedup (search-only) &
%     \result{1.000} & \result{2.996} & \result{3.096} & \result{1.872} &
%     \result{2.505} & \result{23.101} & \result{17.016} & \result{17.016} \\
%     Speedup (search + 1$\times$ write/load) &
%     \result{1.000} & \result{2.842} & \result{2.769} & \result{1.765} &
%     \result{2.576} & \result{23.755} & \result{17.498} & \result{17.498} \\
%     \bottomrule
%   \end{tabularx}}
% \end{table*}



% % ================== TABLE: HEK DATASET (LARGE, SCALED) ==================
% \begin{table*}[t]
%   \centering
%   \caption{HEK dataset scaled (15{,}000 queries; 1{,}000{,}000{,}000 references; HDC BIN size = 1\,TB): normalized energy efficiency and speedup across platforms. We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
%   \label{tab:hek-large}
%   \adjustbox{max width=\textwidth}{
%   \begin{tabularx}{\textwidth}{l *{4}{Y}}
%     \toprule
%     Platform / Device & {H100} & {H100} & {3D NAND} & {FeNAND} \\
%     Method & {GPU HDC} & {GPU HDC} & {ISP} & {ISP} \\
%     Data Type & {INT8 (HOMS-TC)} & {BIN (HyperOMS)} & {BIN} & {BIN} \\
%     \midrule
%     Energy efficiency (search-only) &
%     \result{1.000} & \result{1.991} & \result{4,938.364} & \result{40,958.387} \\
%     Energy efficiency (search + 1$\times$ write/load) &
%     \result{1.000} & \result{2.017} & \result{5,024.3} & \result{41,671.1} \\
%     \midrule
%     Speedup (search-only) &
%     \result{1.000} & \result{1.425} & \result{8.092} & \result{8.092} \\
%     Speedup (search + 1$\times$ write/load) &
%     \result{1.000} & \result{2.866} & \result{20.844} & \result{20.844} \\
%     \bottomrule
%   \end{tabularx}}
% \end{table*}




% \subsection{Comparative Results}
% \label{sec:comparative_results}

% \subsubsection{Baseline Algorithmic Efficiency on GPUs (Table~\ref{tab:hek-managed})}
% Having established that HyperOMS preserves identifications under realistic device-level BER (Section~\ref{sec:acc_preservation}), we next isolate the \emph{algorithmic} benefit of reduced-precision scoring on commodity GPUs. \cesong{
% Table~\ref{tab:hek-managed} compares FP32 ANN-SoLo, INT8 HOMS-TC, and binary HyperOMS on RTX~4090 and H100, with all results normalized to RTX~4090 FP32 ANN-SoLo.}

% % Table~\ref{tab:hek-managed} compares three software mappings on RTX~4090 and H100: a conventional FP32 baseline (ANN-SoLo), an INT8 tensor-core HDC baseline (HOMS-TC), and a binary HDC mapping (HyperOMS). All values are normalized to RTX~4090 FP32 ANN-SoLo.

% \cesong{On RTX~4090, reducing precision from FP32 to INT8/BIN HDC yields substantial benefits even before considering data locality. HOMS-TC achieves a $23.712\times$ speedup and $9.696\times$ energy-efficiency improvement in the search-only case, while HyperOMS further increases these to $33.781\times$ and $18.814\times$, respectively. Scaling to H100 amplifies the same trend: relative to the RTX~4090 FP32 baseline, ANN-SoLo improves to $2.996\times$ speedup and $1.931\times$ energy efficiency, whereas HOMS-TC and HyperOMS reach $71.033\times$ / $18.715\times$ and $101.198\times$ / $37.258\times$, respectively.}

% % On RTX~4090, moving from FP32 to HDC yields large gains even before considering cross-substrate locality. HOMS-TC achieves a $23.712\times$ speedup and $9.696\times$ higher energy efficiency in the search-only case, while HyperOMS further increases these to $33.781\times$ speedup and $18.814\times$ energy efficiency. Scaling to H100 amplifies the same trend: relative to the RTX~4090 FP32 baseline, ANN-SoLo on H100 improves to $2.996\times$ speedup and $1.931\times$ energy efficiency, whereas HOMS-TC reaches $71.033\times$ speedup and $18.715\times$ energy efficiency, and HyperOMS reaches $101.198\times$ speedup and $37.258\times$ energy efficiency. These results quantify the headroom unlocked by kernel simplification (INT8/BIN) on high-bandwidth GPUs, independent of any memory-centric data placement.


% \cesong{Including the one-time write/load cost leaves energy-efficiency trends
% largely unchanged, but reduces apparent speedup when the kernel is very
% fast, as fixed staging overheads become more visible (e.g., H100
% HyperOMS: $101.198\times \rightarrow 93.621\times$). Overall, this tier
% quantifies the headroom unlocked by kernel simplification alone, which
% serves as the baseline context for the cross-substrate comparisons that
% follow.}

% % The search+$1\times$ write/load rows capture the one-time cost of making the working set resident for a run. For this HEK configuration, energy-efficiency trends remain essentially unchanged (e.g., RTX~4090 HyperOMS: $18.814\times \rightarrow 18.804\times$; H100 HyperOMS: $37.258\times \rightarrow 37.211\times$). The speedup impact is more visible when the search kernel is very fast, since a fixed staging cost becomes a larger fraction of end-to-end time (e.g., H100 HOMS-TC: $71.033\times \rightarrow 48.402\times$; H100 HyperOMS: $101.198\times \rightarrow 93.621\times$). Overall, Table~\ref{tab:hek-managed} establishes the GPU-side algorithmic gains from reduced precision, which we use as the baseline context for the cross-substrate comparisons that follow.

% \subsubsection{Mid-Scale Cross-Substrate Comparison with a Unified HyperOMS Kernel (Table~\ref{tab:hek-hyperoms-only})}


% % Table~\ref{tab:hek-hyperoms-only} moves beyond algorithmic effects and evaluates \emph{substrate-dependent} efficiency under a unified kernel. Specifically, we fix the method to HyperOMS with binary HDC (BIN) across all platforms and normalize results to RTX~4090 running HyperOMS (search-only $=1.0$). This removes confounding from precision and scoring function, so the remaining differences primarily reflect where the reference library resides, how it is accessed (streamed vs.\ in-place), and the efficiency of the underlying memory-centric primitives and periphery.

% \cesong{This tier isolates \emph{substrate-dependent} effects by fixing the algorithm to HyperOMS with binary HDC across all platforms. Results in Table~\ref{tab:hek-hyperoms-only} are normalized to RTX~4090 running HyperOMS in the search-only configuration, so remaining differences reflect data locality, access patterns (streamed vs.\ in-place), and memory-centric execution efficiency.}

% % Two trends emerge. First, commodity and near-storage accelerators provide only modest additional gains once the kernel is already reduced to XOR+popcount-style operations. Relative to RTX~4090 HyperOMS, H100 improves throughput by $\sim$3.0$\times$ (2.996$\times$ search-only) and energy efficiency by $\sim$2.0$\times$ (1.980$\times$), while a VP1902-class near-storage FPGA reaches $\sim$3.1$\times$ speedup (3.096$\times$) and $\sim$2.8$\times$ energy efficiency (2.841$\times$). These results indicate that, in the mid-scale regime, moving from a GPU implementation to a carefully pipelined FPGA stream primarily changes microarchitectural utilization and buffering, but does not fundamentally alter the data-movement path.

% \cesong{Among commodity and near-storage accelerators, additional gains are modest once the kernel is reduced to XOR+popcount. Relative to the RTX~4090 baseline, H100 improves throughput by $2.996\times$ and energy efficiency by $1.980\times$, while a VP1902-class near-storage FPGA reaches $3.096\times$ speedup and $2.841\times$ energy efficiency. These results indicate that, in the mid-scale regime, moving from a GPU implementation to a carefully pipelined FPGA stream primarily changes microarchitectural utilization and buffering, but does not fundamentally alter the data-movement path.}

% % Second, memory- and storage-centric designs deliver \emph{orders-of-magnitude} energy gains by keeping the reference library resident within the executing substrate. DRAM-NMP improves energy efficiency to $65.543\times$ (search-only) while providing a comparable end-to-end speedup to the GPU baseline (1.872$\times$). Non-volatile IMP/ISP designs amplify this effect: ReRAM achieves $6.7\times 10^3\times$ energy efficiency with a $2.505\times$ speedup, PCM reaches $1.62\times 10^4\times$ energy efficiency with a $23.101\times$ speedup, and flash-based ISP delivers $4.9\times 10^3\times$ (3D NAND) to $4.07\times 10^4\times$ (FeNAND) energy efficiency while sustaining $\sim$17$\times$ speedup. The key distinction is that these substrates execute similarity in-place and export only compact results, shifting the dominant cost from host-device staging to internal array parallelism and periphery energy.

% \cesong{In contrast, memory- and storage-centric designs achieve orders-of-magnitude energy gains by keeping the reference library resident within the executing substrate. DRAM-NMP improves energy efficiency to $65.543\times$ with comparable throughput, while non-volatile IMP and ISP designs amplify this effect further: ReRAM reaches $6.7\times10^3\times$, PCM reaches $1.62\times 10^4\times$, and flash-based ISP delivers $4.9\times 10^3\times$ (3D NAND) to $4.07\times 10^4\times$ (FeNAND) energy efficiency while sustaining $\sim$17$\times$ speedup. These results show that, once the kernel is fixed, data locality dominates mid-scale OMS efficiency. \textcolor{red}{Need explanations for 3D NAND vs FeNAND for the same speed based on the paper P.-K.Hsu et al.,.}}

% Finally, the search-only versus search+$1\times$ write/load rows remain close for most platforms in this table, because the benchmarked working set is treated as resident within each device’s evaluation model. Where a load term exists (e.g., for volatile buffering or provisioning), its impact is small relative to the steady-state gap in energy efficiency between streamed execution and persistent in-place execution. Overall, Table~\ref{tab:hek-hyperoms-only} shows that once the kernel is fixed, the main discriminator at mid-scale is \emph{data locality}: architectures that avoid repeatedly moving reference data across an external interface achieve one to four orders of magnitude higher energy efficiency while maintaining competitive throughput.



\subsubsection{Datacenter-Scale Scalability at the Terabyte Limit (Table~\ref{tab:hek-large})}
% Table~\ref{tab:hek-large} stress-tests OMS at datacenter scale by increasing the binary reference library to $N=10^9$ ($\approx$1\,TB for $D{=}8192$ BIN), which is intentionally beyond the resident capacity of a single GPU. We normalize all results to H100 running the INT8 HDC baseline (HOMS-TC), and report both \emph{search-only} and \emph{search + $1\times$ write/load} to expose the impact of transient staging at this scale.

\cesong{This tier evaluates system-level scalability when the reference library exceeds the capacity of a single accelerator. Table~\ref{tab:hek-large} increases the binary library size to $N=10^9$ ($\approx$1\,TB for $D{=}8192$ BIN), which is intentionally beyond the resident capacity of a single GPU, and normalizes results to H100 running INT8 HOMS-TC, reporting both search-only and search+$1\times$ write/load metrics.}

Two regimes become explicit. Under \emph{search-only}, the BIN kernel on H100 (HyperOMS) provides only a moderate benefit over INT8, improving energy efficiency by $1.991\times$ and speed by $1.425\times$. This reflects a pure kernel effect under the (idealized) assumption that the working set is already resident. However, once we account for the practical requirement to stage the library (\emph{search + $1\times$ write/load}), the GPU path enters the transient regime and the apparent advantage of the BIN kernel increases to $2.017\times$ energy efficiency and $2.866\times$ speedup, because a smaller representation reduces the amount of data that must traverse the external interface.

In contrast, SSD-scale ISP avoids the staging wall entirely by executing similarity in-place. Both 3D NAND and FeNAND sustain $20.844\times$ speedup in the \emph{search + $1\times$ write/load} metric and $8.092\times$ speedup in \emph{search-only} \textcolor{red}{This part also needs to be checked and need rationale}, indicating that performance is governed by internal die/plane/page-level parallelism rather than by host-device transfer. The energy advantage is even more pronounced: relative to H100 INT8, 3D NAND achieves $5.02\times 10^3\times$ energy efficiency (search + $1\times$ write/load), while FeNAND reaches $4.17\times 10^4\times$. These gains arise because only compact results traverse the host interface; the dominant energy is spent inside the storage package, amortized across massive internal parallelism.

Overall, Table~\ref{tab:hek-large} highlights the scaling inflection described in Section~\ref{sec:oms-scaling}: at terabyte-scale libraries, GPU execution becomes constrained by transient staging over external links, whereas storage-centric ISP remains in a persistent regime where the library is always resident and throughput scales with on-package concurrency. This gap explains why ISP architectures retain large speed and energy advantages exactly in the regime that motivates repository-scale OMS.

 






==> BACKUP/BACKUP_Discussion.tex <==
\section{Discussions}

\sumukh{Things to add/polish : looks text heavy right now, we need to incorporate specific results and inferences from the result sections }

\sumukh{algorithmic comparison and BER}

\cesong{Mid scale vs.  Datacenter scale --> Which device has which bottleneck? }


\subsection{\textbf{Insights and Implications for OMS System Design}}
From the above architectural analysis and evaluation, several key insights emerge for designing next-generation OMS accelerators:

\noindent\textbf{Working-set residency vs.\ staging bandwidth.} Our unified evaluation shows that OMS throughput is compute-limited only when the full reference database resides in device memory. Once the library must be streamed from storage, performance becomes dominated by data movement through the storage-host-device path In the HEK dataset (2.99M references), GPU implementations of HyperOMS achieve high QPS--up to $\sim$101$\times$ speedup on the H100--only when the library fits in 80\,GB HBM. For the 1\,TB synthetic library, however, the same GPU runs are limited by transfers: speedups compress to $\sim$80$\times$ . Device-resident designs (DRAM NMP, ReRAM/PCM IMP and NAND/FeNAND ISP) avoid this stall, sustaining x times speedup and nergy efficiency. by keeping references in place and streaming only the compact top-$k$ results off the device. Thus, OMS accelerators must prioritize data locality--either by $S\le C_{\mathrm{dev}}$.



\noindent\textbf{Amortizing one-time programming costs.} Emerging non-volatile memories (PCM, ReRAM, and flash) are asymmetric: writes are slower and more energy-intensive than reads, and write-verify cycles can be expensive (and may require initial verification or reprogramming steps). Yet OMS workloads are overwhelmingly read-dominated: the library is encoded once and then re-used across batches of queries. In our study, including the one-time load reduces energy efficiency only modestly (e.g., FeNAND drops from $\sim$766k$\times$ to $\sim$658k$\times$ on HEK) because programming cost is amortized over many searches. Consequently, even technologies with slow writes (PCM, ReRAM) remain practical for OMS when the reference data are mostly static, since the cost is spread across a billion-scale corpus. Designers should therefore optimize the read and similarity kernels and treat write operations as an upfront provisioning step.



\noindent \textbf{Leverage internal parallelism of memory-centric devices:} Memory and storage-centric accelerators exploit the fine-grained parallelism inside memory arrays to sustain performance as datasets grow. For example, a DRAM-based near-memory design can activate many banks/subarrays in parallel, turning internal DDR row-access bandwidth into massive search throughput. Likewise, ReRAM and PCM-based in-memory processors execute thousands of analog operations concurrently across crossbar rows and columns, while 3D NAND/FeNAND in-storage processing occurs in parallel across pages, planes, and dies. These architectures show that scaling out through parallelism at the data source (banks, crossbar cells, or flash pages) allows throughput to grow with the data volume. In practice, this means designing OMS systems to fully utilize internal device concurrency (bitline-wise, bank-wise, plane-wise operations) is key to maintaining high throughput as the database scales up.


\noindent \textbf{Incorporate error tolerance and device variability into the design:} Pushing computation into dense memories and analog domains introduces reliability challenges~\cite{ielmini2018inmemory,sebastian2020memdevices}. Devices like ReRAM and PCM suffer from cell variability, drift in stored voltage values, and limited write endurance, which can lead to bit errors in computations~\cite{burr2010drift,ielmini2018inmemory}. In multi-level operation, threshold-voltage shifts and reduced sensing margins manifest as effective bit-error rates (BER) at readout; accordingly, we treat BER as an explicit design parameter at the algorithm and in-memory/near-memory compute levels. A key result of our study is that algorithm-architecture co-design for error resilience is not just beneficial but necessary~\cite{kanerva2009hdc,rahimi2016hdc}. In practice, this means using robust encoding schemes that can tolerate a degree of noise or bit flips, combined with lightweight error mitigation in hardware (ECC on result paths, periodic refresh or recalibration for multi-bit cells)~\cite{rahimi2016hdc,qureshi2010ecp}. In our bit-error injection experiments on HyperOMS, binary Hamming similarity retained \mbox{$\sim$96\%} of the reference identifications at 5\% BER and \mbox{$\sim$92\%} at 15\% BER, indicating smooth, non-catastrophic degradation under realistic error envelopes. In our analysis we did not use ECC; we observed that OMS search accuracy can be preserved under moderate error rates (on the order of a few percent) with these techniques. Thus, future OMS accelerators must be designed with explicit error budgets, or investigate the trade-offs of adding ECC, embracing architectures and algorithms that degrade gracefully in the face of device non-idealities~\cite{ielmini2018inmemory}. This co-design approach ensures that the large gains from in-memory/analog computation are not nullified by reliability issues.





 
\noindent\textbf{Periphery and I/O as design considerations.} While the memory arrays perform similarity operations with extreme parallelism, the surrounding circuitry often sets the performance ceiling~\cite{shafiee2016isaac,chi2016prime}. Sense amplifiers, ADC/DACs, page buffers, and on-chip controllers add latency and consume energy~\cite{shafiee2016isaac}. For example, periphery accounts for a significant portion of the energy and area budgets in state-of-the-art PCM designs~\cite{fan2024specpcm}; scaling these blocks to advanced nodes yields diminishing returns because analog conversion requirements and sensing margins limit further shrink. Similarly, the bandwidth of control links (e.g., the host-to-DIMM interface in NMP or the internal bus in an SSD) can constrain an otherwise massively parallel device. Moreover, key peripheral blocks (sense amps, page buffers, ADC/DACs) scale poorly with process node, so area and energy do not shrink proportionally; in practice, they must be time-multiplexed or shared across tiles/planes to maintain density and efficiency~\cite{murmann2020adc,chi2016prime}. Finally, the host--device interface must be provisioned to avoid bottlenecks when streaming queries and top-$k$ results: a conservative 64-bit, 200\,MHz control link per device suffices for kilohertz-rate query traffic and avoids saturating the interconnect. Therefore, accelerators need holistic co-optimization of periphery, interconnect, and memory cores to realize their theoretical gains.


==> BACKUP/BACKUP_Evaluation.tex <==


\definecolor{resultpurple}{HTML}{7B1FA2}
\newcommand{\result}[1]{\textcolor{resultpurple}{\bfseries #1}}




\subsection{Experimental Setup}

We evaluate OMS accelerators under a common methodology that (i) holds the OMS workload and scoring objective fixed across substrates and (ii) uses a unified reporting convention that cleanly separates steady-state kernel execution from the one-time cost of making the staged working set resident. Table~\ref{tab:hw_summary} summarizes the evaluated platforms, per-package capacities, and the search primitives used in each mapping.


\textbf{Reporting convention.}
We report throughput and energy as \emph{search-only} and \emph{search + $1\times$ load}. \emph{Search-only} assumes the staged working set for a batch is already resident in the executing substrate (e.g., HBM/GDDR, device-side DRAM, or a pre-programmed non-volatile array). \emph{Search + $1\times$ load} adds the one-time cost to make that working set resident: DMA staging into GPU memory, NAND$\rightarrow$DRAM refills on near-storage FPGA systems, or host$\rightarrow$DRAM provisioning for volatile memory-centric designs. This separation isolates kernel efficiency from the staging overhead that dominates in the transient regime defined in Section~\ref{sec:oms-scaling}.


\textbf{GPUs.}
We measure throughput and energy on an NVIDIA RTX~4090 (GDDR6X, 24\,GB, $\sim$1\,TB/s) using three kernels: \textit{ANN-SoLo} (FP32 cosine), \textit{HOMS-TC} (INT8 tensor-core HDC), and \textit{HyperOMS} (binary HDC). Representative results are then scaled to an NVIDIA H100 (HBM3, 80\,GB, $\sim$3.35\,TB/s) using bandwidth and effective compute normalization. When the staged footprint $S$ exceeds the resident capacity $C_{\mathrm{res}}$, the GPU operates in the transient regime by streaming shards over the external interface; otherwise, the working set remains resident and is reused across batches.


\textbf{Near-storage FPGAs.}
For the FPGA path, we anchor search latency and power using a Samsung/Xilinx SmartSSD CSD (Kintex UltraScale+) and scale to a Xilinx Versal VP1902-class design co-located with NVMe storage and attached to board DRAM. RapidOMS~\cite{pinge2024rapidoms} implements XOR+popcount engines with parametric lane parallelism and supports metadata-driven pruning to reduce unnecessary comparisons. We report both search-only and search + $1\times$ load, where the load term captures NAND$\rightarrow$DRAM refills when the hot working set exceeds the device-side buffer.


\textbf{DRAM-NMP.}
For DRAM near-memory processing, we assume commodity DDR4 modules and model near-bank primitives and scan timing following Kang~et~al.~\cite{kang2024dram}. Write energy follows Kim~et~al.~\cite{kim2013memory}. We scale capacity and controller timing to 64\,GB modules for parity with our mid-scale regime and treat the provisioned set of modules as the executing substrate, with their aggregate capacity defining $C_{\mathrm{res}}$ in our workload model.


\textbf{ReRAM/PCM IMP.}
For ReRAM and PCM IMP designs, we adopt an in-array storage scenario in which reference hypervectors are programmed into crossbar arrays and reused across searches. We model 0.2\,TB per chip as a conservative capacity-normalized target comparable to high-density flash packages. ReRAM OMS follows~\cite{fan2024mlcrram}; write energy is taken from Chen~et~al.~\cite{chen2016design}, and latency/energy parameters are grounded in 40\,nm prototypes. For PCM, we use \textit{SpecPCM}~\cite{fan2024specpcm} for bandwidth and write energy and scale peripheral circuitry (drivers, sense/readout, and control) to the same 0.2\,TB target. Unless otherwise noted, we model both ReRAM and PCM with TLC (3\,bits/cell) and default \emph{no write-verify}; because the reference library is written once and then read repeatedly, we treat verify overhead as a sensitivity rather than a mainline term.


\textbf{3D NAND / 3D FeNAND ISP.}
For 3D NAND and FeNAND ISP designs, we adopt device parameters, latency/energy models, and the ISP flow from Hsu~et~al.~\cite{hsu2025fenand}. Across all memory- and storage-centric designs (DRAM-NMP, ReRAM, PCM, 3D NAND, FeNAND), references are resident within the substrate (arrays or provisioned memory modules), queries are broadcast, and only compact indices and scores are returned. Unless otherwise noted, we assume a conservative 64-bit, 200\,MHz host/control interface sufficient for query broadcast and top-$k$ egress, and we include peripheral overheads (sense paths, mixed-signal where applicable, and controller logic) in both latency and energy. Technology nodes are normalized to representative processes (GPU 5\,nm, FPGA 7\,nm, DRAM 22--28\,nm, ReRAM/PCM 40\,nm, and NAND/FeNAND with 14\,nm arrays and 7\,nm CMOS periphery).


% \subsection{Datasets}\label{sec:datasets}
% \textbf{HEK293 (HEK).}
% For the HEK setting (Table~\ref{tab:datasets}), we evaluate 24 peak files with an average of 46{,}665 spectra (queries) per file, using subsets b1906--b1931. Each spectrum is embedded as an $8{,}192$-D vector. Searches are run against the MassIVE-KB human spectral library with $N=2{,}992{,}672$ references. Different baselines use different reference encodings: ANN-SoLo uses a sparse peak representation (m/z--intensity pairs) with shifted dot-product scoring, whereas HOMS-TC and HyperOMS use dense HDC hypervectors. As a result, the library footprints differ: the ANN-SoLo library is $\sim$10\,GB, the INT8 HDC library is $\sim$22.83\,GB, and the binary HDC library is $\sim$2.85\,GB.


% \textbf{Scaled (terabyte) workload.}
% To study datacenter-scale behavior under the transient regime, we construct a terabyte-scale workload with 15{,}000 queries and $N=10^9$ binary references ($8{,}192$-D), totaling $\sim$0.95\,TiB ($\approx 1$\,TB). This workload is intentionally beyond the resident capacity of a single GPU, so the GPU baseline executes by streaming shards over the external interface (captured in the \emph{search + $1\times$ load} term), whereas flash-based ISP executes in-place within SSD-scale 3D NAND/FeNAND packages. For capacity-normalized mid-scale comparisons, we additionally report results where each substrate is provisioned to equal per-package capacity, using the same search-only versus search+$1\times$ load convention to separate steady-state kernel efficiency from staging overhead.







% % ======= TABLE 1 (5 columns): Hardware/Modeling Summary =======
% \begin{table*}[t]
%   \centering
%   \caption{Hardware configurations, per-chip capacity, search primitives, and primary sources. References reside in-device for IMP/ISP designs.}
%   \label{tab:hw_summary}
%   \adjustbox{max width=\textwidth}{
%   \begin{tabularx}{\textwidth}{l l l l l}
%     \toprule
%     \textbf{Accelerator} & \textbf{Device} & \textbf{Capacity / Chip} & \textbf{Search Primitive} & \textbf{Source} \\
%     \midrule
%     GPU & RTX~4090 & 24\,GB (GDDR6X) & ANN-SoLo (FP32); HOMS-TC (INT8); HyperOMS (BIN) & \cite{bittremieux2019extremely,kang2023homstc,kang2022massively} \\
%     GPU & H100 & 80\,GB (HBM2E) & Same primitives as RTX~4090 &  \hspace{1mm}- \\
%     FPGA & Versal VP1902 & 64\,GB (DDR4-2400) & Streaming XOR+popcount lanes with on-fabric reduction & \cite{pinge2024rapidoms} \\
%     DRAM NMP & DDR4 DIMM (NMP) & 64\,GB (DDR4-2400) &  XOR with bit-serial popcount; subarray/bank-parallel scan & \cite{kim2013memory,kang2024dram} \\
%     ReRAM IMP & 40\,nm arrays + periph. & 0.2\,TB/chip & Analog VMM; HDC match (BIN/MLC); no write-verify & \cite{fan2024mlcrram,chen2016design} \\
%     PCM IMP & 40\,nm arrays + periph. & 0.2\,TB/chip & Analog VMM; HDC match (BIN/MLC); no write-verify & \cite{fan2024specpcm} \\
%     3D NAND ISP & 14\,nm arrays + 7\,nm CMOS & 0.2\,TB/chip & In-storage Hamming/bitwise; on-package reduction & \cite{hsu2025fenand} \\
%     3D FeNAND ISP & 14\,nm arrays + 7\,nm CMOS & 0.2\,TB/chip & In-storage Hamming/bitwise; on-package reduction & \cite{hsu2023memsys} \\
%     \bottomrule
%   \end{tabularx}}
% \end{table*}



% % ======= TABLE 2: Datasets =======
% \begin{table}[t]
%   \centering
%   \caption{Datasets used in evaluation. Binary HDC embeddings use 8{,}192 dimensions unless noted.}
%   \label{tab:datasets}
%   \begin{tabular}{l r r l}
%     \toprule
%     \textbf{Dataset} & \textbf{\#Queries} & \textbf{\#References} & \textbf{Notes} \\
%     \midrule
%     HEK293 & 46{,}665 & 2{,}992{,}672 & 24 peak files; MassIVE-KB library \\
%     Synthetic & 15{,}000 & 1{,}000{,}000{,}000 & $\sim$1\,TB binary store (8{,}192-D) \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \subsection{Experimental Setup}

% We evaluate OMS accelerators under a common methodology that holds constant the placement of the reference library and the host–device I/O path for queries and results. Table~\ref{tab:hw_summary} summarizes the platform configurations, per-chip capacities, and search primitives used in our evaluation. For GPUs, we measure throughput and energy on an NVIDIA RTX~4090 (GDDR6X, 24\,GB, $\sim$1\,TB/s) using three kernels—\textit{ANN-SoLo} (FP32 cosine), \textit{HOMS-TC} (HDC on INT8 tensor cores), and \textit{HyperOMS} (HDC with binary encodings)—and scale these measurements to an NVIDIA H100 (HBM2E, 80\,GB, $\sim$3.35\,TB/s) using bandwidth/compute normalization (memory bandwidth and effective TOPS). For the FPGA path, we use a near-storage configuration on a Samsung/Xilinx SmartSSD CSD (Kintex UltraScale+) to anchor search latency and power, and then scale to a Xilinx Versal VP1902 attached to a 64\,GB DDR4-2400 RDIMM (effective $\sim$19.2\,GB/s). For DRAM NMP, we assume the same DDR4 module and model near-memory primitives; write energy follows Kim~et~al.~\cite{kim2013memory}, while peripheral behavior and search latency follow Kang~et~al.~\cite{kang2024dram}. Although prior DRAM-NMP results assume 8\,GB DIMMs, we scale capacities and controller timing to 64\,GB for fair comparison.

% For ReRAM and PCM IMP designs, we adopt an in-array storage scenario in which the full reference library resides in the device, modeling 0.2\,TB per chip. This capacity reflects a conservative, near-future target comparable to modern high-density NAND packages and is plausible for 3D-integrated ReRAM/PCM with MLC/TLC operation. ReRAM OMS follows \cite{fan2024mlcrram}; write energy is taken from Chen~et~al.~\cite{chen2016design}, and search latency as well as read/write energy are grounded in 40\,nm fabricated prototypes. For PCM, we use \textit{SpecPCM}~\cite{fan2024specpcm} for write energy and bandwidth; the peripheral circuitry (drivers, sense/readout, and control at 500~MHz, assuming single-wordline activation per cycle) is scaled to a 0.2\,TB target and, for parity, the same peripheral methodology is applied to ReRAM. We choose the Sb$_2$Te$_3$/Ge$_4$Sb$_6$Te$_7$ PCM case fabricated at 40\,nm in \cite{fan2024specpcm}. Both ReRAM and PCM are modeled as TLC (3\,bits/cell) with default \emph{no write-verify}. Because the reference library is written once and reused across searches, we ignore verify overhead in the mainline results. 

% For 3D NAND and FeNAND ISP designs, we adopt device parameters, latency/energy models, and the ISP flow from Hsu~et~al.~\cite{hsu2025fenand}. Across all memory/storage-centric devices (DRAM NMP, ReRAM, PCM, 3D NAND, FeNAND), references are stored directly in the array, queries are broadcast to all devices, and indices/similarity scores are read out sequentially. Unless noted otherwise, we assume a 64-bit, 200\,MHz host/control interface,
% matching conservative clocking and AXI-class widths in 7\,nm periphery, sufficient for query broadcast and top-$k$ egress. Given that the reference library is written once and then read repeatedly, we ignore write-verify overhead in the main results. We include peripheral overheads (sense paths, lightweight mixed-signal where applicable, and controller logic) in both latency and energy, and normalize technology nodes to representative processes: GPU 5\,nm, FPGA 7\,nm, DRAM 22–28\,nm, ReRAM 40\,nm, PCM 40\,nm, and NAND/FeNAND with 14\,nm arrays and 7\,nm CMOS periphery. We treat mature hardware measurements as golden baselines for device/array-level simulations and use a unified reporting convention of \emph{search-only} versus \emph{search + one-time reference load.}


% For the \textbf{Synthetic} setting, we construct a terabyte-scale workload to study billion-scale behavior: 15{,}000 queries and 1{,}000{,}000{,}000 binary references (8{,}192-D), totaling $\sim$0.95\,TiB ($\sim$1\,TB). During search, the full reference database resides in device-local memory to exclude host/storage I/O. Concretely, the RTX~4090 uses on-board GDDR6X (24\,GB, $\sim$1\,TB/s), the H100 uses HBM2E (80\,GB, $\sim$3.35\,TB/s), and the FPGA path uses board DRAM on a VP1902-class design. Memory-centric devices store references directly in the array. To hold $\sim$1\,TB of references, we replicate devices by capacity: $\sim$43$\times$ RTX~4090, $\sim$13$\times$ H100, $\sim$16$\times$ VP1902 (with DRAM), $\sim$16$\times$ DRAM-NMP devices, and $\sim$5 chips each for ReRAM, PCM, 3D NAND, and FeNAND (assuming 0.2\,TB/chip for NVM/ISP). We reuse the same normalization and scaling methodology as above, including the \emph{search + one-time reference load} reporting convention.


% ==================================================================
% ==================================================================
% ==================================================================


% % --- table helpers (ensure these are in preamble if not already) ---
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \definecolor{resultpurple}{HTML}{7B1FA2}
% %\newcommand{\result}[1]{\textcolor{black}{\bfseries #1}}
% \setlength{\tabcolsep}{4pt}
% \renewcommand\theadfont{\normalsize\bfseries}

% % ================== TABLE 3: HEK DATASET ==================
% \begin{table*}[t]
%   \centering
%   \caption{HEK dataset: normalized energy efficiency and speedup across platforms.}
%   % ---------- GPU PART ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{GPU}}
%     \label{tab:hek}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
%       Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
%       Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
%       \midrule
%       % Energy efficiency (search) &
%       % \result{1.000} & \result{9.696} & \result{18.814} &
%       % \result{1.926} & \result{18.714} & \result{36.246} \\
%       Energy efficiency (search + load) &
%       \result{1.0} & \result{9.7} & \result{18.8} &
%       \result{1.9} & \result{18.7} & \result{36.2} \\
%       Speedup &
%       \result{1.000} & \result{23.661} & \result{33.769} &
%       \result{2.996} & \result{70.897} & \result{101.166} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}

%   \vspace{0.6em}

%   % ---------- OTHERS ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{FPGA / NMP / IMP / ISP}}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
%       Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
%       Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
%       \midrule
%       % Energy efficiency (search) &
%       % \result{53.454} & \result{1,233.125} & \result{126,792.305} &
%       % \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\
%       Energy efficiency (search + load) &
%       \result{53.5} & \result{1,201.9} & \result{112,190.8} &
%       \result{257,166.2} & \result{66,041.6} & \result{657,605.8} \\
%       Speedup &
%       \result{98.375} & \result{60.912} & \result{77.962} &
%       \result{239.541} & \result{389.675} & \result{389.675} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}
% \end{table*}

% % ============== TABLE 4.0: SYNTHETIC - ENTIRE DATASET ==============
% \begin{table*}[t]
%   \centering
%   \caption{Synthetic dataset (entire library, single device).}
%   % ---------- GPU PART ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{GPU}}
%     \label{tab:syn-entire-1device}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
%       Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
%       Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
%       Capacity/Chip & {24\,GB} & {24\,GB} & {24\,GB} & {80\,GB} & {80\,GB} & {80\,GB} \\
%       Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {3.17\,TB} & {8\,TB} & {1\,TB} \\
%       Devices required (GPUs) & {136.0} & {342.0} & {43.0} & {41.0} & {103.0} & {13.0} \\
%       \midrule
%       Energy efficiency (search) &
%       \result{1.000} & \result{9.621} & \result{18.783} &
%       \result{1.931} & \result{18.431} & \result{37.125} \\
%       Energy efficiency (search + load) &
%       \result{1.0} & \result{9.6} & \result{18.8} &
%       \result{1.9} & \result{18.7} & \result{36.2} \\
%       Speedup &
%       \result{1.000} & \result{59.201} & \result{10.668} &
%       \result{0.903} & \result{53.453} & \result{9.663} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}

%   \vspace{0.6em}

%   % ---------- OTHERS ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{FPGA / NMP / IMP / ISP}}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
%       Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
%       Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
%       Capacity/Chip & {64\,GB} & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\
%       Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\
%       Devices required & {16.0} & {16.0} & {5.0} & {5.0} & {5.0} & {5.0} \\
%       \midrule
%       Energy efficiency (search) &
%       \result{53.173} & \result{1,092.076} & \result{126,834.526} &
%       \result{304,658.462} & \result{92,452.364} & \result{766,792.413} \\
%       Energy efficiency (search + load) &
%       \result{53.5} & \result{1,140.9} & \result{126,834.526} &
%       \result{304,658.462} & \result{92,452.364} & \result{766,792.413} \\
%       Speedup &
%       \result{10.164} & \result{6.600} & \result{2.388} &
%       \result{3.359} & \result{8.169} & \result{8.169} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}
% \end{table*}


% % ============== TABLE 4.1: SYNTHETIC - ENTIRE DATASET ==============
% \begin{table*}[t]
%   \centering
%   \caption{Synthetic dataset (single device for volatile-memory systems; entire library stored in non-volatile memory systems).}
%   % ---------- GPU PART ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{GPU}}
%     \label{tab:syn-entire}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
%       Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
%       Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
%       Capacity/Chip & {24\,GB} & {24\,GB} & {24\,GB} & {80\,GB} & {80\,GB} & {80\,GB} \\
%       Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {3.17\,TB} & {8\,TB} & {1\,TB} \\
%       Devices required (GPUs) & {1.0} & {1.0} & {1.0} & {1.0} & {1.0} & {1.0} \\
%       \midrule
%       Energy efficiency (search + load) &
%       \result{1.000} & \result{9.621} & \result{18.783} &
%       \result{1.931} & \result{18.431} & \result{37.125} \\
%       Speed up (pure search) &
%       \result{1.000} & \result{23.712} & \result{33.781} &
%       \result{2.996} & \result{71.033} & \result{101.198} \\
%       Speedup (search + load) &
%       \result{1.000} & \result{15.623} & \result{31.136} &
%       \result{2.945} & \result{27.822} & \result{79.724} \\
%       \textit{Speedup drop (\%)}\footnotesize~(pure$\rightarrow$search\,+\,load) &
%       \result{-} & \result{34.1\%} & \result{7.8\%} &
%       \result{1.7\%} & \result{60.8\%} & \result{21.2\%} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}

%   \vspace{0.6em}

%   % ---------- OTHERS ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{FPGA / NMP / IMP / ISP}}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
%       Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
%       Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
%       Capacity/Chip & {64\,GB} & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\
%       Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\
%       Devices required & {1.0} & {1.0} & {5.0} & {5.0} & {5.0} & {5.0} \\
%       \midrule
%       Energy efficiency (search + load) &
%       \result{53.173} & \result{1,092.076} & \result{126,834.526} &
%       \result{304,658.462} & \result{92,452.364} & \result{766,792.413} \\
%       Speed up (pure search) &
%       \result{104.572} & \result{63.231} & \result{423.132} &
%       \result{3901.899} & \result{2874.126} & \result{2874.126} \\
%       Speedup (search + load) &
%       \result{53.930} & \result{56.587} & \result{426.888} &
%       \result{3936.533} & \result{2899.638} & \result{2899.638} \\
%       \textit{Speedup drop (\%)}\footnotesize~(pure$\rightarrow$search\,+\,load) &
%       \result{48.4\%} & \result{10.5\%} & \result{$\sim$0\%} &
%       \result{$\sim$0\%} & \result{$\sim$0\%} & \result{$\sim$0\%} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}
% \end{table*}





% % ============== TABLE 5: SYNTHETIC - SAME SPEED ==============
% \begin{table*}[t]
%   \centering
%   \caption{Synthetic dataset (device counts chosen to match GPU throughput; ``same speed'').}
%   % ---------- GPU PART ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{GPU}}
%     \label{tab:syn-same-speed}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
%       Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
%       Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
%       Capacity/Chip & {24\,GB} & {24\,GB} & {24\,GB} & {80\,GB} & {80\,GB} & {80\,GB} \\
%       Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {3.17\,TB} & {8\,TB} & {1\,TB} \\
%       Devices used (GPUs) & {136.0} & {6.0} & {5.0} & {46.0} & {2.0} & {2.0} \\
%       \midrule
%       Energy efficiency (search) &
%       \result{1.000} & \result{9.696} & \result{18.814} &
%       \result{1.931} & \result{18.715} & \result{37.258} \\
%       Energy efficiency (search + load) &
%       \result{1.0} & \result{9.621} & \result{18.783} &
%       \result{1.931} & \result{18.431} & \result{37.125} \\
%       Speedup & \result{1.0} & \result{1.0} & \result{1.0} &
%       \result{1.0} & \result{1.0} & \result{1.0} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}



%   \vspace{0.6em}

%   % ---------- OTHERS ----------
%   \begin{subtable}{\textwidth}
%     \caption*{\textbf{FPGA / NMP / IMP / ISP}}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabularx}{\textwidth}{l *{6}{Y}}
%       \toprule
%       Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
%       Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
%       Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
%       Capacity/Chip & {64\,GB} & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\
%       Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\
%       Devices used & {2.0} & {3.0} & {5.0} & {3.0} & {2.0} & {1.0} \\
%       \midrule
%       Energy efficiency (search) &
%       \result{53.454} & \result{1,233.125} & \result{126,792.305} &
%       \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\
%       Energy efficiency (search + load) &
%       \result{53.173} & \result{1,092.076} & \result{102,044.292} &
%       \result{247,826.935} & \result{74,048.676} & \result{695,146.160} \\
%       Speedup & \result{1.0} & \result{1.0} & \result{1.0} &
%       \result{1.0} & \result{1.0} & \result{1.0} \\
%       \bottomrule
%     \end{tabularx}}
%   \end{subtable}
% \end{table*}



% \begin{table*}[t]

%   \centering

%   \caption{Synthetic dataset (device counts chosen to match GPU throughput; ``same speed'').}

%   % ---------- GPU PART ----------

%   \begin{subtable}{\textwidth}

%     \caption*{\textbf{GPU / FPGA}}

%     \label{tab:syn-same-speed}

%     \adjustbox{max width=\textwidth}{

%     \begin{tabularx}{\textwidth}{l *{4}{Y}}

%       \toprule

%       Device / Memory Type & {H100} & {H100} & {H100} & {FPGA} \\

%       Process/Device & {} & {} & {} & {VP1902} \\

%       Algorithm / Searching Type & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {Digital} \\

%       Data Type & {FP32} & {INT8} & {BIN} & {BIN} \\

%       Capacity/Chip & {80\,GB} & {80\,GB} & {80\,GB} & {64\,GB} \\

%       Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {1\,TB} \\

%       Devices used & {46.0} & {2.0} & {2.0} & {2.0} \\

%       \midrule

%       Energy efficiency (search) &

%       \result{1.931} & \result{18.715} & \result{37.258} & \result{53.454} \\

%       Energy efficiency (search + load) &

%       \result{1.931} & \result{18.431} & \result{37.125} & \result{53.173} \\

%       Speedup &

%       \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} \\

%       \bottomrule

%     \end{tabularx}}

%   \end{subtable}







%   \vspace{0.6em}



%   % ---------- OTHERS ----------

%   \begin{subtable}{\textwidth}

%     \caption*{\textbf{NMP / IMP / ISP}}

%     \adjustbox{max width=\textwidth}{

%     \begin{tabularx}{\textwidth}{l *{5}{Y}}

%       \toprule

%       Memory Type & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\

%       Process/Device & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\

%       Searching Type & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\

%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\

%       Capacity/Chip & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\

%       Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\

%       Devices used & {3.0} & {5.0} & {3.0} & {2.0} & {1.0} \\

%       \midrule

%       Energy efficiency (search) &

%       \result{1,233.125} & \result{126,792.305} &

%       \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\

%       Energy efficiency (search + load) &

%       \result{1,092.076} & \result{102,044.292} &

%       \result{247,826.935} & \result{74,048.676} & \result{695,146.160} \\

%       Speedup & \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} \\

%       \bottomrule

%     \end{tabularx}}

%   \end{subtable}

% \end{table*}









% \begin{table*}[t]

%   \centering

%   \caption{Synthetic dataset (device counts chosen to match GPU throughput; ``same speed'').}

%   % ---------- GPU PART ----------

%   \begin{subtable}{\textwidth}

%     \caption*{\textbf{GPU / FPGA}}

%     \label{tab:syn-same-speed}

%     \adjustbox{max width=\textwidth}{

%     \begin{tabularx}{\textwidth}{l *{4}{Y}}

%       \toprule

%       Device / Memory Type & {H100} & {H100} & {H100} & {FPGA} \\

%       Process/Device & {} & {} & {} & {VP1902} \\

%       Algorithm / Searching Type & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {Digital} \\

%       Data Type & {FP32} & {INT8} & {BIN} & {BIN} \\

%       Capacity/Chip & {80\,GB} & {80\,GB} & {80\,GB} & {64\,GB} \\

%       Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {1\,TB} \\

%       Devices used & {242.0} & {7.0} & {103.0} & {72.0} \\

%       \midrule

%       % Energy efficiency (search) &

%       % \result{1.000} & \result{11.206} & \result{19.292} & \result{27.677} \\

%       Energy efficiency (search + load) &

%       \result{0.1} & \result{1.0} & \result{1.7} & \result{2.5} \\

%       Speedup &

%       \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} \\

%       \bottomrule

%     \end{tabularx}}

%   \end{subtable}







%   \vspace{0.6em}



%   % ---------- OTHERS ----------

%   \begin{subtable}{\textwidth}

%     \caption*{\textbf{NMP / IMP / ISP}}

%     \adjustbox{max width=\textwidth}{

%     \begin{tabularx}{\textwidth}{l *{5}{Y}}

%       \toprule

%       Memory Type & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\

%       Process/Device & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\

%       Searching Type & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\

%       Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\

%       Capacity/Chip & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\

%       Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\

%       Devices used & {85.0} & {130.0} & {112.0} & {80.0} & {33.0} \\

%       \midrule

%       % Energy efficiency (search) &

%       % \result{638.493} & \result{65,651.135} &

%       % \result{157,695.025} & \result{47,854.499} & \result{396,901.331} \\

%       Energy efficiency (search + load) &

%       \result{34.4} & \result{581.8} &

%       \result{1,383.3} & \result{464.1} & \result{8,047.3} \\

%       Speedup & \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} & \result{1.0} \\

%       \bottomrule

%     \end{tabularx}}

%   \end{subtable}

% \end{table*}




\subsection{Accuracy Preservation}
\label{sec:acc_preservation}
% HDC-based methods achieve consistent identifications under device-level bit errors.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{fig/final_identifications_comparison_ber_withdrops.pdf}
  \caption{Impact of injected bit error rate (BER) on HyperOMS identifications for datasets b1906--b1931.}
  \label{fig:hyperoms-ber}
\end{figure}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{fig/upset.pdf}%
  \caption{Identification consistency across BER levels (UpSet overlaps, b1906).}
  \label{fig:UPSET}
\end{figure*}



Before comparing performance, we first establish that HyperOMS preserves identification accuracy under the device-level errors expected in memory-centric deployments. Concretely, we inject random bit flips into the binary hypervectors at a controlled bit error rate (BER), modeling readout uncertainty under tight sensing margins in multi-level non-volatile memories. The BER levels we sweep are aligned with regimes reported for higher bits-per-cell operation in ReRAM/PCM arrays, and therefore represent a realistic operating stress rather than an adversarial corruption model~\cite{fan2024mlcrram,fan2024specpcm}.


We evaluate robustness along two complementary axes. First, we measure \emph{coverage} via total identifications at a fixed FDR (Fig.~\ref{fig:hyperoms-ber}). Across datasets b1906--b1931, HyperOMS-BIN tracks the INT8 baseline closely for BER $\le 10\%$. At 15\% BER, the reduction in total identifications remains modest and dataset dependent (approximately 9--14\%), indicating that discovery coverage degrades smoothly as the error rate increases.

Total identifications alone cannot determine whether the same peptides are being recovered. We therefore evaluate identification \emph{consistency} using UpSet overlaps (Fig.~\ref{fig:UPSET}), which quantify agreement in high-confidence identifications across BER settings. In effect, totals summarize coverage, while overlaps test whether the reported set is stable under device noise. The measured resilience is consistent with hyperdimensional computing: binary encodings with Hamming-style similarity distribute information across many dimensions, so random bit flips tend to average out rather than induce catastrophic rank changes.


To operationalize this notion of consistency, we summarize UpSet overlaps for dataset b1906 across BER $\in \{0,5,10,15\%\}$. Because ground truth is not available for HEK293, we treat the \emph{consensus} between ANN-SoLo and HOMS-TC (INT8) as a proxy reference set: this intersection captures identifications that are supported by both a conventional scoring baseline and an 8-bit HDC baseline, and is therefore a conservative approximation of ``high-confidence'' peptides for comparing robustness. We then quantify \emph{recovery} as the fraction of this proxy consensus that is also identified by HyperOMS-BIN:

{\footnotesize
\begin{equation}
\mathrm{Recovery} \;=\; 
\frac{|\mathrm{ANN}\_\mathrm{SoLo} \cap \mathrm{HOMS\text{-}TC} \cap \mathrm{HyperOMS}\_\mathrm{BIN}|}
{|\mathrm{ANN}\_\mathrm{SoLo} \cap \mathrm{HOMS\text{-}TC}|}
\end{equation}
}

Using the verified counts, recovery is $96.78\%$ at $0\%$ BER, $95.73\%$ at $5\%$ BER, $94.47\%$ at $10\%$ BER, and $91.41\%$ at $15\%$ BER. Thus, agreement with the proxy consensus remains high through $10\%$ BER and shrinks moderately at $15\%$ BER, with most differences concentrated near the reporting threshold rather than reflecting wholesale rank shifts. Taken together, total identifications and UpSet overlaps indicate that HyperOMS maintains substantial discovery coverage and preserves a large fraction of high-confidence peptides under realistic device-level BER, supporting its suitability for memory-centric deployments.

\sumukh{fixed until here}








% To complement total identifications, we summarize identification consistency with UpSet plots (Fig.\ref{fig:UPSET}) for dataset b1906 across BER $\in \{0,5,10,15\%\}$. Because ground truth is not available for HEK293, we treat the consensus of ANN-SoLo and HOMS-TC (INT8) as a proxy reference and quantify HyperOMS recovery of that consensus. Here, \emph{recovery} is the size of the three-way intersection (ANN\_SoLo $\cap$ HyperOMS\_BIN $\cap$ HOMS-TC) divided by the sum of the two-way consensus (ANN\_SoLo $\cap$ HOMS-TC) and that three-way intersection. Using the verified counts, recovery is $96.78\%$ at $0\%$ BER, $95.73\%$ at $5\%$ BER, $94.47\%$ at $10\%$ BER, and $91.41\%$ at $15\%$ BER. The consensus remains close to the $0\%$ BER reference through $10\%$ BER and shrinks moderately at $15\%$ BER, with most differences concentrated near the reporting threshold rather than reflecting wholesale rank shifts. Taken together, the UpSet overlaps provide the accuracy-oriented counterpart to totals: they show that HyperOMS preserves the bulk of high-confidence identifications while degrading smoothly as BER increases, consistent with the robustness of HDC encodings and Hamming-style similarity.


% Taken together, the totals and the UpSet overlaps indicate that HyperOMS maintains substantial identification coverage and preserves a large fraction of high-confidence peptides under realistic device-level error, supporting its suitability for memory-centric deployments.






% ================== TABLE: HEK DATASET (MANAGEABLE) ==================
\begin{table*}[t]
  \centering
  \caption{HEK293 (Human Embryonic Kidney 293) dataset: Algorithmic comparisions with normalized energy efficiency and speedup across platforms (normalized to RTX~4090 FP32 ANN-SoLo = 1.0). We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
  \label{tab:hek-managed}
  \adjustbox{max width=\textwidth}{
  \begin{tabularx}{\textwidth}{l *{6}{Y}}
    \toprule
    Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
    Memory & {GDDR6X} & {GDDR6X} & {GDDR6X} & {HBM3} & {HBM3} & {HBM3} \\
    Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
    Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
    \midrule
    Energy efficiency (search-only) &
    \result{1.000} & \result{9.696} & \result{18.814} &
    \result{1.931} & \result{18.715} & \result{37.258} \\
    Energy efficiency (search + 1$\times$ write/load) &
    \result{1.000} & \result{9.671} & \result{18.804} &
    \result{1.931} & \result{18.613} & \result{37.211} \\
    \midrule
    Speedup (search-only) &
    \result{1.000} & \result{23.712} & \result{33.781} &
    \result{2.996} & \result{71.033} & \result{101.198} \\
    Speedup (search + 1$\times$ write/load) &
    \result{1.000} & \result{20.517} & \result{32.944} &
    \result{2.979} & \result{48.402} & \result{93.621} \\
    \bottomrule
  \end{tabularx}}
\end{table*}

% ================== TABLE: HEK DATASET (PART B: HyperOMS-only) ==================
\begin{table*}[t]
  \centering
  \caption{HEK293 (Human Embryonic Kidney 293) dataset (Part B): HyperOMS (BIN) across platforms for an equitable comparison. We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
  \label{tab:hek-hyperoms-only}
  \adjustbox{max width=\textwidth}{
  \begin{tabularx}{\textwidth}{l *{8}{Y}}
    \toprule
    Platform / Device & {RTX 4090} & {H100} & {VP1902} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
    Memory / Tech. & {GDDR6X} & {HBM3} & {FPGA} & {NMP} & {40\,nm} & {\textcolor{red}{TBD}} & {ISP} & {ISP} \\
    Method / Type & {GPU HDC} & {GPU HDC} & {NSP} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
    Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
    \midrule
    Energy efficiency (search-only) &
    \result{1.000} & \result{1.980} & \result{2.841} & \result{65.543} &
    \result{6,737.430} & \result{16,187.919} & \result{4,912.424} & \result{40,743.243} \\
    Energy efficiency (search + 1$\times$ write/load) &
    \result{1.000} & \result{1.979} & \result{2.840} & \result{63.926} &
    \result{6,741.883} & \result{16,198.617} & \result{4,915.670} & \result{40,770.169} \\
    \midrule
    Speedup (search-only) &
    \result{1.000} & \result{2.996} & \result{3.096} & \result{1.872} &
    \result{2.505} & \result{23.101} & \result{17.016} & \result{17.016} \\
    Speedup (search + 1$\times$ write/load) &
    \result{1.000} & \result{2.842} & \result{2.769} & \result{1.765} &
    \result{2.576} & \result{23.755} & \result{17.498} & \result{17.498} \\
    \bottomrule
  \end{tabularx}}
\end{table*}



% ================== TABLE: HEK DATASET (LARGE, SCALED) ==================
\begin{table*}[t]
  \centering
  \caption{HEK dataset scaled (15{,}000 queries; 1{,}000{,}000{,}000 references; HDC BIN size = 1\,TB): normalized energy efficiency and speedup across platforms. We report both \emph{search-only} and \emph{search + one-time write/load (1$\times$)} results.}
  \label{tab:hek-large}
  \adjustbox{max width=\textwidth}{
  \begin{tabularx}{\textwidth}{l *{4}{Y}}
    \toprule
    Platform / Device & {H100} & {H100} & {3D NAND} & {FeNAND} \\
    Method & {GPU HDC} & {GPU HDC} & {ISP} & {ISP} \\
    Data Type & {INT8 (HOMS-TC)} & {BIN (HyperOMS)} & {BIN} & {BIN} \\
    \midrule
    Energy efficiency (search-only) &
    \result{1.000} & \result{1.991} & \result{4,938.364} & \result{40,958.387} \\
    Energy efficiency (search + 1$\times$ write/load) &
    \result{1.000} & \result{2.017} & \result{5,024.3} & \result{41,671.1} \\
    \midrule
    Speedup (search-only) &
    \result{1.000} & \result{1.425} & \result{8.092} & \result{8.092} \\
    Speedup (search + 1$\times$ write/load) &
    \result{1.000} & \result{2.866} & \result{20.844} & \result{20.844} \\
    \bottomrule
  \end{tabularx}}
\end{table*}




\subsection{Comparative Results}
\label{sec:comparative_results}

\subsubsection{Baseline Algorithmic Efficiency on GPUs (Table~\ref{tab:hek-managed})}
Having established that HyperOMS preserves identifications under realistic device-level BER (Section~\ref{sec:acc_preservation}), we next isolate the \emph{algorithmic} benefit of reduced-precision scoring on commodity GPUs. Table~\ref{tab:hek-managed} compares three software mappings on RTX~4090 and H100: a conventional FP32 baseline (ANN-SoLo), an INT8 tensor-core HDC baseline (HOMS-TC), and a binary HDC mapping (HyperOMS). All values are normalized to RTX~4090 FP32 ANN-SoLo.

On RTX~4090, moving from FP32 to HDC yields large gains even before considering cross-substrate locality. HOMS-TC achieves a $23.712\times$ speedup and $9.696\times$ higher energy efficiency in the search-only case, while HyperOMS further increases these to $33.781\times$ speedup and $18.814\times$ energy efficiency. Scaling to H100 amplifies the same trend: relative to the RTX~4090 FP32 baseline, ANN-SoLo on H100 improves to $2.996\times$ speedup and $1.931\times$ energy efficiency, whereas HOMS-TC reaches $71.033\times$ speedup and $18.715\times$ energy efficiency, and HyperOMS reaches $101.198\times$ speedup and $37.258\times$ energy efficiency. These results quantify the headroom unlocked by kernel simplification (INT8/BIN) on high-bandwidth GPUs, independent of any memory-centric data placement.

The search+$1\times$ write/load rows capture the one-time cost of making the working set resident for a run. For this HEK configuration, energy-efficiency trends remain essentially unchanged (e.g., RTX~4090 HyperOMS: $18.814\times \rightarrow 18.804\times$; H100 HyperOMS: $37.258\times \rightarrow 37.211\times$). The speedup impact is more visible when the search kernel is very fast, since a fixed staging cost becomes a larger fraction of end-to-end time (e.g., H100 HOMS-TC: $71.033\times \rightarrow 48.402\times$; H100 HyperOMS: $101.198\times \rightarrow 93.621\times$). Overall, Table~\ref{tab:hek-managed} establishes the GPU-side algorithmic gains from reduced precision, which we use as the baseline context for the cross-substrate comparisons that follow.

\subsubsection{Mid-Scale Cross-Substrate Comparison with a Unified HyperOMS Kernel (Table~\ref{tab:hek-hyperoms-only})}
Table~\ref{tab:hek-hyperoms-only} moves beyond algorithmic effects and evaluates \emph{substrate-dependent} efficiency under a unified kernel. Specifically, we fix the method to HyperOMS with binary HDC (BIN) across all platforms and normalize results to RTX~4090 running HyperOMS (search-only $=1.0$). This removes confounding from precision and scoring function, so the remaining differences primarily reflect where the reference library resides, how it is accessed (streamed vs.\ in-place), and the efficiency of the underlying memory-centric primitives and periphery.

Two trends emerge. First, commodity and near-storage accelerators provide only modest additional gains once the kernel is already reduced to XOR+popcount-style operations. Relative to RTX~4090 HyperOMS, H100 improves throughput by $\sim$3.0$\times$ (2.996$\times$ search-only) and energy efficiency by $\sim$2.0$\times$ (1.980$\times$), while a VP1902-class near-storage FPGA reaches $\sim$3.1$\times$ speedup (3.096$\times$) and $\sim$2.8$\times$ energy efficiency (2.841$\times$). These results indicate that, in the mid-scale regime, moving from a GPU implementation to a carefully pipelined FPGA stream primarily changes microarchitectural utilization and buffering, but does not fundamentally alter the data-movement path.

Second, memory- and storage-centric designs deliver \emph{orders-of-magnitude} energy gains by keeping the reference library resident within the executing substrate. DRAM-NMP improves energy efficiency to $65.543\times$ (search-only) while providing a comparable end-to-end speedup to the GPU baseline (1.872$\times$). Non-volatile IMP/ISP designs amplify this effect: ReRAM achieves $6.7\times 10^3\times$ energy efficiency with a $2.505\times$ speedup, PCM reaches $1.62\times 10^4\times$ energy efficiency with a $23.101\times$ speedup, and flash-based ISP delivers $4.9\times 10^3\times$ (3D NAND) to $4.07\times 10^4\times$ (FeNAND) energy efficiency while sustaining $\sim$17$\times$ speedup. The key distinction is that these substrates execute similarity in-place and export only compact results, shifting the dominant cost from host-device staging to internal array parallelism and periphery energy.

Finally, the search-only versus search+$1\times$ write/load rows remain close for most platforms in this table, because the benchmarked working set is treated as resident within each device’s evaluation model. Where a load term exists (e.g., for volatile buffering or provisioning), its impact is small relative to the steady-state gap in energy efficiency between streamed execution and persistent in-place execution. Overall, Table~\ref{tab:hek-hyperoms-only} shows that once the kernel is fixed, the main discriminator at mid-scale is \emph{data locality}: architectures that avoid repeatedly moving reference data across an external interface achieve one to four orders of magnitude higher energy efficiency while maintaining competitive throughput.



\subsubsection{Datacenter-Scale Scalability at the Terabyte Limit (Table~\ref{tab:hek-large})}
Table~\ref{tab:hek-large} stress-tests OMS at datacenter scale by increasing the binary reference library to $N=10^9$ ($\approx$1\,TB for $D{=}8192$ BIN), which is intentionally beyond the resident capacity of a single GPU. We normalize all results to H100 running the INT8 HDC baseline (HOMS-TC), and report both \emph{search-only} and \emph{search + $1\times$ write/load} to expose the impact of transient staging at this scale.

Two regimes become explicit. Under \emph{search-only}, the BIN kernel on H100 (HyperOMS) provides only a moderate benefit over INT8, improving energy efficiency by $1.991\times$ and speed by $1.425\times$. This reflects a pure kernel effect under the (idealized) assumption that the working set is already resident. However, once we account for the practical requirement to stage the library (\emph{search + $1\times$ write/load}), the GPU path enters the transient regime and the apparent advantage of the BIN kernel increases to $2.017\times$ energy efficiency and $2.866\times$ speedup, because a smaller representation reduces the amount of data that must traverse the external interface.

In contrast, SSD-scale ISP avoids the staging wall entirely by executing similarity in-place. Both 3D NAND and FeNAND sustain $20.844\times$ speedup in the \emph{search + $1\times$ write/load} metric and $8.092\times$ speedup in \emph{search-only}, indicating that performance is governed by internal die/plane/page-level parallelism rather than by host-device transfer. The energy advantage is even more pronounced: relative to H100 INT8, 3D NAND achieves $5.02\times 10^3\times$ energy efficiency (search + $1\times$ write/load), while FeNAND reaches $4.17\times 10^4\times$. These gains arise because only compact results traverse the host interface; the dominant energy is spent inside the storage package, amortized across massive internal parallelism.

Overall, Table~\ref{tab:hek-large} highlights the scaling inflection described in Section~\ref{sec:oms-scaling}: at terabyte-scale libraries, GPU execution becomes constrained by transient staging over external links, whereas storage-centric ISP remains in a persistent regime where the library is always resident and throughput scales with on-package concurrency. This gap explains why ISP architectures retain large speed and energy advantages exactly in the regime that motivates repository-scale OMS.


% ===================OLD TEXT for Improvement=================================
% \textcolor{red}{
% \subsection{Baseline and Metrics}
% We report results relative to two GPU baselines to reflect both conventional and HDC-style software stacks: the conventional baseline is \textit{ANN-SoLo (FP32)} on GPU and the HDC baseline is \textit{HOMS-TC (INT8)} on GPU. Unless otherwise noted, all normalizations use the ANN-SoLo (FP32) implementation measured on RTX~4090 as the reference; H100 and other platforms are obtained by bandwidth/compute scaling from this RTX~4090 baseline.
% %
% We measure end-to-end throughput (QPS) and per-query latency including on-device reduction and score egress. To remove redundancy and be explicit about normalization, we compute speedup by \emph{latency} normalization,
% \[
% \text{Speedup} \;=\; \frac{t_{\text{baseline}}}{t_{\text{device}}}
% \quad\text{(equivalently, } \text{QPS}_{\text{device}}/\text{QPS}_{\text{baseline}}\text{)},
% \]
% where \(t_{\text{baseline}}\) is the search latency of ANN-SoLo (FP32) on RTX~4090 and \(t_{\text{device}}\) is the search latency of the target platform. Energy per query includes in-media operations, peripheral activity, and host ingress/egress, and is reported as \textit{search-only} and \textit{search + one-time reference load} (amortized). For the latter, the one-time reference load is modeled as a sequential read from a WD\_BLACK SN8100 PCIe Gen5 NVMe SSD (8\,TB, 14.9\,GB/s). Normalized energy efficiency follows the same convention,
% \[
% \text{Energy efficiency} \;=\; \frac{(E/\text{query})_{\text{baseline}}}{(E/\text{query})_{\text{device}}}\,.
% \]
% For the iso-throughput comparison in Table~\ref{tab:syn-same-speed}, device counts are chosen to match the GPU throughput using the speedup coefficients from Table~\ref{tab:syn-entire}; energy efficiency is then computed at this matched operating point.
% %
% Accuracy on HEK is evaluated at a fixed FDR. We report total identifications relative to the GPU HDC baseline (HOMS-TC, INT8) and identification consistency via UpSet overlaps against a proxy consensus (ANN-SoLo $\cap$ HOMS-TC). Robustness of binary HDC to device non-idealities is probed by injecting a bit-error rate (BER) into the binary embeddings and tracking changes in totals (Fig.~\ref{fig:hyperoms-ber}) and overlaps (Fig.~\ref{fig:UPSET}) for BER $\in\{0,5,10,15\%\}$.
% %
% \subsection{Comparative Results}
% Tables~\ref{tab:hek}--\ref{tab:syn-same-speed} show the energy efficiency and speedup factors of each device compared to the baseline. Table~\ref{tab:hek} assumes the HEK library fits in a single chip/package for each device class and reports per-chip metrics with the library preloaded. Table~\ref{tab:syn-entire} reports results on the Synthetic dataset. For volatile-memory systems (GPUs, FPGAs, and DRAM-NMP), we report single-device performance with the library staged into device memory for the run; because the memory is volatile, the library must be (re)written whenever the device is reprovisioned. For non-volatile systems (ReRAM/PCM IMP and NAND/FeNAND ISP), the full library resides in-device by scaling the number of chips, reflecting their role as storage surrogates where the dataset persists across runs. Per-reference footprints for ANN-SoLo/INT8/BIN use the same FP32$\rightarrow$INT8$\rightarrow$BIN scaling factors as in HEK. Table~\ref{tab:syn-same-speed} then fixes throughput across platforms: for each device class, it selects the minimum number of devices needed to match the GPU throughput (iso-speed) and reports energy efficiency at that matched rate.
% %
% \subsubsection{Speedup}
% On the HEK single-chip setting (Table~\ref{tab:hek}), storage-centric in-storage processing (ISP) achieves the highest throughput, with 3D~NAND and FeNAND delivering roughly $390\times$ speedup over the RTX~4090 ANN-SoLo baseline. PCM~IMP follows at $\sim$240$\times$, ReRAM~IMP $\sim$78$\times$, DRAM~NMP $\sim$61$\times$, and the FPGA pipeline $\sim$98$\times$. DRAM~NMP exposes bank-level parallelism ($\sim$256 banks), but a VP1902-class FPGA instantiates many more bitwise lanes and wider streaming datapaths; this greater fine-grained concurrency explains the FPGA's larger speedup relative to DRAM~NMP. GPU-side HDC also scales favorably, reaching $\sim$24$\times$ (HOMS-TC) and $\sim$34$\times$ (HyperOMS) on RTX~4090, and up to $\sim$71$\times$ and $\sim$101$\times$ on H100.
% %
% For the synthetic dataset (Table~\ref{tab:syn-entire})--which uses a single device for volatile-memory systems and keeps the entire library resident in non-volatile systems--we observe a clear divergence between \emph{pure search} and \emph{search + load} scenarios. Among volatile systems, adding the one-time load phase causes a noticeable reduction in apparent speedup: on RTX~4090, HOMS-TC drops by $\sim$34\% and HyperOMS by $\sim$8\%; on H100, the loss is more pronounced, HOMS-TC $\sim$61\%, HyperOMS $\sim$21\%, and ANN-SoLo $\sim$2\%. Similar trends appear in near-memory designs: the FPGA pipeline falls by $\sim$48\% and DRAM~NMP by $\sim$11\%. In contrast, non-volatile architectures like ReRAM, PCM, and NAND/FeNAND ISP--show virtually no degradation ($\le 1\%$), as their reference libraries remain permanently programmed within the memory array and require no host transfers.
% %
% These results highlight that when data must be staged repeatedly from host memory, volatile systems become I/O-bound and their realized speedup collapses; in contrast, non-volatile, device-resident architectures maintain nearly constant performance since query traffic dominates rather than data movement.
% %
% \subsubsection{Energy Efficiency}
% For HEK (Table~\ref{tab:hek}), energy efficiency (\emph{search + load}) peaks with storage-/NVM-centric designs: FeNAND $\sim$6.58$\times 10^{5}$, PCM $\sim$2.57$\times 10^{5}$, ReRAM $\sim$1.12$\times 10^{5}$, and 3D~NAND $\sim$6.60$\times 10^{4}$, followed by DRAM~NMP $\sim$1.20$\times 10^{3}$ and FPGA $\sim$53.5. GPU-side HDC improves efficiency as well: on RTX~4090, HOMS-TC $\sim$9.7 and HyperOMS $\sim$18.8; on H100 these rise to $\sim$18.7--$36.2$. Including the one-time reference load preserves the ordering.
% %
% On the synthetic dataset under the methodology (single device for volatile systems; entire library resident for non-volatile systems), the same pattern holds when we account for \emph{search + load} energy (Table~\ref{tab:syn-entire}). FeNAND reaches $\sim$7.67$\times 10^{5}$, PCM $\sim$3.05$\times 10^{5}$, ReRAM $\sim$1.27$\times 10^{5}$, and 3D~NAND $\sim$9.25$\times 10^{4}$; DRAM~NMP is $\sim$1.09$\times 10^{3}$ and FPGA $\sim$53.2. GPU efficiencies range from $\sim$9.6 (RTX~4090 HOMS-TC) and $\sim$18.8 (RTX~4090 HyperOMS) to $\sim$18.4--$37.1$ on H100. Because the non-volatile designs keep the library resident, the one-time load is amortized, and their advantage remains three to six orders of magnitude over the FP32 GPU baseline. Under iso-speed (Table~\ref{tab:syn-same-speed}), the relative ordering is unchanged: at equal throughput, IMP/ISP designs remain two to six orders of magnitude more energy-efficient than the GPU baseline, while GPU HDC retains a consistent 1–2 orders of magnitude gain over ANN-SoLo.
% }
% ===================OLD TEXT for Improvement=================================


% We evaluate robustness along two complementary axes. First, we measure \emph{coverage} via total identifications at a fixed FDR (Fig.~\ref{fig:hyperoms-ber}). Across datasets b1906--b1931, HyperOMS-BIN tracks the INT8 baseline closely for BER $\le 10\%$. At 15\% BER, the reduction in total identifications remains modest and dataset dependent (approximately 9--14\%), indicating that discovery coverage degrades smoothly as the error rate increases. Second, because totals alone cannot determine whether the same peptides are recovered, we measure \emph{consistency} using UpSet overlaps (Fig.~\ref{fig:UPSET}), which quantify agreement in high-confidence identifications across BER settings. This distinction is important: totals summarize how much is reported, whereas overlaps test whether the reported set is stable under device noise.




% \paragraph{Discussion.}
% Results show that memory- and storage-centric accelerators deliver one to three orders of magnitude speedup over GPUs by reducing data movement. Non-volatile IMP (PCM/ReRAM) achieves the highest energy efficiency, leveraging MLC density and HDC’s noise tolerance. 3D NAND and FeNAND provide unmatched scalability; FeNAND further alleviates NAND’s sequential bottleneck with DBAM. GPUs remain effective for moderate-size libraries but require hundreds of devices for terabyte-scale OMS. These findings indicate that future OMS accelerators will likely combine GPU-class compute with memory-/storage-centric search primitives.



% \subsection{HEK293 Dataset and Evaluation Setup}
% We evaluate HEK293 tandem mass spectrometry data with 24 peak files and an average of 46{,}665 spectra per file. Queries use subsets b1906 to b1931. Each spectrum is embedded as an 8{,}192 dimensional vector. Searches are run against the MassIVE-KB human spectral library with 2{,}992{,}672 reference spectra. The original reference footprint is about 10\,GB; with a binary representation it is about 2.85\,GB (1 bit per element), and with INT8 it is about 22.83\,GB.

% We use a unified metric for both energy and latency: search plus a one time reference write (load). The one time write is appropriate because the library is static, and it is especially relevant for memory centric designs where per query search is extremely fast and the initial load can dominate amortized cost. We run on available mature hardware and treat those measurements as golden baselines for device and array level simulations. For fair cross platform comparisons, we scale these baselines to representative devices and technology nodes. On GPUs we run ANN-SoLo (shifted cosine or shifted dot product rescoring) and HyperOMS in binary and INT8 (HOMS-TC on tensor cores) on an RTX\,4090, then scale to an H100 target using normalized memory bandwidth and compute throughput or TOPs. For FPGA we use a near storage configuration on Samsung or Xilinx SmartSSD CSD (Kintex UltraScale+), then scale to a Versal Premium VP1902 device with attached DRAM. For ReRAM we run on a NeuRRAM chip and report two projections at 130\,nm and 40\,nm.



% \subsection{Synthetic TB-Scale Reference (SYN)}
% We construct a synthetic terabyte scale workload to study billion scale behavior. The dataset contains 15{,}000 queries and 1{,}000{,}000{,}000 references, each a binary 8{,}192 dimensional vector (about 1\,KiB per reference), for a total reference store of about 0.95\,TiB (about 1\,TB).

% During search, the full reference database resides in device local memory to exclude host or storage I/O. Concretely, RTX\,4090 uses on board GDDR6X (24\,GB, about 1\,TB/s), H100 uses HBM (80\,GB, about 3.35\,TB/s), and the FPGA path uses board DRAM on a VP1902 class design. Memory centric designs (DRAM NMP, ReRAM, PCM, 3D NAND, FeNAND) store references directly in the array.

% To hold about 1\,TB of references, we replicate devices according to capacity: about 43 RTX\,4090 GPUs, about 13 H100 GPUs, about 16 VP1902 boards with DRAM, about 16 DRAM NMP devices, and about 5 packages each for ReRAM, PCM, 3D NAND, and FeNAND. For memory centric devices we model a 64 bit interface at 200\,MHz with sequential readout of indices and similarity scores, broadcast queries to all devices, include peripheral overheads (sense paths, lightweight mixed signal, controller), and normalize technology nodes to representative processes (GPU 5\,nm, FPGA 7\,nm, DRAM 22\,nm, ReRAM 40 to 130\,nm, PCM 40\,nm, NAND or FeNAND 14\,nm arrays with 7\,nm CMOS periphery). We reuse the same methodology as above: RTX\,4090 measurements scaled to H100 using normalized memory bandwidth and compute throughput or TOPs, SmartSSD CSD scaled to VP1902 with DRAM, and NeuRRAM measurements with projections at 130\,nm and 40\,nm. We apply the same reporting convention of search plus one time reference write (load).





% \subsubsection{Accuracy Preservation}
% % - HDC-based methods achieve consistent results across devices


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1\columnwidth]{fig/final_identifications_comparison_ber_withdrops.pdf}
%   \caption{Impact of injected bit error rate (BER) on HyperOMS identifications for datasets b1906--b1931}
%   \label{fig:hyperoms-ber}
% \end{figure}


% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\textwidth]{fig/upset.pdf}%
%   \caption{Identification accuracy across BER levels (UpSet overlaps, b1906)}
%   \label{fig:UPSET}
% \end{figure*}


% Total identifications (Fig.\ref{fig:hyperoms-ber})  is a indicator of robustness and practical utility at fixed FDR. In our BER experiments, HyperOMS-BIN tracks the INT8 baseline closely at low BER ($\leq 10\%$), and the decline at $15\%$ BER is modest and dataset dependent (about $9$--$14\%$). These totals show that overall discovery coverage degrades gracefully as errors increase.

% At the same time, total identifications alone cannot determine whether the same peptides are being recovered. To assess correctness more directly, we analyze set overlaps with UpSet plots. The UpSet overlaps quantify agreement on high-confidence peptide identifications between HyperOMS and the INT8 reference across BER settings. In effect, totals summarize coverage, while UpSet overlaps provide an accuracy-oriented counterpart that tests the consistency of the recovered peptides.

% The injected BER models device-level bit errors observed in multi-level non-volatile memories operated at tight sensing margins. The chosen BER levels correspond to regimes reported for higher bits-per-cell operation, so the stress tests reflect realistic hardware conditions\cite{fan2024mlcrram,fan2024specpcm}. The measured resilience is consistent with hyperdimensional computing: binary encodings with Hamming-style similarity distribute information across many dimensions, so random bit flips tend to average out rather than cause catastrophic rank changes.

% To complement total identifications, we summarize identification consistency with UpSet plots (Fig.\ref{fig:UPSET}) for dataset b1906 across BER $\in \{0,5,10,15\%\}$. Because ground truth is not available for HEK293, we treat the consensus of ANN-SoLo and HOMS-TC (INT8) as a proxy reference and quantify HyperOMS recovery of that consensus. Here, \emph{recovery} is the size of the three-way intersection (ANN\_SoLo $\cap$ HyperOMS\_BIN $\cap$ HOMS-TC) divided by the sum of the two-way consensus (ANN\_SoLo $\cap$ HOMS-TC) and that three-way intersection. Using the verified counts, recovery is $96.78\%$ at $0\%$ BER, $95.73\%$ at $5\%$ BER, $94.47\%$ at $10\%$ BER, and $91.41\%$ at $15\%$ BER. The consensus remains close to the $0\%$ BER reference through $10\%$ BER and shrinks moderately at $15\%$ BER, with most differences concentrated near the reporting threshold rather than reflecting wholesale rank shifts. Taken together, the UpSet overlaps provide the accuracy-oriented counterpart to totals: they show that HyperOMS preserves the bulk of high-confidence identifications while degrading smoothly as BER increases, consistent with the robustness of HDC encodings and Hamming-style similarity.


% Taken together, the totals and the UpSet overlaps indicate that HyperOMS maintains substantial identification coverage and preserves a large fraction of high-confidence peptides under realistic device-level error, supporting its suitability for memory-centric deployments.











% \subsection{Comparative Results}
% Tables~\ref{tab:hek}--\ref{tab:syn-same-speed} show the energy efficiency and speedup factors of each device compared to the baseline. Table~\ref{tab:hek} assumes the HEK library fits in a single chip/package for each device class and reports per-chip metrics with the library preloaded. Table~\ref{tab:syn-entire} reports results on the Synthetic dataset. For volatile-memory systems (GPUs, FPGAs, and DRAM-NMP), we report single-device performance with the library staged into device memory for the run; because the memory is volatile, the library must be (re)written whenever the device is reprovisioned. For non-volatile systems (ReRAM/PCM IMP and NAND/FeNAND ISP), the full library resides in-device by scaling the number of chips, reflecting their role as storage surrogates where the dataset persists across runs. Per-reference footprints for ANN-SoLo/INT8/BIN use the same FP32$\rightarrow$INT8$\rightarrow$BIN scaling factors as in HEK. Table~\ref{tab:syn-same-speed} then fixes throughput across platforms: for each device class, it selects the minimum number of devices needed to match the GPU throughput (iso-speed) and reports energy efficiency at that matched rate.




% \subsubsection{Speedup}
% On the HEK single-chip setting (Table~\ref{tab:hek}), storage-centric in-storage processing (ISP) achieves the highest throughput, with 3D~NAND and FeNAND delivering roughly $390\times$ speedup over the RTX~4090 ANN-SoLo baseline. PCM~IMP follows at $\sim$240$\times$, ReRAM~IMP $\sim$78$\times$, DRAM~NMP $\sim$61$\times$, and the FPGA pipeline $\sim$98$\times$. DRAM~NMP exposes bank-level parallelism ($\sim$256 banks), but a VP1902-class FPGA instantiates many more bitwise lanes and wider streaming datapaths; this greater fine-grained concurrency explains the FPGA's larger speedup relative to DRAM~NMP. GPU-side HDC also scales favorably, reaching $\sim$24$\times$ (HOMS-TC) and $\sim$34$\times$ (HyperOMS) on RTX~4090, and up to $\sim$71$\times$ and $\sim$101$\times$ on H100.

% For the synthetic dataset (Table~\ref{tab:syn-entire})--which uses a single device for volatile-memory systems and keeps the entire library resident in non-volatile systems--we observe a clear divergence between \emph{pure search} and \emph{search + load} scenarios. Among volatile systems, adding the one-time load phase causes a noticeable reduction in apparent speedup: on RTX~4090, HOMS-TC drops by $\sim$34\% and HyperOMS by $\sim$8\%; on H100, the loss is more pronounced, HOMS-TC $\sim$61\%, HyperOMS $\sim$21\%, and ANN-SoLo $\sim$2\%. Similar trends appear in near-memory designs: the FPGA pipeline falls by $\sim$48\% and DRAM~NMP by $\sim$11\%. In contrast, non-volatile architectures like ReRAM, PCM, and NAND/FeNAND ISP--show virtually no degradation ($\le 1\%$), as their reference libraries remain permanently programmed within the memory array and require no host transfers.

% These results highlight that when data must be staged repeatedly from host memory, volatile systems become I/O-bound and their realized speedup collapses; in contrast, non-volatile, device-resident architectures maintain nearly constant performance since query traffic dominates rather than data movement.

% \subsubsection{Energy Efficiency}
% For HEK (Table~\ref{tab:hek}), energy efficiency (\emph{search + load}) peaks with storage-/NVM-centric designs: FeNAND $\sim$6.58$\times 10^{5}$, PCM $\sim$2.57$\times 10^{5}$, ReRAM $\sim$1.12$\times 10^{5}$, and 3D~NAND $\sim$6.60$\times 10^{4}$, followed by DRAM~NMP $\sim$1.20$\times 10^{3}$ and FPGA $\sim$53.5. GPU-side HDC improves efficiency as well: on RTX~4090, HOMS-TC $\sim$9.7 and HyperOMS $\sim$18.8; on H100 these rise to $\sim$18.7--$36.2$. Including the one-time reference load preserves the ordering.

% On the synthetic dataset under the methodology (single device for volatile systems; entire library resident for non-volatile systems), the same pattern holds when we account for \emph{search + load} energy (Table~\ref{tab:syn-entire}). FeNAND reaches $\sim$7.67$\times 10^{5}$, PCM $\sim$3.05$\times 10^{5}$, ReRAM $\sim$1.27$\times 10^{5}$, and 3D~NAND $\sim$9.25$\times 10^{4}$; DRAM~NMP is $\sim$1.09$\times 10^{3}$ and FPGA $\sim$53.2. GPU efficiencies range from $\sim$9.6 (RTX~4090 HOMS-TC) and $\sim$18.8 (RTX~4090 HyperOMS) to $\sim$18.4--$37.1$ on H100. Because the non-volatile designs keep the library resident, the one-time load is amortized, and their advantage remains three to six orders of magnitude over the FP32 GPU baseline. Under iso-speed (Table~\ref{tab:syn-same-speed}), the relative ordering is unchanged: at equal throughput, IMP/ISP designs remain two to six orders of magnitude more energy-efficient than the GPU baseline, while GPU HDC retains a consistent 1–2 orders of magnitude gain over ANN-SoLo.


==> BACKUP/BACKUP_JAN4_Discussion.tex <==
\section{Discussions}
\label{sec:discussion}


\sumukh{start with algorithmic comparison and BER}

\cesong{Mid scale vs.  Datacenter scale --> Which device has which bottleneck? }



This work uses OMS as a concrete, high-throughput similarity-search workload to expose broader architectural trade-offs in memory-centric acceleration. The results highlight three coupled dimensions that generalize beyond mass spectrometry: (i) \emph{kernel representation} (FP32 vs.\ INT8 vs.\ binary HD), (ii) \emph{robustness under device non-idealities} (BER and variability), and (iii) \emph{operating regime} (resident vs.\ transient staging) as the database scales.


\subsection{Representation and Robustness of Binary HDC Kernel}
A consistent message across Tables~\ref{tab:hek-managed}--\ref{tab:hek-large} is that the representation chosen for similarity scoring sets the ceiling for both performance and energy, and simultaneously determines whether the kernel can be instantiated on dense memory substrates. On GPUs, moving from FP32 ANN-SoLo to reduced-precision HDC mappings yields substantial gains in the mid-scale regime where the working set can be treated as resident: on H100, INT8 HOMS-TC and binary HyperOMS reach $71.0\times$ and $101.2\times$ speedup over the RTX~4090 FP32 baseline, respectively (Table~\ref{tab:hek-managed}). These improvements reflect not only reduced arithmetic cost, but also a shift toward primitives (XOR + popcount / bit-parallel accumulation) that align naturally with wide SIMD and tensor-style execution.

More importantly for memory-centric substrates, the binary HDC form makes a single similarity kernel (HyperOMS) portable across DRAM-NMP, emerging NVM IMP, and flash-based ISP without requiring in-array FP32/INT8 dot products, which are fundamentally mismatched to MLC sensing margins and device variability. However, this portability comes with an explicit accuracy--robustness trade-off that is central to deployment on multi-level NVMs (e.g., ReRAM, PCM, NAND), where tighter read margins and variability manifest as effective bit errors during readout and in-array operations~\cite{ielmini2018inmemory,sebastian2020memdevices,burr2010drift}. Our BER injection study shows that HyperOMS degrades smoothly under such perturbations: for HEK293, recovery relative to the ANN-SoLo$\cap$HOMS-TC proxy consensus remains $95.7\%$ at 5\% BER and $91.4\%$ at 15\% BER (Section~\ref{sec:acc_preservation}, Fig.~\ref{fig:hyperoms-ber}). This behavior is consistent with the distributed nature of HDC representations, where independent bit flips tend to average out rather than catastrophically reshuffle rankings~\cite{kanerva2009hdc,rahimi2016hdc}.

Practically, these results reframe reliability for memory-centric accelerators. Instead of demanding near-zero BER at the device level (often expensive under MLC operation), designers can allocate a system-level \emph{error budget} and combine algorithmic tolerance with lightweight mitigation where it is most cost-effective. This is especially relevant for read-dominant workloads like OMS, where the reference library is written (or programmed) once and then reused across many query batches: the one-time provisioning overhead can be amortized, while steady-state search benefits from operating at more aggressive sensing points.






\subsection{Mid-Scale Versus Datacenter-Scale Regimes: Bottlenecks by Memory Class}
Section~\ref{sec:oms-scaling} frames OMS execution in terms of two regimes: when the reference footprint is effectively resident, throughput reflects in-substrate execution efficiency; when it is not, throughput collapses toward the cost of repeatedly staging data across an external interface. Interpreting Tables~\ref{tab:hek-managed}--\ref{tab:hek-large} through this lens yields a memory-class view of \emph{which constraint dominates at what scale}, without tying conclusions to any single prototype.

\paragraph{On-package high-bandwidth volatile memory (HBM/GDDR).}
HBM/GDDR-equipped GPUs sit at the high-bandwidth, low-latency end of the spectrum, with mature compute stacks and strong reduced-precision support. In the mid-scale dataset regime, where the working set can be treated as resident, performance is set primarily by on-package bandwidth and execution efficiency of the chosen kernel; reduced-precision mappings therefore translate directly into higher throughput and better energy (Table~\ref{tab:hek-managed}). As the repository grows beyond accelerator memory, the dominant constraint shifts from on-package bandwidth to staging orchestration and external data movement. In this transient regime, representation size becomes a first-order design parameter because it directly determines how much data must cross the interface, which is why the benefit of binary over INT8 is more pronounced once the load term is included (Table~\ref{tab:hek-large}). Practically, this class is most compelling when the application can keep the hot set resident; otherwise, external bandwidth and staging overhead dominate end-to-end efficiency.

\paragraph{Near-memory processing (DRAM-NMP).}
DRAM-NMP moves the similarity primitive into a larger capacity tier and replaces repeated host--device movement with internal bank/subarray activity~\cite{kang2024dram}. In the mid-scale comparison under a unified HyperOMS kernel, DRAM-NMP delivers a substantial energy-efficiency improvement while maintaining throughput in the same order as a GPU baseline (Table~\ref{tab:hek-hyperoms-only}), indicating that the dominant savings arise from reduced movement and high internal concurrency rather than from higher compute intensity. The limiting factors for this class are DRAM timing (activate/precharge), achievable bank-level parallelism, and the efficiency of near-bank primitives and control. While capacity can be increased by provisioning more modules, scaling to multi-terabyte repositories at the memory tier quickly implies a large module count and system footprint; DRAM-NMP is therefore best positioned as a mid-scale or intermediate tier rather than the natural endpoint for repository-scale storage.

\paragraph{Emerging NVM IMP/CIM (ReRAM/PCM).}
ReRAM/PCM IMP/CIM keeps references in-place and evaluates similarity at the array- and periphery-level, which is why it delivers orders-of-magnitude energy gains in the mid-scale regime under a fixed binary HDC kernel (Table~\ref{tab:hek-hyperoms-only}). Because the reference library is provisioned once and reused across many searches, write/verify and drift-management overheads primarily affect deployment time and can be treated as an amortized provisioning cost rather than a steady-state term. For this class, the critical constraints are not external interfaces but device and periphery realities: variability and drift, sensing margins under multi-level operation, and the latency/energy overhead of drivers and readout (including mixed-signal components when used)~\cite{fan2024mlcrram,fan2024specpcm}. The BER tolerance established in Section~\ref{sec:acc_preservation} is therefore a deployment enabler, as it allows the architecture to trade sensing margin for throughput/energy within a controlled error budget. Scaling this class to terabytes, however, typically requires many chips and substantial periphery replication, which can erode density and system simplicity; this is why our datacenter-scale tier emphasizes storage-class ISP, where density scaling is structurally favorable.


\paragraph{Storage-class ISP (3D NAND/FeNAND).}
Flash-based ISP occupies the opposite corner from HBM/GDDR: extreme capacity and persistence, with slower individual accesses but massive internal die/plane/page-level parallelism. Its defining advantage is regime stability: the repository remains resident at the storage tier, so performance does not hinge on repeated staging once the dataset exceeds accelerator memory. This becomes decisive at terabyte scale. In Table~\ref{tab:hek-large}, ISP sustains large \emph{search+$1\times$ load} speedups and achieves $10^3$--$10^4\times$ energy-efficiency gains over the H100 INT8 baseline because only compact results traverse the host interface while the dominant work is amortized inside the package. For this class, throughput is governed by how effectively internal parallelism is exploited and how efficiently periphery and control translate array-level operations into end-to-end progress~\cite{hsu2025fenand}. As 3D integration continues to increase density, storage-class ISP becomes increasingly aligned with repository-scale deployments where the dataset naturally resides in persistent storage.





















==> BACKUP/BACKUP_OMS.tex <==
 

\section{Methodology  for Comparative Study}\label{sec:eval}

Given the wide variety of device characteristics, memory capacity, and operating mechanisms across accelerator platforms, it is crucial to establish a consistent and fair evaluation setup for the comparative study. This section outlines the methodology used to construct a fair evaluation framework across the datasets, algorithms, and hardware configurations.


\subsection{Algorithm and Workload Configuration}
\label{sec:algo-workload}

\mingu{\\- While GPU handles FP32 and INT, INP is hard to process in MLC limit. 
\\
- Often it is mapped on the more favorable form as introduced in background. (kernel simplification goes here, but without such name, just say HD)
\\
- We employ the workloads in Table I with 2 different scales, mid and large ($>$1TB). 
\\
- Table I shows  HOMS-TC (int), RapidOMS and ANN-SoLO (fp) used for GPU or FPGA, HyperOMS for IMC along with the dataset XXXX}

\sumukh{added}

Our comparative study covers both conventional FP32 OMS and HDC-based OMS across GPUs, near-storage FPGAs, and memory-centric accelerators. On commodity GPUs, we run ANN-SoLo, which performs FP32 shifted dot-product / cosine similarity using vector units, together with HOMS-TC (INT8 tensor-core) and HyperOMS (binary HDC). These devices can natively handle FP32 and INT8 arithmetic and therefore serve as the reference software-style OMS baselines.

In contrast, in-/near-memory computing on multi-level non-volatile memories (ReRAM, PCM, 3D NAND, FeNAND) is constrained by MLC sensing margins and device variability, so directly implementing high-precision FP32 or even INT8 dot products inside the arrays is impractical. For these substrates, OMS is mapped to the high-dimensional (HD) form introduced in Section~\ref{sec:hdc}, where spectra are encoded as binary hypervectors and similarity is evaluated using massively parallel in-array MVM operations or bitwise XOR+popcount primitives implemented near the memory-array periphery. HyperOMS in this HD form is used as the common OMS kernel for DRAM-NMP, ReRAM/PCM in-memory computing (IMP), and 3D NAND / FeNAND in-storage processing (ISP).

We employ two workload scales that are representative of today’s OMS deployments. The mid-scale configuration uses the HEK293 dataset: 24 peak files with an average of 46{,}665 spectra per file, each embedded as an 8{,}192-dimensional vector, searched against the MassIVE-KB human spectral library with \(N = 2{,}992{,}672\) references. The same library is encoded in three ways for the GPU baselines: \(m/z\)-intensity peaks for ANN-SoLo (about 10\,GB), INT8 HDC vectors for HOMS-TC (about 22.8\,GB), and binary HDC vectors for HyperOMS (about 2.85\,GB). These encodings exercise FP32, INT8, and binary similarity kernels while keeping the underlying OMS task fixed. To study the regime where the reference library no longer fits in a single accelerator, we construct a terabyte-scale binary HDC workload with 15{,}000 queries and \(N = 10^{9}\) references at 8{,}192 dimensions, corresponding to roughly 1\,TB of reference data in binary form and about 8\,TB if stored in INT8. This configuration places GPUs in the transient streaming regime, while ISP designs keep the library persistent within SSD-scale 3D NAND and FeNAND packages.

Table~\ref{tab:hw_summary} summarizes how these workloads are mapped to each hardware class. For GPUs and near-storage FPGAs, the table lists ANN-SoLo (FP32), HOMS-TC (INT8), and RapidOMS (binary HyperOMS) on the HEK workload, and extends HOMS-TC and HyperOMS to the 1\,TB configuration on H100. For memory-centric substrates (DRAM-NMP, ReRAM IMP, PCM IMP, and 3D NAND / FeNAND ISP), HyperOMS in HD form is used for the mid-scale HEK setting and, where capacity permits, the terabyte-scale workload. This setup pairs each device with a numerically appropriate similarity kernel while providing a consistent OMS workload across the comparative study.


\begin{table}[t]
\caption{OMS workloads and evaluated device--algorithm configurations. ``Mid-scale'' corresponds to the HEK293 workload; ``Terabyte-scale'' corresponds to the 1\,TB binary HDC workload with $N = 10^9$ references.}
\label{tab:hw_summary}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\columnwidth}{@{}l l l c c@{}}
\toprule
\textbf{Device / class} & \textbf{Algorithm} & \textbf{Representation} & \textbf{Mid-Scale} & \textbf{Terabyte-Scale} \\
\midrule
\multirow{3}{*}{GPU (RTX~4090)} &
ANN-SoLo   & FP32 cosine & $\checkmark$ & -- \\
& HOMS-TC  & INT8 HDC    & $\checkmark$ & -- \\
& HyperOMS & Binary HDC  & $\checkmark$ & -- \\
\midrule
\multirow{3}{*}{GPU (H100)} &
ANN-SoLo   & FP32 cosine & $\checkmark$ & -- \\
& HOMS-TC  & INT8 HDC    & $\checkmark$ & $\checkmark$ \\
& HyperOMS & Binary HDC  & $\checkmark$ & $\checkmark$ \\
\midrule
Near-storage FPGA          & HyperOMS & Binary HDC & $\checkmark$ & -- \\
DRAM-NMP                   & HyperOMS & Binary HDC & $\checkmark$ & -- \\
ReRAM IMP                  & HyperOMS & Binary HDC & $\checkmark$ & -- \\
PCM IMP                    & HyperOMS & Binary HDC & $\checkmark$ & -- \\
3D NAND ISP                & HyperOMS & Binary HDC & $\checkmark$ & $\checkmark$ \\
FeNAND ISP                 & HyperOMS & Binary HDC & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabularx}
\end{table}



To structure the comparative analysis across these heterogeneous substrates, we adopt a three-tier evaluation methodology that cleanly separates (i) baseline algorithmic efficiency on GPUs, (ii) substrate-dependent execution efficiency in the \emph{mid-scale deployment} regime, and (iii) system-level efficiency in the \emph{datacenter} regime at terabyte scale.

\paragraph{\textbf{Baseline Algorithmic Efficiency (Table~\ref{tab:hek-managed})}}
We first measure the impact of representation and arithmetic on commodity accelerators by comparing an FP32 baseline (ANN-SoLo) against INT8 HOMS-TC and binary HyperOMS on RTX~4090 and H100 GPUs under the HEK workload. This tier isolates the speedup and energy gains attributable to HD-based kernels and reduced precision, without changing where the data reside or how they are staged.

\paragraph{\textbf{Mid-Scale Substrate Analysis via Unified HDC Algorithm (Table~\ref{tab:hek-hyperoms-only})}}
Next, we fix the algorithm to HyperOMS (binary HDC, $b=1$) to enable an equitable comparison across memory technologies in the \emph{mid-scale deployment} regime. We compare commodity and near-data substrates---GPUs, near-storage FPGAs, DRAM-NMP~\cite{kang2024dram}, non-volatile IMP (ReRAM~\cite{fan2024mlcrram}, PCM~\cite{fan2024specpcm}), and capacity-normalized 3D NAND/FeNAND ISP tiles~\cite{hsu2023memsys,hsu2025fenand}---using identical per-package capacity and a common HEK workload. For each device, we report both ``search-only'' and ``search + load'' metrics to quantify the energy penalty of volatile architectures that must repeatedly stage reference data from host memory versus non-volatile substrates where the library is persistent in-place.

\paragraph{\textbf{Datacenter-Scale Scalability at the Terabyte Limit (Table~\ref{tab:hek-large})}}
Finally, we stress-test scalability by increasing the reference library to $N = 10^{9}$ ($\approx 1$\,TB for binary HDC) in a datacenter setting. For this regime, we restrict comparisons to NVIDIA H100 and full SSD-scale ISP architectures (3D NAND and FeNAND), which exploit die/plane-level parallelism for large-corpus OMS~\cite{hsu2023memsys,hsu2025fenand}. DRAM-NMP and ReRAM/PCM-IMP are excluded from this experiment because provisioning terabyte-scale capacity on these technologies implies an impractical device count and area footprint. This tier therefore focuses on the contrast between the transient regime (GPU streaming over PCIe/NVLink) and the persistent regime (in-place ISP execution), using the workload scales and mappings summarized in Table~\ref{tab:hw_summary}.


\subsection{OMS Workload Scaling and Data-Movement}
\label{sec:oms-scaling}

To compare heterogeneous substrates on equal footing, we use a simple OMS workload model that makes explicit when a configuration operates in a \emph{resident} regime versus a \emph{transient} staging regime, and how representation choices (FP32, INT8, binary) translate into library footprint and data movement. This model provides the common normalization basis for the comparative results reported in Section~\ref{sec:eval}. \mingu{this paragraph's language should be more clear.}\sumukh{simplified}

\begin{table}[h]
\caption{Notation for OMS computational model.\mingu{do we need all of them ? or, just abstract and explain in a text ?}\sumukh{reduced}}
\label{tab:oms-notation}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{@{}lX lX@{}}
\toprule
\textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
\midrule
$Q_b$ & Query batch set & $b$ & Precision (bits/element) \\
$C_q$ & Reference set for query $q$ & $N$ & Total reference count \\
$D$ & Vector dimensionality & $F$ & Per-reference footprint (B) \\
$S$ & Total library size ($N \cdot F$) & $C_{\mathrm{res}}$ & Resident capacity of device \\
\bottomrule
\end{tabularx}
\end{table}

Beyond the spectrum-encoding pipeline, OMS performance is shaped by how the workload scales with library size, representation precision, and device-resident capacity. Table~\ref{tab:oms-notation} summarizes the notation used in our model. For a query batch $Q_b$, the arithmetic work grows with the number of candidate comparisons, roughly as \(\sum_{q \in Q_b} |C_q| \cdot D\), where \(|C_q|\) is the candidate set size for query $q$ and $D$ is the embedding dimension. At repository scale, however, we often find that throughput is dominated by staging the reference library $\mathcal{L}$ into the execution units rather than by this raw compute.

References are stored in contiguous blocks (pages or erase blocks) to amortize I/O latency. We define the total library footprint as
\begin{equation}
    S = N \times F = N \times \left\lceil \frac{D \cdot b}{8} \right\rceil .
\end{equation}
This expression makes the effect of representation precision explicit: standard pipelines use FP32 ($b=32$), quantized GPU pipelines (e.g., HOMS-TC) use INT8 ($b=8$), and HyperOMS uses binary hypervectors ($b=1$). Because OMS typically operates under wide precursor tolerances, the candidate sets $C_q$ often span a large fraction of the library; in the limiting case, the staged footprint approaches a full linear scan over $S$.

The operating regime of each substrate is determined by how this footprint relates to the device’s resident capacity. Let $C_{\mathrm{res}}$ denote the resident capacity of the executing device (e.g., a GPU’s HBM/GDDR or a device-side DRAM buffer). When $S \le C_{\mathrm{res}}$, the library (or the hot working set) can be kept resident, and queries are served by reusing in-device data. When $S$ exceeds $C_{\mathrm{res}}$, the workload enters a \emph{transient staging regime}: reference blocks must be repeatedly streamed over an external interface with effective bandwidth \(\mathrm{BW}_{\mathrm{ext}}\) (e.g., PCIe/NVLink or a storage link), where \(\mathrm{BW}_{\mathrm{ext}}\) denotes the achievable external I/O bandwidth. Each pass over the staged working set then incurs \(\Theta(S / \mathrm{BW}_{\mathrm{ext}})\) worth of transfer time, which quickly dominates per-batch execution as $S$ grows. This model links $(b, D)$ and library size $N$ to staging cost via $S$, and provides the normalization basis used in our cross-platform speedup and energy-efficiency comparisons.










 


==> BACKUP/backup_omsmodel_jan10.tex <==



% \textcolor{red}{Below 2 sections are changed heavily}

\section{Methodology for Comparative Study}\label{sec:eval}

Given the wide variety of device characteristics, memory capacity, and operating mechanisms across various accelerator platforms, it is crucial to establish a consistent and fair evaluation setup for the comparative study. This section outlines the methodology used to construct a fair evaluation framework across the datasets, algorithms, and hardware configurations.


\subsection{Unified Algorithm and Workload Configuration}
\label{sec:algo-workload}

\mingu{\\- While GPU handles FP32 and INT, INP is hard to process in MLC limit. 
\\
- Often it is mapped on the more favorable form as introduced in background. (kernel simplification goes here, but without such name, just say HD)
\\
- We employ the workloads in Table I with 2 different scales, mid and large ($>$1TB). 
\\
- Table I shows  HOMS-TC (int), RapidOMS and ANN-SoLO (fp) used for GPU or FPGA, HyperOMS for IMC along with the dataset XXXX}

\sumukh{added}

% Our comparative study covers both conventional FP32 OMS and HDC-based OMS across GPUs, near-storage FPGAs, and memory-centric accelerators. On commodity GPUs, we run ANN-SoLo, which performs FP32 shifted dot-product / cosine similarity using vector units, together with HOMS-TC (INT8 HDC) and HyperOMS (binary HDC). These devices can natively handle FP32 and INT8/binary arithmetic and therefore serve as the reference software-style OMS baselines.

\cesong{Our study evaluates both conventional FP32 OMS and HDC-based OMS across GPUs, near-storage FPGAs, and memory-centric accelerators. On commodity GPUs, we consider ANN-SoLo, which performs FP32 shifted dot-product (cosine) similarity using vector units, together with HOMS-TC (INT8 HDC) and HyperOMS (binary HDC). Because GPUs natively support FP32, INT8, and binary arithmetic, these implementations serve as software-style OMS baselines.}

% In contrast, in-/near-memory processing on multi-level non-volatile memories (e.g., ReRAM, PCM, 3D NAND, and FeNAND) is constrained by MLC sensing margins and device variability, so directly implementing high-precision FP32 or even INT8 dot products inside the arrays is impractical. For these platforms, OMS is mapped to the high-dimensional form (e.g., HD) introduced in Section~\ref{sec:hdc}, where spectra are encoded as binary HVs and similarity is evaluated using massively parallel in-array MVM operations or bitwise XOR+popcount primitives implemented near the memory-array periphery. HyperOMS in this HD form is used as the common OMS kernel for DRAM-NMP, ReRAM/PCM IMP, and 3D NAND / FeNAND ISP.

\cesong{In contrast, in- and near-memory processing on multi-level non-volatile memories (e.g., ReRAM, PCM, 3D NAND, and FeNAND) is constrained by limited sensing margins and device variability under MLC operation, making high-precision FP32 or INT8 dot-products impractical inside the arrays. For these platforms, OMS is therefore mapped to the high-dimensional (e.g., HD) formulation introduced in Section~\ref{sec:hdc}, where spectra are encoded as binary HVs and similarity is evaluated using massively parallel in-array VMM operations or bitwise XOR+popcount primitives implemented near the memory periphery. We use HyperOMS in this binary HD form as the common OMS kernel for DRAM-NMP, ReRAM/PCM IMP, and 3D NAND/FeNAND ISP, enabling a numerically appropriate and portable mapping across memory-centric platforms.}

% We employ two workload scales that are representative of today’s OMS deployments. The mid-scale configuration uses the HEK293 dataset: 24 peak files with an average of 46{,}665 spectra per file, each embedded as an 8{,}192-dimensional vector, searched against the MassIVE-KB human spectral library with \(N = 2{,}992{,}672\) references. The same library is encoded in three ways for the GPU baselines: \(m/z\)-intensity peaks for ANN-SoLo (about 10\,GB), INT8 HDC vectors for HOMS-TC (about 22.8\,GB), and binary HDC vectors for HyperOMS (about 2.85\,GB). These encodings exercise FP32, INT8, and binary similarity kernels while keeping the underlying OMS task fixed. To study the regime where the reference library no longer fits in a single accelerator, we construct a terabyte-scale binary HDC workload with 15{,}000 queries and \(N = 10^{9}\) references at 8{,}192 dimensions, corresponding to roughly 1\,TB of reference data in binary form and about 8\,TB if stored in INT8. This configuration places GPUs in the transient streaming regime, while ISP designs keep the library persistent within SSD-scale 3D NAND and FeNAND packages.

\cesong{We evaluate two workload scales that reflect practical OMS deployments. The \emph{mid-scale} configuration targets a single-accelerator settingand uses the HEK293 dataset: 24 peak files with an average of 46{,}665 spectra per file, each embedded as an 8{,}192-dimensional vector, searched against the MassIVE-KB human spectral library with
\(N = 2{,}992{,}672\) references. The same library is encoded in three forms for GPU execution: \(m/z\)-intensity peaks for ANN-SoLo (about 10\,GB), INT8 HDC vectors for HOMS-TC (about 22.8\,GB), and binary HDC vectors for HyperOMS (about 2.85\,GB). To capture \emph{datacenter-scale} OMS, where the reference library exceeds the capacity of a single accelerator, we construct a terabyte-scale binary HDC workload with 15{,}000 queries and
\(N = 10^{9}\) references at 8{,}192 dimensions. This corresponds to approximately 1\,TB of reference data in binary form (and about 8\,TB in INT8), placing GPU-based execution in a transient streaming regime, while ISP designs retain the library persistently within SSD-scale 3D NAND and FeNAND packages.
Based on these two workload regimes, we organize the evaluation using a three-tier methodology that separates (i) baseline algorithmic efficiency on GPUs, (ii) platform-dependent execution efficiency in the \emph{mid-scale} deployment regime, and (iii) system-level scalability in the \emph{datacenter} regime at terabyte scale.}

\cesong{Table~\ref{tab:hw_summary} summarizes the mapping of workloads, algorithms, and evaluation tiers across hardware classes. The baseline algorithmic efficiency tier evaluates GPU-based execution to isolate the speedup and energy gains attributable to HD-based kernels and reduced precision, without altering data placement or staging behavior. The mid-scale platform analysis tier fixes the algorithm to binary HyperOMS and compares heterogeneous platforms under identical per-package capacity and a common HEK workload, reporting both ``search-only'' and ``search + load'' metrics to capture the energy penalty of repeated data staging in volatile architectures versus persistent in-place execution. Finally, the datacenter-scale scalability tier restricts evaluation to NVIDIA H100 and full SSD-scale ISP architectures (3D NAND and FeNAND), excluding DRAM-NMP and ReRAM/PCM-IMP due to impractical capacity scaling, and highlights the contrast between transient GPU streaming over PCIe/NVLink and persistent in-place ISP execution at terabyte scale.}

\begin{table}[t]
\caption{OMS workloads and evaluated device--algorithm configurations. ``Mid-scale'' corresponds to the HEK293 workload; ``Terabyte-scale'' corresponds to the 1\,TB binary HDC workload with $N = 10^9$ references.}
\label{tab:hw_summary}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\columnwidth}{@{}l l l c c@{}}
\toprule
\textbf{Device / class} & \textbf{Algorithm} & \textbf{Representation} & \textbf{Mid-Scale} & \textbf{Terabyte-Scale} \\
\midrule
\multirow{3}{*}{GPU (RTX~4090)} &
ANN-SoLo   & FP32 cosine & $\checkmark$ & -- \\
& HOMS-TC  & INT8 HDC    & $\checkmark$ & -- \\
& HyperOMS & Binary HDC  & $\checkmark$ & -- \\
\midrule
\multirow{3}{*}{GPU (H100)} &
ANN-SoLo   & FP32 cosine & $\checkmark$ & -- \\
& HOMS-TC  & INT8 HDC    & $\checkmark$ & $\checkmark$ \\
& HyperOMS & Binary HDC  & $\checkmark$ & $\checkmark$ \\
\midrule
Near-storage FPGA          & HyperOMS & Binary HDC & $\checkmark$ & -- \\
DRAM NMP                   & HyperOMS & Binary HDC & $\checkmark$ & -- \\
ReRAM IMP                  & HyperOMS & Binary HDC & $\checkmark$ & -- \\
PCM IMP                    & HyperOMS & Binary HDC & $\checkmark$ & -- \\
3D NAND ISP                & HyperOMS & Binary HDC & $\checkmark$ & $\checkmark$ \\
FeNAND ISP                 & HyperOMS & Binary HDC & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabularx}
\end{table}


% Table~\ref{tab:hw_summary} summarizes how these workloads are mapped to each hardware class. For GPUs and near-storage FPGAs, the table lists ANN-SoLo (FP32), HOMS-TC (INT8), and RapidOMS (binary HyperOMS) on the HEK workload, and extends HOMS-TC and HyperOMS to the 1\,TB configuration on H100. For memory-centric platforms (DRAM-NMP, ReRAM IMP, PCM IMP, and 3D NAND / FeNAND ISP), HyperOMS in HD form is used for the mid-scale HEK setting and, where capacity permits, the terabyte-scale workload. This setup pairs each device with a numerically appropriate similarity kernel while providing a consistent OMS workload across the comparative study.

\begin{table*}[t]
\centering
\caption{Workload and representation parameters used across OMS mappings. \cesong{We don't need this maybe?}}
\label{tab:params_workload}
\small
\begin{tabular}{l l l l l l}
\hline
\textbf{Item} & \textbf{Symbol} & \textbf{Value} & \textbf{Notes} \\
\hline
HV dimensionality & $D$ & 8,192 & OMS HDC setting used throughout \\
Query batch size & $B$ & \textcolor{red}{Fill} & Queries processed per launch/batch  \\
Similarity kernel & -- & FP32 cosine / INT8 dot / XOR+popcount & Per platform mapping  \\
Top-$k$ output & $k$ & \textcolor{red}{Fill} (e.g., 10/50/100) & Candidates passed to FDR stage \\
Data precision (query/ref) & -- & FP32 / INT8 / 1b / MLC-packed & Representation-dependent \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Platform-level parameters used for OMS mapping and modeling.}
\label{tab:params_platform}
\small
\begin{tabular}{l l l l l l l}
\hline
\textbf{Platform} & \textbf{Resident device} & \textbf{Capacity} & \textbf{Search primitive} & \textbf{Peri. circuitry} & \textbf{I/O / staging path} \\
\hline
GPU (RTX 4090) &
GDDR6X & 24\,GB &
CUDA/Tensor Cores &
-- &
Host$\rightarrow$GPU \\
GPU (H100) &
HBM3 & 80\,GB &
CUDA/Tensor Cores &
-- &
Host$\rightarrow$GPU \\
\hline
FPGA (VP1902)~\cite{pinge2024rapidoms} &
On-board DRAM &
\textcolor{red}{Fill} &
XOR + popcount &
-- &
NAND$\rightarrow$DRAM refill \\
\hline
DRAM NMP~\cite{kang2024dram} & 
DDR4 &
64~GB &
XOR + popcount &
-- &
Host$\rightarrow$DRAM provisioning\\
\hline
ReRAM IMP~\cite{fan2024mlcrram} &
In-array (MLC)&
3~GB &
Analog VMM + ADC &
7-b ADC &
Pre-programmed refs\\
PCM IMP~\cite{fan2024specpcm} &
In-array (MLC) &
3~GB &
Analog VMM + ADC &
6-b ADC; 3-b DAC&
Pre-programmed refs \\
\hline
Storage ISP~\cite{hsu2025fenand} &
In-storage arrays &
0.2~TB &
In-storage scoring &
-- &
Host/control link 64-bit @ 200\,MHz \\
\hline
\end{tabular}
\end{table*}







% To structure the comparative analysis across these heterogeneous platforms, we adopt a three-tier evaluation methodology that cleanly separates (i) baseline algorithmic efficiency on GPUs, (ii) platform-dependent execution efficiency in the \emph{mid-scale deployment} regime, and (iii) system-level efficiency in the \emph{datacenter} regime at terabyte scale.

% \paragraph{\textbf{Baseline Algorithmic Efficiency (Table~\ref{tab:hek-managed})}}
% We first measure the impact of representation and arithmetic on commodity accelerators by comparing an FP32 baseline (ANN-SoLo) against INT8 HOMS-TC and binary HyperOMS on RTX~4090 and H100 GPUs under the HEK workload. This tier isolates the speedup and energy gains attributable to HD-based kernels and reduced precision, without changing where the data reside or how they are staged.

% \paragraph{\textbf{Mid-Scale platform Analysis via Unified HDC Algorithm (Table~\ref{tab:hek-hyperoms-only})}}
% Next, we fix the algorithm to HyperOMS (binary HDC, $b=1$) to enable an equitable comparison across memory technologies in the \emph{mid-scale deployment} regime. We compare commodity and near-data platforms---GPUs, near-storage FPGAs, DRAM-NMP~\cite{kang2024dram}, non-volatile IMP (ReRAM~\cite{fan2024mlcrram}, PCM~\cite{fan2024specpcm}), and capacity-normalized 3D NAND/FeNAND ISP tiles~\cite{hsu2023memsys,hsu2025fenand}---using identical per-package capacity and a common HEK workload. For each device, we report both ``search-only'' and ``search + load'' metrics to quantify the energy penalty of volatile architectures that must repeatedly stage reference data from host memory versus non-volatile platforms where the library is persistent in-place.

% \paragraph{\textbf{Datacenter-Scale Scalability at the Terabyte Limit (Table~\ref{tab:hek-large})}}
% Finally, we stress-test scalability by increasing the reference library to $N = 10^{9}$ ($\approx 1$\,TB for binary HDC) in a datacenter setting. For this regime, we restrict comparisons to NVIDIA H100 and full SSD-scale ISP architectures (3D NAND and FeNAND), which exploit die/plane-level parallelism for large-corpus OMS~\cite{hsu2023memsys,hsu2025fenand}. DRAM-NMP and ReRAM/PCM-IMP are excluded from this experiment because provisioning terabyte-scale capacity on these technologies implies an impractical device count and area footprint. This tier therefore focuses on the contrast between the transient regime (GPU streaming over PCIe/NVLink) and the persistent regime (in-place ISP execution), using the workload scales and mappings summarized in Table~\ref{tab:hw_summary}.


\subsection{OMS Workload Scaling and Data-Movement}
\label{sec:oms-scaling}

To compare heterogeneous platforms on equal footing, we use a simple OMS workload model that makes explicit when a configuration operates in a \emph{resident} regime versus a \emph{transient} staging regime, and how representation choices (FP32, INT8, binary) translate into library footprint and data movement. This model provides the common normalization basis for the comparative results reported in Section~\ref{sec:eval}. \mingu{this paragraph's language should be more clear.}\sumukh{simplified}

\begin{table}[h]
\caption{Notation for OMS computational model.\mingu{do we need all of them ? or, just abstract and explain in a text ?}\sumukh{reduced}}
\label{tab:oms-notation}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{@{}lX lX@{}}
\toprule
\textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
\midrule
$Q_b$ & Query batch set & $b$ & Precision (bits/element) \\
$C_q$ & Reference set for query $q$ & $N$ & Total reference count \\
$D$ & Vector dimensionality & $F$ & Per-reference footprint (B) \\
$S$ & Total library size ($N \cdot F$) & $C_{\mathrm{res}}$ & Resident capacity of device \\
\bottomrule
\end{tabularx}
\end{table}

Beyond the spectrum-encoding pipeline, OMS performance is shaped by how the workload scales with library size, representation precision, and device-resident capacity. Table~\ref{tab:oms-notation} summarizes the notation used in our model. For a query batch $Q_b$, the arithmetic work grows with the number of candidate comparisons, roughly as \(\sum_{q \in Q_b} |C_q| \cdot D\), where \(|C_q|\) is the candidate set size for query $q$ and $D$ is the embedding dimension. At repository scale, however, we often find that throughput is dominated by staging the reference library $\mathcal{L}$ into the execution units rather than by this raw compute.

References are stored in contiguous blocks (pages or erase blocks) to amortize I/O latency. We define the total library footprint as
\begin{equation}
    S = N \times F = N \times \left\lceil \frac{D \cdot b}{8} \right\rceil .
\end{equation}
This expression makes the effect of representation precision explicit: standard pipelines use FP32 ($b=32$), quantized GPU pipelines (e.g., HOMS-TC) use INT8 ($b=8$), and HyperOMS uses binary HVs ($b=1$). Because OMS typically operates under wide precursor tolerances, the candidate sets $C_q$ often span a large fraction of the library; in the limiting case, the staged footprint approaches a full linear scan over $S$.

The operating regime of each platform is determined by how this footprint relates to the device’s resident capacity. Let $C_{\mathrm{res}}$ denote the resident capacity of the executing device (e.g., a GPU’s HBM/GDDR or a device-side DRAM buffer). When $S \le C_{\mathrm{res}}$, the library (or the hot working set) can be kept resident, and queries are served by reusing in-device data. When $S$ exceeds $C_{\mathrm{res}}$, the workload enters a \emph{transient staging regime}: reference blocks must be repeatedly streamed over an external interface with effective bandwidth \(\mathrm{BW}_{\mathrm{ext}}\) (e.g., PCIe/NVLink or a storage link), where \(\mathrm{BW}_{\mathrm{ext}}\) denotes the achievable external I/O bandwidth. Each pass over the staged working set then incurs \(\Theta(S / \mathrm{BW}_{\mathrm{ext}})\) worth of transfer time, which quickly dominates per-batch execution as $S$ grows. This model links $(b, D)$ and library size $N$ to staging cost via $S$, and provides the normalization basis used in our cross-platform speedup and energy-efficiency comparisons.















% \subsection{OMS Workload Scaling and Data-Movement}
% \label{sec:oms-scaling}

% To support a structured evaluation across platforms, we now formalize the workload-scaling and data-movement model used throughout Section~\ref{sec:eval}. The goal is to make explicit when OMS operates in a resident regime versus a transient staging regime, and to define a consistent normalization basis for cross-platform comparisons.\mingu{this paragraph's language should be more clear.}

% \subsubsection{OMS Computational Model and Staging Constraints}\label{sec:oms-model}

% \begin{table}[h]
% \caption{Notation for OMS Computational Model \mingu{do we need all of them ? or, just abstract and explain in a text ?}}
% \label{tab:oms-notation}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabularx}{\columnwidth}{@{}lX lX@{}}
% \toprule
% \textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
% \midrule
% $Q_b$ & Query batch set & $b$ & Precision (bits/element) \\
% $q$ & Single query ($q \in Q_b$) & $N$ & Total reference count \\
% $C_q$ & Candidate reference set & $F$ & Per-reference footprint (B) \\
% $D$ & Vector dimensionality & $S$ & Total Library Size ($N \cdot F$) \\
% $W_{\mathrm{calc}}$ & Arithmetic Workload & $P$ & Device packages required \\
% $C_{\mathrm{res}}$ & Resident capacity of executing device & $C_{\mathrm{dev}}$ & Usable capacity per persistent device/package \\
% $\mathrm{BW}_{\mathrm{ext}}$ & External I/O bandwidth &  &  \\
% \bottomrule
% \end{tabularx}
% \end{table}




% \cesong{Beyond the spectrum-encoding pipeline, OMS performance is fundamentally shaped by how the workload scales with library size, representation precision, and device-resident capacity. 
% To clarify these effects, we summarize the dominant factors governing data movement and throughput.}
% Table~\ref{tab:oms-notation} defines the core notation for the OMS workload. For a query batch $Q_b$, the arithmetic work scales as $W_{\mathrm{calc}} = \sum_{q \in Q_b} |C_q| \cdot D$. At repository scale, however, throughput is often dominated by the cost of staging the reference library $\mathcal{L}$ into the execution units rather than by the raw compute required for scoring.

% References are stored in contiguous blocks (pages or erase blocks) to amortize I/O latency. We define the total library size (footprint) as
% \begin{equation}
%     S = N \times F = N \times \left\lceil \frac{D \cdot b}{8} \right\rceil .
% \end{equation}
% This exposes the direct impact of representation precision: standard pipelines typically use FP32 ($b=32$), quantized approaches (e.g., HOMS-TC) use INT8 ($b=8$), and HyperOMS uses binary representations ($b=1$). Unlike targeted search, OMS often operates under wide precursor tolerances, so the candidate sets $C_q$ can span a substantial fraction of the library; in the worst case, the staged footprint approaches a full linear scan.

% The system's operating regime is determined by whether the staged working set fits within the resident capacity of the executing device. Let $C_{\mathrm{res}}$ denote the resident capacity (e.g., a GPU's HBM/GDDR or a device-side buffer), and let $C_{\mathrm{dev}}$ denote the usable capacity of a provisioned persistent platform (e.g., DIMM/SSD package or a capacity-normalized tile budget). If we provision a persistent platform to store the entire library in-place, the minimum number of device packages is $P = \left\lceil S / C_{\mathrm{dev}} \right\rceil$. In contrast, commodity accelerators typically execute with a limited resident working set. When the staged footprint $S$ exceeds $C_{\mathrm{res}}$, the workload enters a \textit{transient staging regime}: reference blocks must be repeatedly streamed over the external interface, and throughput becomes bounded by the effective external bandwidth $\mathrm{BW}_{\mathrm{ext}}$ (e.g., PCIe/NVLink or a storage link) rather than by on-device compute. In this regime, each pass over the staged working set incurs $\Theta(S / \mathrm{BW}_{\mathrm{ext}})$ data movement, which quickly dominates per-batch execution time as $S$ scales. This model links representation choices $(b, D)$ to staging cost via $S$, and we use it as the normalization basis for cross-platform evaluation.



==> TEX/Evaluation_Backup.tex <==
\section{Evaluation}\label{sec:eval}

% ======= TABLE 1 (5 columns): Hardware/Modeling Summary =======
\begin{table*}[t]
  \centering
  \caption{Hardware configurations, per-chip capacity, search primitives, and primary sources. References reside in-device for IMP/ISP designs.}
  \label{tab:hw_summary}
  \adjustbox{max width=\textwidth}{
  \begin{tabularx}{\textwidth}{l l l l l}
    \toprule
    \textbf{Accelerator} & \textbf{Device} & \textbf{Capacity / Chip} & \textbf{Search Primitive} & \textbf{Source} \\
    \midrule
    GPU & RTX~4090 & 24\,GB (GDDR6X) & ANN-SoLo (FP32); HOMS-TC (INT8); HyperOMS (BIN) & \cite{bittremieux2019extremely,kang2023homstc,kang2022massively} \\
    GPU & H100 & 80\,GB (HBM2E) & same kernels (scaled from RTX~4090) & - \\
    FPGA & Versal VP1902 & 64\,GB (DDR4-2400) & XOR+popcount pipeline (RapidOMS) & \cite{pinge2024rapidoms} \\
    DRAM NMP & DDR4 DIMM (NMP) & 64\,GB (DDR4-2400) & row-parallel XOR+popcount; on-DIMM reduce & \cite{kim2013memory,kang2024dram} \\
    ReRAM IMP & 40\,nm arrays + periph. & 0.2\,TB/chip & BIN HDC match; TLC (no verify); periph.\ scaled & \cite{fan2024mlcrram,chen2016design} \\
    PCM IMP & 40\,nm arrays + periph. & 0.2\,TB/chip & BIN/MLC packing (HDC); TLC (no verify); periph.\ scaled & \cite{fan2024specpcm} \\
    3D NAND ISP & 14\,nm arrays + 7\,nm CMOS & 0.2\,TB/chip & in-storage bitwise ops; block-level reduce & \cite{hsu2025fenand} \\
    3D FeNAND ISP & 14\,nm arrays + 7\,nm CMOS & 0.2\,TB/chip & \textcolor{red}{multi-WL activation; ISP reduction} & \cite{hsu2023memsys} \\
    \bottomrule
  \end{tabularx}}
\end{table*}



% ======= TABLE 2: Datasets =======
\begin{table}[t]
  \centering
  \caption{Datasets used in evaluation. Binary HDC embeddings use 8{,}192 dimensions unless noted.}
  \label{tab:datasets}
  \begin{tabular}{l r r l}
    \toprule
    \textbf{Dataset} & \textbf{\#Queries} & \textbf{\#References} & \textbf{Notes} \\
    \midrule
    HEK293 & 46{,}665 & 2{,}992{,}672 & 24 peak files; MassIVE-KB library \\
    Synthetic & 15{,}000 & 1{,}000{,}000{,}000 & $\sim$1\,TB binary store (8{,}192-D) \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Experimental Setup}

We evaluate OMS accelerators under a common methodology that holds constant the placement of the reference library and the host–device I/O path for queries and results. For GPUs, we measure throughput and energy on an NVIDIA RTX~4090 (GDDR6X, 24\,GB, $\sim$1\,TB/s) using three kernels—\textit{ANN-SoLo} (FP32 cosine), \textit{HOMS-TC} (HDC on INT8 tensor cores), and \textit{HyperOMS} (HDC with binary encodings)—and scale these measurements to an NVIDIA H100 (HBM2E, 80\,GB, $\sim$3.35\,TB/s) using bandwidth/compute normalization (memory bandwidth and effective TOPS). For the FPGA path, we use a near-storage configuration on a Samsung/Xilinx SmartSSD CSD (Kintex UltraScale+) to anchor search latency and power, and then scale to a Xilinx Versal VP1902 attached to a 64\,GB DDR4-2400 RDIMM (effective $\sim$19.2\,GB/s). For DRAM NMP, we assume the same DDR4 module and model near-memory primitives; write energy follows Kim~et~al.~\cite{kim2013memory}, while peripheral behavior and search latency follow Kang~et~al.~\cite{kang2024dram}. Although prior DRAM-NMP results assume 8\,GB DIMMs, we scale capacities and controller timing to 64\,GB for fair comparison.

For ReRAM and PCM IMP designs, we adopt an in-array storage scenario in which the full reference library resides in the device, modeling 0.2\,TB per chip. This capacity reflects a conservative, near-future target comparable to modern high-density NAND packages and is plausible for 3D-integrated ReRAM/PCM with MLC/TLC operation. ReRAM OMS follows \cite{fan2024mlcrram}; write energy is taken from Chen~et~al.~\cite{chen2016design}, and search latency as well as read/write energy are grounded in 40\,nm fabricated prototypes. For PCM, we use \textit{SpecPCM}~\cite{fan2024specpcm} for write energy and bandwidth; the peripheral circuitry (drivers, sense/readout, and control at 500~MHz, assuming single-wordline activation per cycle) is scaled to a 0.2\,TB target and, for parity, the same peripheral methodology is applied to ReRAM. We choose the Sb$_2$Te$_3$/Ge$_4$Sb$_6$Te$_7$ PCM case fabricated at 40\,nm in \cite{fan2024specpcm}. Both ReRAM and PCM are modeled as TLC (3\,bits/cell) with default \emph{no write-verify}. Because the reference library is written once and reused across searches, we ignore verify overhead in the mainline results and report both \emph{search-only} and \emph{search + one-time reference load}.

For 3D NAND and FeNAND ISP designs, we adopt device parameters, latency/energy models, and the ISP flow from Hsu~et~al.~\cite{hsu2025fenand}. Across all memory/storage-centric devices (DRAM NMP, ReRAM, PCM, 3D NAND, FeNAND), references are stored directly in the array, queries are broadcast to all devices, and indices/similarity scores are read out sequentially. Unless noted otherwise, we assume a 64-bit, 200\,MHz host/control interface,
matching conservative clocking and AXI-class widths in 7\,nm periphery, sufficient for query broadcast and top-$k$ egress. We include peripheral overheads (sense paths, lightweight mixed-signal where applicable, and controller logic) in both latency and energy, and normalize technology nodes to representative processes: GPU 5\,nm, FPGA 7\,nm, DRAM 22–28\,nm, ReRAM 40\,nm, PCM 40\,nm, and NAND/FeNAND with 14\,nm arrays and 7\,nm CMOS periphery. We treat mature hardware measurements as golden baselines for device/array-level simulations and use a unified reporting convention of \emph{search-only} versus \emph{search + one-time reference load.} \sumukh{Given that the reference library is written once and then read repeatedly, we ignore write-verify overhead in the main results}.

\subsection{Datasets}
For the \textbf{HEK293} (HEK) setting (Table~\ref{tab:datasets}), we evaluate 24 peak files with an average of 46{,}665 spectra (queries) per file, using subsets b1906–b1931. Each spectrum is embedded as an 8{,}192-dimensional vector. Searches are run against the MassIVE-KB human spectral library with 2{,}992{,}672 reference spectra. The original floating-point footprint is $\sim$10\,GB under the ANN-SoLo representation, which ranks candidates using the shifted dot product (often referred to as shifted cosine in subsequent accelerator papers) with spectrum normalization and sparse peak encoding (m/z–intensity pairs); using INT8 it is $\sim$22.83\,GB, and using a binary HDC representation (1 bit/element) it is $\sim$2.85\,GB.

For the \textbf{Synthetic} setting, we construct a terabyte-scale workload to study billion-scale behavior: 15{,}000 queries and 1{,}000{,}000{,}000 binary references (8{,}192-D), totaling $\sim$0.95\,TiB ($\sim$1\,TB). During search, the full reference database resides in device-local memory to exclude host/storage I/O. Concretely, the RTX~4090 uses on-board GDDR6X (24\,GB, $\sim$1\,TB/s), the H100 uses HBM2E (80\,GB, $\sim$3.35\,TB/s), and the FPGA path uses board DRAM on a VP1902-class design. Memory-centric devices store references directly in the array. To hold $\sim$1\,TB of references, we replicate devices by capacity: $\sim$43$\times$ RTX~4090, $\sim$13$\times$ H100, $\sim$16$\times$ VP1902 (with DRAM), $\sim$16$\times$ DRAM-NMP devices, and $\sim$5 chips each for ReRAM, PCM, 3D NAND, and FeNAND (assuming 0.2\,TB/chip for NVM/ISP). We reuse the same normalization and scaling methodology as above, including the \emph{search + one-time reference load} reporting convention.

\subsection{Baseline and Metrics}
We report results relative to two GPU baselines to reflect both conventional and HDC-style software stacks: the conventional baseline is \textit{ANN-SoLo (FP32)} on GPU and the HDC baseline is \textit{HOMS-TC (INT8)} on GPU. Unless otherwise noted, all normalizations use the ANN-SoLo (FP32) implementation measured on RTX~4090 as the reference; H100 and other platforms are obtained by bandwidth/compute scaling from this RTX~4090 baseline.

We measure end-to-end throughput (QPS) and per-query latency including on-device reduction and score egress. To remove redundancy and be explicit about normalization, we compute speedup by \emph{latency} normalization,
\[
\text{Speedup} \;=\; \frac{t_{\text{baseline}}}{t_{\text{device}}}
\quad\text{(equivalently, } \text{QPS}_{\text{device}}/\text{QPS}_{\text{baseline}}\text{)},
\]
where \(t_{\text{baseline}}\) is the search latency of ANN-SoLo (FP32) on RTX~4090 and \(t_{\text{device}}\) is the search latency of the target platform. Energy per query includes in-media operations, peripheral activity, and host ingress/egress, and is reported as \textit{search-only} and \textit{search + one-time reference load} (amortized). Normalized energy efficiency follows the same convention,
\[
\text{Energy efficiency} \;=\; \frac{(E/\text{query})_{\text{baseline}}}{(E/\text{query})_{\text{device}}}\,.
\]
For the iso-throughput comparison in Table~\ref{tab:syn-same-speed}, device counts are chosen to match the GPU throughput using the speedup coefficients from Table~\ref{tab:syn-entire}; energy efficiency is then computed at this matched operating point.

Accuracy on HEK is evaluated at a fixed FDR. We report total identifications relative to the GPU HDC baseline (HOMS-TC, INT8) and identification consistency via UpSet overlaps against a proxy consensus (ANN-SoLo $\cap$ HOMS-TC). Robustness of binary HDC to device non-idealities is probed by injecting a bit-error rate (BER) into the binary embeddings and tracking changes in totals (Fig.~\ref{fig:hyperoms-ber}) and overlaps (Fig.~\ref{fig:UPSET}) for BER $\in\{0,5,10,15\%\}$.



% --- table helpers (ensure these are in preamble if not already) ---
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\definecolor{resultpurple}{HTML}{7B1FA2}
%\newcommand{\result}[1]{\textcolor{black}{\bfseries #1}}
\setlength{\tabcolsep}{4pt}
\renewcommand\theadfont{\normalsize\bfseries}

% ================== TABLE 3: HEK DATASET ==================
\begin{table*}[t]
  \centering
  \caption{HEK dataset: normalized energy efficiency and speedup across platforms.}
  % ---------- GPU PART ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{GPU}}
    \label{tab:hek}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
      Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
      Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
      \midrule
      Energy efficiency (search) &
      \result{1.000} & \result{9.696} & \result{18.814} &
      \result{1.926} & \result{18.714} & \result{36.246} \\
      Energy efficiency (search + load) &
      \result{1.0} & \result{9.7} & \result{18.8} &
      \result{1.9} & \result{18.7} & \result{36.2} \\
      Speedup &
      \result{1.000} & \result{23.661} & \result{33.769} &
      \result{2.996} & \result{70.897} & \result{101.166} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}

  \vspace{0.6em}

  % ---------- OTHERS ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{FPGA / NMP / IMP / ISP}}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
      Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
      Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
      Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
      \midrule
      Energy efficiency (search) &
      \result{53.454} & \result{1,233.125} & \result{126,792.305} &
      \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\
      Energy efficiency (search + load) &
      \result{53.5} & \result{1,201.9} & \result{112,190.8} &
      \result{257,166.2} & \result{66,041.6} & \result{657,605.8} \\
      Speedup &
      \result{98.375} & \result{60.912} & \result{77.962} &
      \result{239.541} & \result{389.675} & \result{389.675} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}
\end{table*}




% ============== TABLE 4.1: SYNTHETIC - ENTIRE DATASET ==============
\begin{table*}[t]
  \centering
  \caption{Synthetic dataset (single device for volatile-memory systems; entire library stored in non-volatile memory systems).}
  % ---------- GPU PART ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{GPU}}
    \label{tab:syn-entire}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
      Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
      Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
      Capacity/Chip & {24\,GB} & {24\,GB} & {24\,GB} & {80\,GB} & {80\,GB} & {80\,GB} \\
      Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {3.17\,TB} & {8\,TB} & {1\,TB} \\
      Number of Devices (GPUs) & {136.0} & {342.0} & {43.0} & {41.0} & {103.0} & {13.0} \\
      \midrule
      Energy efficiency (search) &
      \result{1.000} & \result{9.696} & \result{18.814} &
      \result{1.926} & \result{18.714} & \result{36.246} \\
      Energy efficiency (search + load) &
      \result{1.0} & \result{9.7} & \result{18.8} &
      \result{1.9} & \result{18.7} & \result{36.2} \\
      Speedup &
      \result{1.000} & \result{59.201} & \result{10.668} &
      \result{0.903} & \result{53.453} & \result{9.663} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}

  \vspace{0.6em}

  % ---------- OTHERS ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{FPGA / NMP / IMP / ISP}}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
      Process/Device & {VP1902} & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
      Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
      Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
      Capacity/Chip & {64\,GB} & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\
      Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\
      Number of Devices & {16.0} & {16.0} & {5.0} & {5.0} & {5.0} & {5.0} \\
      \midrule
      Energy efficiency (search) &
      \result{53.454} & \result{1,233.125} & \result{126,792.305} &
      \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\
      Energy efficiency (search + load) &
      \result{53.5} & \result{1,140.9} & \result{90,250.5} &
      \result{193,578.7} & \result{41,210.4} & \result{505,854.2} \\
      Speedup &
      \result{10.164} & \result{6.600} & \result{2.388} &
      \result{3.359} & \result{8.169} & \result{8.169} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}
\end{table*}











% ============== TABLE 5: SYNTHETIC - SAME SPEED ==============
\begin{table*}[t]
  \centering
  \caption{Synthetic dataset (device counts chosen to match GPU throughput; ``same speed'').}
  % ---------- GPU PART ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{GPU}}
    \label{tab:syn-same-speed}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Device & {RTX 4090} & {RTX 4090} & {RTX 4090} & {H100} & {H100} & {H100} \\
      Algorithm & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} & {ANN-SoLo} & {HOMS-TC} & {HyperOMS} \\
      Data Type & {FP32} & {INT8} & {BIN} & {FP32} & {INT8} & {BIN} \\
      Capacity/Chip & {24\,GB} & {24\,GB} & {24\,GB} & {80\,GB} & {80\,GB} & {80\,GB} \\
      Library size (by data type) & {3.17\,TB} & {8\,TB} & {1\,TB} & {3.17\,TB} & {8\,TB} & {1\,TB} \\
      Devices used (GPUs) & {136.0} & {6.0} & {5.0} & {46.0} & {2.0} & {2.0} \\
      \midrule
      Energy efficiency (search) &
      \result{1.000} & \result{9.696} & \result{18.814} &
      \result{1.926} & \result{18.714} & \result{36.246} \\
      Energy efficiency (search + load) &
      \result{1.0} & \result{9.7} & \result{18.8} &
      \result{1.9} & \result{18.7} & \result{36.2} \\
      Speedup & \result{1.0} & \result{1.0} & \result{1.0} &
      \result{1.0} & \result{1.0} & \result{1.0} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}

  \vspace{0.6em}

  % ---------- OTHERS ----------
  \begin{subtable}{\textwidth}
    \caption*{\textbf{FPGA / NMP / IMP / ISP}}
    \adjustbox{max width=\textwidth}{
    \begin{tabularx}{\textwidth}{l *{6}{Y}}
      \toprule
      Memory Type & {FPGA} & {DRAM} & {ReRAM} & {PCM} & {3D NAND} & {FeNAND} \\
      Process/Device & {VP1902 } & {DDR4} & {TSMC 40nm} & {TSMC 40nm} & {TSMC 14nm} & {TSMC 14nm} \\
      Searching Type & {Digital} & {NMP} & {IMP} & {IMP} & {ISP} & {ISP} \\
      Data Type & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} & {BIN} \\
      Capacity/Chip & {64\,GB} & {64\,GB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} & {0.2\,TB} \\
      Library size (by data type) & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} & {1\,TB} \\
      Devices used & {2.0} & {3.0} & {5.0} & {3.0} & {2.0} & {1.0} \\
      \midrule
      Energy efficiency (search) &
      \result{53.454} & \result{1,233.125} & \result{126,792.305} &
      \result{304,557.047} & \result{92,421.589} & \result{766,537.162} \\
      Energy efficiency (search + load) &
      \result{53.5} & \result{1,214.7} & \result{102,010.3} &
      \result{247,744.4} & \result{74,024.0} & \result{694,914.8} \\
      Speedup & \result{1.0} & \result{1.0} & \result{1.0} &
      \result{1.0} & \result{1.0} & \result{1.0} \\
      \bottomrule
    \end{tabularx}}
  \end{subtable}
\end{table*}




\subsection{Comparative Results}
Tables~\ref{tab:hek}–\ref{tab:syn-same-speed} show the energy efficiency and speedup factors of each device compared to the baseline. Table~\ref{tab:hek} assumes the HEK library fits in a single chip/package for each device class and reports per-chip metrics with the library preloaded. Table~\ref{tab:syn-entire} sizes device counts to hold the entire synthetic library at once; for GPUs, per-reference footprints for ANN-SoLo/INT8/BIN apply the same FP32$\rightarrow$INT8$\rightarrow$BIN scaling factors as in HEK before choosing chip counts so that all references reside in device-local memory. Table~\ref{tab:syn-same-speed} then fixes throughput across platforms: using the speedup factors from Table~\ref{tab:syn-entire}, it selects the minimum device counts per class that match the GPU throughput (iso-speed) and compares energy efficiency at equal speed.



\subsubsection{Speedup}
On the HEK single-chip setting (Table~\ref{tab:hek}), storage-centric ISP delivers the highest throughput: 3D NAND and FeNAND reach $\sim$389.7$\times$ over the RTX~4090 ANN-SoLo baseline, while PCM IMP attains $\sim$239.5$\times$, ReRAM IMP $\sim$78.0$\times$, DRAM NMP $\sim$60.9$\times$, and the FPGA pipeline $\sim$98.4$\times$. GPU-side HDC also scales well: on RTX~4090, HOMS-TC and HyperOMS reach $\sim$23.7$\times$ and $\sim$33.8$\times$, respectively; scaling to H100 yields $\sim$70.9$\times$ (HOMS-TC) and $\sim$101.2$\times$ (HyperOMS).

When the entire synthetic library must reside in device-local memory (Table~\ref{tab:syn-entire}), speedups compress due to capacity-driven device replication and ingress/egress effects. Memory-/storage-centric designs span $\sim$2.4$\times$ (ReRAM) to $\sim$10.2$\times$ (FPGA) and $\sim$8.2$\times$ (3D NAND/FeNAND). On GPUs, HOMS-TC remains strong on RTX~4090 at $\sim$59.2$\times$, while HyperOMS yields $\sim$10.7$\times$ and H100 ANN-SoLo sits near parity at $\sim$0.90$\times$. The iso-speed configuration (Table~\ref{tab:syn-same-speed}) sets all speedups to 1 by construction and is used solely to compare energy at matched throughput.

\subsubsection{Energy Efficiency}
For HEK (Table~\ref{tab:hek}), energy efficiency (search) peaks with storage-/NVM-centric designs: FeNAND $\sim$7.67$\times 10^{5}$, PCM $\sim$3.05$\times 10^{5}$, ReRAM $\sim$1.27$\times 10^{5}$, and 3D NAND $\sim$9.24$\times 10^{4}$, followed by DRAM NMP $\sim$1.23$\times 10^{3}$ and FPGA $\sim$53.5. GPU-side HDC improves efficiency as well: RTX~4090 HOMS-TC $\sim$9.70, HyperOMS $\sim$18.8, and on H100 these rise to $\sim$18.7$–$36.2. Including the one-time reference load (search + load) reduces all values but preserves ordering; even then, FeNAND and PCM remain in the $\mathcal{O}(10^{5}$–$10^{6})$ range and ReRAM/NAND in the $\mathcal{O}(10^{4}$–$10^{5})$ range.

On the synthetic entire-library setting (Table~\ref{tab:syn-entire}), the same pattern holds. Memory-/storage-centric designs retain large advantages on search energy (e.g., FeNAND $\sim$7.67$\times 10^{5}$, PCM $\sim$3.05$\times 10^{5}$), while \emph{search + load} values drop as the one-time write is amortized over the billion-scale corpus (e.g., FeNAND $\sim$5.06$\times 10^{5}$, PCM $\sim$1.94$\times 10^{5}$, ReRAM $\sim$9.03$\times 10^{4}$, 3D NAND $\sim$4.12$\times 10^{4}$). Under iso-speed (Table~\ref{tab:syn-same-speed}), the relative ordering is unchanged: at equal throughput, IMP/ISP designs remain two to six orders of magnitude more energy-efficient than the GPU baseline, while GPU HDC retains a consistent 1–2 orders of magnitude gain over ANN-SoLo.




\subsubsection{Accuracy Preservation}
% - HDC-based methods achieve consistent results across devices


\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{fig/final_identifications_comparison_ber_withdrops.pdf}
  \caption{Impact of injected bit error rate (BER) on HyperOMS identifications for datasets b1906--b1931}
  \label{fig:hyperoms-ber}
\end{figure}


\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{fig/upset.pdf}%
  \caption{TEMP: Comparing upset plot}
  \label{fig:UPSET}
\end{figure*}


Total identifications (Fig.\ref{fig:hyperoms-ber})  is a indicator of robustness and practical utility at fixed FDR. In our BER experiments, HyperOMS-BIN tracks the INT8 baseline closely at low BER ($\leq 10\%$), and the decline at $15\%$ BER is modest and dataset dependent (about $9$--$14\%$). These totals show that overall discovery coverage degrades gracefully as errors increase.

At the same time, total identifications alone cannot determine whether the same peptides are being recovered. To assess correctness more directly, we analyze set overlaps with UpSet plots. The UpSet overlaps quantify agreement on high-confidence peptide identifications between HyperOMS and the INT8 reference across BER settings. In effect, totals summarize coverage, while UpSet overlaps provide an accuracy-oriented counterpart that tests the consistency of the recovered peptides.

The injected BER models device-level bit errors observed in multi-level non-volatile memories operated at tight sensing margins. The chosen BER levels correspond to regimes reported for higher bits-per-cell operation, so the stress tests reflect realistic hardware conditions \sumukh{need citation}. The measured resilience is consistent with hyperdimensional computing: binary encodings with Hamming-style similarity distribute information across many dimensions, so random bit flips tend to average out rather than cause catastrophic rank changes.

To complement total identifications, we summarize identification consistency with UpSet plots (Fig.\ref{fig:UPSET}) for dataset b1906 across BER $\in \{0,5,10,15\%\}$. Because ground truth is not available for HEK293, we treat the consensus of ANN-SoLo and HOMS-TC (INT8) as a proxy reference and quantify HyperOMS recovery of that consensus. Here, \emph{recovery} is the size of the three-way intersection (ANN\_SoLo $\cap$ HyperOMS\_BIN $\cap$ HOMS-TC) divided by the sum of the two-way consensus (ANN\_SoLo $\cap$ HOMS-TC) and that three-way intersection. Using the verified counts, recovery is $96.78\%$ at $0\%$ BER, $95.73\%$ at $5\%$ BER, $94.47\%$ at $10\%$ BER, and $91.41\%$ at $15\%$ BER. The consensus remains close to the $0\%$ BER reference through $10\%$ BER and shrinks moderately at $15\%$ BER, with most differences concentrated near the reporting threshold rather than reflecting wholesale rank shifts. Taken together, the UpSet overlaps provide the accuracy-oriented counterpart to totals: they show that HyperOMS preserves the bulk of high-confidence identifications while degrading smoothly as BER increases, consistent with the robustness of hyperdimensional encodings and Hamming-style similarity.


Taken together, the totals and the UpSet overlaps indicate that HyperOMS maintains substantial identification coverage and preserves a large fraction of high-confidence peptides under realistic device-level error, supporting its suitability for memory-centric deployments.







% \paragraph{Discussion.}
% Results show that memory- and storage-centric accelerators deliver one to three orders of magnitude speedup over GPUs by reducing data movement. Non-volatile IMP (PCM/ReRAM) achieves the highest energy efficiency, leveraging MLC density and HDC’s noise tolerance. 3D NAND and FeNAND provide unmatched scalability; FeNAND further alleviates NAND’s sequential bottleneck with DBAM. GPUs remain effective for moderate-size libraries but require hundreds of devices for terabyte-scale OMS. These findings indicate that future OMS accelerators will likely combine GPU-class compute with memory-/storage-centric search primitives.



% \subsection{HEK293 Dataset and Evaluation Setup}
% We evaluate HEK293 tandem mass spectrometry data with 24 peak files and an average of 46{,}665 spectra per file. Queries use subsets b1906 to b1931. Each spectrum is embedded as an 8{,}192 dimensional vector. Searches are run against the MassIVE-KB human spectral library with 2{,}992{,}672 reference spectra. The original reference footprint is about 10\,GB; with a binary representation it is about 2.85\,GB (1 bit per element), and with INT8 it is about 22.83\,GB.

% We use a unified metric for both energy and latency: search plus a one time reference write (load). The one time write is appropriate because the library is static, and it is especially relevant for memory centric designs where per query search is extremely fast and the initial load can dominate amortized cost. We run on available mature hardware and treat those measurements as golden baselines for device and array level simulations. For fair cross platform comparisons, we scale these baselines to representative devices and technology nodes. On GPUs we run ANN-SoLo (shifted cosine or shifted dot product rescoring) and HyperOMS in binary and INT8 (HOMS-TC on tensor cores) on an RTX\,4090, then scale to an H100 target using normalized memory bandwidth and compute throughput or TOPs. For FPGA we use a near storage configuration on Samsung or Xilinx SmartSSD CSD (Kintex UltraScale+), then scale to a Versal Premium VP1902 device with attached DRAM. For ReRAM we run on a NeuRRAM chip and report two projections at 130\,nm and 40\,nm.



% \subsection{Synthetic TB-Scale Reference (SYN)}
% We construct a synthetic terabyte scale workload to study billion scale behavior. The dataset contains 15{,}000 queries and 1{,}000{,}000{,}000 references, each a binary 8{,}192 dimensional vector (about 1\,KiB per reference), for a total reference store of about 0.95\,TiB (about 1\,TB).

% During search, the full reference database resides in device local memory to exclude host or storage I/O. Concretely, RTX\,4090 uses on board GDDR6X (24\,GB, about 1\,TB/s), H100 uses HBM (80\,GB, about 3.35\,TB/s), and the FPGA path uses board DRAM on a VP1902 class design. Memory centric designs (DRAM NMP, ReRAM, PCM, 3D NAND, FeNAND) store references directly in the array.

% To hold about 1\,TB of references, we replicate devices according to capacity: about 43 RTX\,4090 GPUs, about 13 H100 GPUs, about 16 VP1902 boards with DRAM, about 16 DRAM NMP devices, and about 5 packages each for ReRAM, PCM, 3D NAND, and FeNAND. For memory centric devices we model a 64 bit interface at 200\,MHz with sequential readout of indices and similarity scores, broadcast queries to all devices, include peripheral overheads (sense paths, lightweight mixed signal, controller), and normalize technology nodes to representative processes (GPU 5\,nm, FPGA 7\,nm, DRAM 22\,nm, ReRAM 40 to 130\,nm, PCM 40\,nm, NAND or FeNAND 14\,nm arrays with 7\,nm CMOS periphery). We reuse the same methodology as above: RTX\,4090 measurements scaled to H100 using normalized memory bandwidth and compute throughput or TOPs, SmartSSD CSD scaled to VP1902 with DRAM, and NeuRRAM measurements with projections at 130\,nm and 40\,nm. We apply the same reporting convention of search plus one time reference write (load).


==> TEX/NOT_USEDMEMORYAccelerators.tex <==
\textcolor{red}{\section{NOT used Accelerator Architectures for MS Search}
\subsection{Memory-Centric Accelerators}
\subsubsection{ReRAM and PCM IMP}
%
Resistive RAM (ReRAM) and Phase-Change Memory (PCM) support analog in-memory computing through crossbar arrays. Their multi-level-cell (MLC) capability increases density while enabling massively parallel similarity operations.
%
\paragraph{Architecture }
In both designs~\cite{dac2024rram,jxcdc2024pcm}, queries are applied as voltages across bitlines, with references stored in device conductances. Summed currents along columns implement matrix–vector multiplications that approximate similarity. Techniques such as differential mapping (ReRAM) and dimension packing (PCM) align binary hypervectors with MLC operation.
%
\paragraph{Peripheral Modifications }
\begin{itemize}
    \item DAC drivers to generate analog voltages.  
    \item Sense amplifiers or flash ADCs for digitization.  
    \item Write-verify modules for MLC calibration.  
    \item Near-memory ASIC logic for accumulation and thresholding.  
\end{itemize}
PCM designs further optimize material stacks (low-voltage PCM for clustering, high-retention PCM for DB search).
%
% 
ReRAM and PCM IMP achieve $25$–$143\times$ speedup and three to four orders of magnitude energy improvement versus GPU baselines. However, endurance (ReRAM), drift (PCM), and ADC overhead remain challenges. Section~\ref{sec:accelerators} discusses how these trade-offs impact OMS workloads.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/RRAM.pdf}
    \caption{ReRAM IMP: crossbar arrays with ADCs.}
    \label{fig:reram}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/PCM.pdf}
    \caption{PCM IMP: crossbar arrays with DACs, ADCs, and near-memory ASIC support MLC-based in-memory computing.}
    \label{fig:pcm}
\end{figure}
%
%
\subsection{Memory-Centric Accelerators}
\subsubsection{ReRAM IMP}
ReRAM arrays~\cite{dac2024rram} store reference hypervectors as multi-level conductance values. Queries are applied as voltages on wordlines, producing summed bitline currents proportional to overlaps. Flash ADCs digitize these currents, and digital counters accumulate Hamming similarities. A 64-bank design demonstrated $76.7\times$ GPU speedup and $500$–$3000\times$ better energy efficiency. HDC robustness tolerates up to $10\%$ device errors, ensuring accuracy despite analog variation.
%
\subsubsection{PCM IMP}
PCM designs~\cite{jxcdc2024pcm} follow a similar mapping but employ binary and multi-level cells jointly. Reference hypervectors are packed across multiple banks, while queries are applied as voltage pulses to activate resistive states. Dimension packing and data grouping reduce latency and storage footprint. With optimized calibration and verify circuits, PCM IMP achieved up to $5303\times$ GPU speedup and $817{,}000\times$ efficiency, though drift and endurance remain limiting factors.
}









% \subsubsection{3D NAND ISP for OMS}

% \textbf{Motivation and architecture.} 
% In-storage processing with 3D NAND enables large-scale similarity search to be performed directly within the memory array, avoiding the costly host--device transfers that dominate latency and energy in conventional systems. The spectral library is stored as hypervectors mapped along wordlines, one per page. Demonstrations to date have primarily targeted SLC devices, while MLC and TLC increase storage density but require iterative threshold sensing, extending the time per read.

% \textbf{Query application and similarity primitive.} 
% Queries are injected on the bitlines. When a wordline is activated, thousands of bitlines evaluate in parallel, and the resulting source-line current encodes the bitwise overlap between the query and the stored references. These currents are sensed through the existing periphery (page buffers and sense amplifiers), digitized per page, and accumulated across the wordlines that together form a reference vector.

% \textbf{Parallelism and constraints.} 
% Parallelism is achieved across three dimensions: bitlines within a page, planes and blocks within a die, and multiple tiles across the package. The primary constraint is that conventional arrays typically allow only one wordline per block to be active at a time, forcing sequential progress along the vertical axis. In multi-level devices, iterative reads further increase dwell time. Device variation and wear-induced drift limit precision, but modest calibration and lightweight post-processing ensure robust operation.

% \textbf{Outcome.} 
% 3D NAND ISP executes HyperOMS fully inside storage, harnessing extreme capacity and eliminating PCIe traffic. The principal limitation is sequential progress across wordlines, which constrains fine-grained parallelism compared to DRAM- or ReRAM-based PIM, but the energy and capacity advantages are substantial for terabyte-scale OMS libraries.

% \subsubsection{3D FeNAND ISP for OMS (FeNOMS)}

% \textbf{Architectural extensions.} 
% FeNAND preserves the same high-level tile structure as NAND but introduces a column-wise mapping of hypervectors. References are stored vertically along strings, which enables controlled activation of multiple wordlines simultaneously. Queries are applied through the wordlines, aligning query bits with their vertical positions in the stored hypervector. This arrangement allows multiple rows to be activated in one step, producing a binary outcome per string delivered directly by the sense amplifiers and page-buffer path. Unlike conventional NAND ISP, no on-tile ADC is required.

% \textbf{Dual-Bound Approximate Matching (DBAM).} 
% To address the latency of sequential wordline activation, FeNAND introduces Dual-Bound Approximate Matching (DBAM). DBAM applies tolerance-based checks on subsets of rows: an upper bound imposes a strict acceptance condition, while a lower bound applies a more relaxed criterion. Candidates that fail both checks can be eliminated before completing all row evaluations, thereby reducing the total number of reads. This mechanism requires only minor decoder modifications for multi-row activation and reuses existing peripheral circuits, with less than 0.5\% reported overhead.

% \textbf{Multi-level sensing.} 
% For MLC and TLC devices, DBAM reduces reliance on iterative threshold sensing. Instead of multiple reads per page, DBAM produces a single binary pass/fail output, significantly lowering per-candidate energy and latency.

% \textbf{Accuracy and trade-offs.} 
% DBAM is designed with conservative bounds to maintain OMS ranking fidelity. Slightly relaxed tolerances allow more aggressive pruning, yielding higher throughput at the cost of small reductions in accuracy. This balance makes FeNAND well-suited for large-scale OMS where throughput and energy efficiency are critical.

% \textbf{Outcome.} 
% FeNAND inherits the capacity and database-locality advantages of NAND ISP while alleviating vertical serialization through column-wise mapping, multi-row activation, and DBAM. Together, these enhancements deliver higher throughput and lower energy consumption, establishing FeNAND as a scalable in-storage accelerator for OMS workloads.


==> TEX/Section3BACKUP.tex <==
\section{Cross-Domain OMS Accelerator Designs (Architecture \& Mapping)}

Section II established that OMS is constrained by bandwidth and capacity at scale and benefits from simple similarity kernels. Section III now details concrete accelerator designs and how OMS maps to each platform.

\subsection{GPU (NVIDIA RTX 4090, H100)}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/gpu_placeholder.png}
    \caption{GPU WILL BE CHANGED}
    \label{fig:gpu_arch}
\end{figure}

GPUs serve as the baseline for OMS acceleration, pairing tens of teraflops of compute with high-bandwidth device memory (e.g., 24\,GB GDDR6X on RTX~4090, 80\,GB HBM2E on H100). Two kernel mappings capture their role. \textit{ANN-SoLo}~\cite{annsolo} evaluates real-valued spectra with FP32 cosine similarity, exploiting vectorized math units but incurring heavy cost once the library exceeds device capacity. In contrast, HDC-based designs such as \textit{HyperOMS}~\cite{kang2022massively} and \textit{HOMS-TC}~\cite{kang2023homstc} score binary (BIN) or low-precision encodings with XOR + population count or INT8 tensor-core kernels, offering higher throughput and efficiency.

When the library fits in memory, queries are staged and scored entirely on device. For larger databases, shards must be streamed over PCIe/NVLink, and multi-GPU deployments require sharding/replication with host-side top-$k$ merging. GPUs thus provide strong compute and a mature software stack, but limited memory relative to terabyte-scale OMS makes data movement the dominant bottleneck.

% Modern GPUs provide the baseline for high-throughput OMS acceleration. Devices such as the NVIDIA H100 couple 80~GB of HBM3e with multi-terabyte per second sustained bandwidth and tens of thousands of SIMT and tensor cores. Prosumer cards such as the NVIDIA RTX~4090 provide 24~GB of GDDR6X and roughly one terabyte per second of device memory bandwidth. The hierarchical memory system, HBM or GDDR, multi-level caches, shared memory, and registers, supports massive concurrency, and tensor cores accelerate low-precision operations.

% Two representative kernel mappings illustrate GPU capabilities for OMS. In ANN-SoLo~\cite{annsolo}, feature-hashed real-valued vectors are stored in device memory and scored with cosine similarity. This exploits the GPU's vectorized math units, but exact FP32 cosine on large libraries is heavy and requires partitioning once the database exceeds device capacity. In contrast, the HDC pipeline encodes spectra as binary hypervectors and scores with Hamming similarity. HyperOMS~\cite{kang2022massively} demonstrated binary encoding with XOR and population count, which can be implemented efficiently on GPUs. HOMS-TC added configurable precision, for example FP32 or INT8, and tensor-core friendly tiling so users can trade accuracy and throughput while staying within the HDC framework.

% When the database fits in device memory, queries are staged in batches, scored against all resident references, and reduced to top-$k$ entirely on device. Larger libraries require streaming shards from host DRAM or storage over PCIe, which introduces substantial transfer overhead. Multi-GPU systems mitigate this by sharding or replicating libraries across devices, then merging per-device top-$k$ through host-coordinated aggregation. GPUs offer strong computational throughput and a mature software stack, but on-device memory is modest relative to terabyte-scale OMS libraries, and repeated host to device transfers dominate latency and energy at scale.






\subsection{FPGAs (SmartSSD-class, VP1902-class)}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{fig/FPGA.pdf}
    \caption{FPGA SmartSSD architecture: FPGA fabric, DRAM buffer, and NVMe controller process spectra near storage.}
    \label{fig:fpga_arch}
\end{figure}

As shown in Figure~\ref{fig:fpga_arch}, near-storage FPGA systems couple reconfigurable logic with device DRAM inside the SSD enclosure, so reference traffic does not traverse the host. A SmartSSD-class device integrates an FPGA and DRAM buffer alongside NAND and an NVMe controller; newer VP1902-class fabrics scale resources for wider parallelism and deeper buffering while preserving the same streaming dataflow.

OMS maps cleanly to FPGA bitwise engines~\cite{pinge2024rapidoms}. References are stored as binary hypervectors and compared with XOR + population count across many parallel lanes, with per-query top-$k$ maintained on device. Queries arrive as streams, are fanned into the lanes, and only compact results return to the host. Cached reference slices in device DRAM serve repeated queries; larger libraries are streamed block by block from NAND into device DRAM while the fabric processes the current block. FPGAs thus provide a flexible near-storage substrate, trading higher programmability for less density compared to NVM-based designs.

% Near-storage FPGA systems place reconfigurable logic and device DRAM inside the SSD enclosure so compute sits close to the data. A SmartSSD-class device couples an NVMe controller, an FPGA (Xilinx KU15P), and a small device DRAM cache, while the spectral library remains on NAND. KU15P is an older fabric; newer VP1902-class devices provide roughly $16\times$ more resources in a similar near-storage configuration. With VP1902-class logic colocated with NVMe storage, systems can host more parallel lanes, deeper on-chip score buffers, and larger device-DRAM caches, raising ceiling performance while preserving the streaming dataflow. The FPGA pulls library blocks over the internal path, executes lightweight similarity, and returns only compact results to the host.

% OMS maps cleanly to bitwise engines. References are encoded as binary hypervectors for XOR and population count. The FPGA instantiates many parallel lanes with simple control and maintains per-query running top-$k$ on device. The core is an unrolled XOR plus population-count kernel, implemented with HLS optimizations. Queries arrive as streams from the host and are fanned into the parallel lanes. Because the library stays on the drive side, high-volume reference traffic does not traverse the host. The fabric is fully configurable, so kernels can be tuned for vector width, lane count, buffering, and top-$k$ reducer depth.

% When the working set fits in device DRAM, cached reference slices are reused across many queries. Larger libraries are streamed block by block from NAND into device DRAM while the fabric computes on the current block.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{fig/FPGA.pdf}
%     \caption{FPGA SmartSSD architecture: FPGA fabric, DRAM buffer, and NVMe controller process spectra near storage.}
%     \label{fig:fpga_arch}
% \end{figure}



\subsection{DRAM-Centric Accelerator}

DRAM NMP augments commodity DDR4 banks with lightweight Hamming Search Engines (HSEs) placed near the row buffer. Reference hypervectors are striped across rows, with multiple vectors packed per row via column offsets. When a query arrives, it is broadcast into per-bank registers, and each bank scans its shard in parallel.

On a row activation, the sense amplifiers expose $K$-bit segments that are XORed with the query and accumulated with a bit-serial popcount. To reduce work, the HSE employs folding: it computes a partial similarity first and rejects low-quality candidates before completing the full evaluation. This early-exit mechanism eliminates nearly half the bit operations with minimal accuracy loss. Each bank maintains its top matches locally while scanning proceeds asynchronously, so overall throughput scales with the number of banks and subarrays.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/DRAM.pdf}
    \caption{DRAM: encoding banks use in-DRAM primitives; search banks integrate near-bank HSEs with a dispatcher.}
    \label{fig:dram_IMP}
\end{figure}


% \subsection{DRAM-Centric Accelerator}

% This design built on commodity DDR4 DRAM chips. Each DRAM bank integrates a small Hamming Search Engine (HSE) near the bottom-subarray row buffer. Reference hypervectors are striped across rows: a $D$-bit vector is split into $D/K$ consecutive rows, each row holding $K$-bit segments. Multiple references are packed per row using column offsets so that one row activation fetches segments for more than one hypervector. A dispatcher maintains a mapping of row and column offsets for each stored reference.

% When a query arrives, it is loaded into small query registers inside each bank. The controller broadcasts the relevant row range, and every bank searches its shard in parallel. A row activation latches its bits into sense amps and row buffers (sub-60~ns). The row buffer is divided into $K$-bit segments, and the HSE performs parallel XORs between the query and all segments, followed by bit-serial popcount to compute Hamming similarity. To reduce work, the HSE uses folding: it first evaluates a partial similarity (for example, half of the bits) and rejects candidates below a threshold before reading the remainder. This ``early exit'' path avoids nearly half the bit operations with little loss in accuracy. Each bank tracks its best match locally while scanning rows asynchronously.


\subsection{Memory-Centric Accelerators (ReRAM and PCM)}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/RRAM.pdf}
    \caption{ReRAM IMP: crossbar arrays with ADC-based readout.}
    \label{fig:reram}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/PCM.pdf}
    \caption{PCM IMP: crossbar arrays with DAC/ADC support for multi-level cells (MLCs).}
    \label{fig:pcm}
\end{figure}

Resistive RAM (ReRAM) and phase-change memory (PCM) are non-volatile memories that support massively parallel in-memory operations through crossbar arrays. Both technologies offer multi-level-cell (MLC) capability, increasing effective density and enabling vector–matrix style computations suitable for similarity search. In OMS, reference hypervectors are mapped to device conductances, and queries are applied as input voltages across bitlines. Column currents represent partial similarities, which are digitized by ADCs and accumulated by peripheral logic.

As illustrated in Fig.~\ref{fig:reram}, ReRAM IMP applies query voltages to the bitlines of 1T1R crossbars, where programmed cell conductances encode reference bits. The resulting column currents are sensed and converted to digital form, effectively computing XOR- or dot-product style similarity inside the array. ReRAM-based designs~\cite{fan2024mlcrram} exploit fast reads, simple fabrication, and high density. Binary or few-level operation provides stable storage, while MLC expands capacity but introduces conductance drift and relaxation, which degrade precision. Hyperdimensional computing mitigates this by distributing information across thousands of dimensions, allowing OMS to tolerate drift and bit errors during MLC operation.

PCM IMP, shown in Fig.~\ref{fig:pcm}, follows a similar crossbar principle but incorporates DAC drivers for multi-level programming and ADCs for precise digitization. SpecPCM~\cite{fan2024specpcm} demonstrates how optimized PCM stacks reduce programming voltage, switching energy, and resistance drift, stabilizing MLC operation and raising effective density. In this design, queries drive analog voltages across wordlines, accumulated currents are digitized, and near-memory ASIC logic aggregates partial results. Despite these advantages, PCM still faces challenges from write latency, endurance, and residual MLC error rates that can exceed 10\% even after verify. Here too, the error resilience of HDC is critical for practical deployment.

Overall, ReRAM and PCM IMP achieve large speedups and multi-order-of-magnitude energy improvements compared to GPU baselines, but their adoption depends on balancing density and parallelism against device-level variability, endurance, and ADC overheads.



\subsection{Storage-Centric Accelerators (3D NAND and FeNAND)}

Modern OMS workloads routinely exceed main memory capacity, so spectral libraries live on SSDs. Even with high SSD bandwidth, shuttling gigabytes per query batch across the host to device boundary dominates latency and energy. In-storage processing addresses this by performing the core similarity inside the storage package, collapsing host to storage movement. Storage-centric accelerators execute similarity search inside high-density flash packages so the library remains on device. A tile augments a 3D NAND or FeNAND array with lightweight mixed-signal and digital periphery. References are stored as binary hypervectors in the array, and queries are applied as bitline voltage patterns. Activating a wordline drives thousands of bitlines in parallel; source-line currents encode the bitwise overlap with the query; tile-local page buffers and ADCs digitize these signals; small accumulators sum across the wordlines that compose a vector to produce per-reference scores. Only compact outputs, for example top-$k$ indices and scores, leave the device. Parallelism comes from bitlines within a page, planes and dies within a package, and multiple tiles on the module. FeNAND preserves the same tile structure and OMS execution flow as 3D NAND; under like configurations, latency is governed by shared 3D array RC characteristics, so architectural behavior is similar. Heterogeneous integration can fold periphery beneath and above the array, with CMOS-under-array for high-voltage switching and face-to-face bonding of low-voltage mixed-signal and digital logic, creating dense tiles that support both HDC encoding and similarity and that share queries and reductions over an on-package network.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/NAND.pdf}
    \caption{3D NAND and FeNAND ISP: heterogeneous integration enables in-storage encoding and search; FeNAND reduces latency with D-BAM. \cesong{need to be changed}}
    \label{fig:nand_fenand}
\end{figure}







 


==> TEX/backup_5.OMS_Model.tex <==



% \textcolor{red}{Below 2 sections are changed heavily}

\section{Methodology  for Comparative Study}\label{sec:eval}

Given the wide variety of device characteristics, memory capacity, and operating mechanisms across accelerator platforms, it is crucial to establish a consistent and fair evaluation setup for the comparative study. This section outlines the methodology to construct a fair evaluation framework for both the dataset, algorithm, and the hardware setups.


\subsection{Algorithm and Workload Configuration}\label{sec:bottlenecks}


\mingu{\\- While GPU handles FP32 and INT, INP is hard to process in MLC limit. 
\\
- Often it is mapped on the more favorable form as introduced in background. (kernel simplification goes here, but without such name, just say HD)
\\
- We employ the workloads in Table I with 2 different scales, mid and large ($>$1TB). 
\\
- Table I shows  HOMS-TC (int), RapidOMS and ANN-SoLO (fp) used for GPU or FPGA, HyperOMS for IMC along with the dataset XXXX}

Building on Section~\ref{sec:oms-model}, a \emph{memory wall} emerges once the staged working set exceeds the resident capacity of the executing device (e.g., a GPU's HBM/GDDR). In this regime, throughput is no longer set by on-device arithmetic; instead, the accelerator must repeatedly stream reference data over the host-device interface (or from storage), and performance is bounded by external bandwidth and staging overhead. \sumukh{Motivated by this bottleneck, we organize our designs around two architectural design targets that we enforce whenever the substrate permits:}

%\textbf{Data locality:} Execute scoring where the references reside (in-memory or in-storage), so that only compact top-$k$ results traverse the interconnect.
Use massively parallel, bitwise primitives (XOR + popcount) that map efficiently to memory-array periphery without incurring the area/energy overhead of floating-point datapaths~\cite{imani2017voicehd,kang2023homstc,kang2022massively}.


To quantify the benefit of these rules across heterogeneous substrates, we adopt a three-tier evaluation methodology that cleanly separates (i) algorithmic simplification, (ii) substrate-dependent execution efficiency in the \emph{mid-scale deployment} regime, and (iii) system-level efficiency in the \emph{datacenter} regime at extreme scale.

\paragraph{\textbf{Baseline Algorithmic Efficiency (Table~\ref{tab:hek-managed})}}
We first measure the performance impact of reduced precision on commodity accelerators by comparing an FP32 baseline (ANN-SoLo) against INT8 execution (HOMS-TC) on RTX~4090 and H100 GPUs. This comparison isolates the speedup achievable via arithmetic simplification before addressing the data movement bottleneck.

\paragraph{\textbf{Mid-Scale Substrate Analysis via Unified HDC Algorithm (Table~\ref{tab:hek-hyperoms-only})}}
Next, we fix the algorithm to HyperOMS (binary HDC, $b=1$) to enable an equitable comparison across memory technologies in the \emph{mid-scale deployment} regime. We compare commodity and near-data substrates---GPUs, near-storage FPGAs, DRAM-NMP~\cite{kang2024dram}, non-volatile IMP (ReRAM~\cite{fan2024mlcrram}, PCM~\cite{fan2024specpcm}), and capacity-normalized 3D NAND/FeNAND ISP tiles~\cite{hsu2023memsys,hsu2025fenand}---using identical per-package capacity and an identical OMS workload. Crucially, we report both ``Search-Only'' and ``Search + Load'' metrics to quantify the energy penalty of volatile architectures that must repeatedly stage reference data from host memory, versus non-volatile substrates where the library is persistent in-place.

\paragraph{\textbf{Datacenter-Scale Scalability at the Terabyte Limit (Table~\ref{tab:hek-large})}}
Finally, we stress test scalability by increasing the reference library to $N=10^9$ ($\approx 1$~TB for binary HDC) in a datacenter setting. For this regime, we restrict comparisons to NVIDIA H100 and full SSD-scale ISP architectures (3D NAND and FeNAND), which exploit die/plane-level parallelism for large-corpus OMS~\cite{hsu2023memsys,hsu2025fenand}. We exclude DRAM-NMP and ReRAM/PCM-IMP from this experiment because provisioning terabyte-scale capacity on these technologies implies an impractical device count and area footprint. This study therefore isolates the dominant bottlenecks of the \emph{transient} regime (GPU streaming over PCIe/NVLink) versus the \emph{persistent} regime (in-place ISP execution).


\subsection{OMS Workload Scaling and Data-Movement}
\label{sec:oms-scaling}

To support a structured evaluation across substrates, we now formalize the workload-scaling and data-movement model used throughout Section~\ref{sec:eval}. The goal is to make explicit when OMS operates in a resident regime versus a transient staging regime, and to define a consistent normalization basis for cross-platform comparisons.\mingu{this paragraph's language should be more clear.}

\subsubsection{OMS Computational Model and Staging Constraints}\label{sec:oms-model}

\begin{table}[h]
\caption{Notation for OMS Computational Model \mingu{do we need all of them ? or, just abstract and explain in a text ?}}
\label{tab:oms-notation}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{@{}lX lX@{}}
\toprule
\textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
\midrule
$Q_b$ & Query batch set & $b$ & Precision (bits/element) \\
$q$ & Single query ($q \in Q_b$) & $N$ & Total reference count \\
$C_q$ & Candidate reference set & $F$ & Per-reference footprint (B) \\
$D$ & Vector dimensionality & $S$ & Total Library Size ($N \cdot F$) \\
$W_{\mathrm{calc}}$ & Arithmetic Workload & $P$ & Device packages required \\
$C_{\mathrm{res}}$ & Resident capacity of executing device & $C_{\mathrm{dev}}$ & Usable capacity per persistent device/package \\
$\mathrm{BW}_{\mathrm{ext}}$ & External I/O bandwidth &  &  \\
\bottomrule
\end{tabularx}
\end{table}




\cesong{Beyond the spectrum-encoding pipeline, OMS performance is fundamentally shaped by how the workload scales with library size, representation precision, and device-resident capacity. 
To clarify these effects, we summarize the dominant factors governing data movement and throughput.}
Table~\ref{tab:oms-notation} defines the core notation for the OMS workload. For a query batch $Q_b$, the arithmetic work scales as $W_{\mathrm{calc}} = \sum_{q \in Q_b} |C_q| \cdot D$. At repository scale, however, throughput is often dominated by the cost of staging the reference library $\mathcal{L}$ into the execution units rather than by the raw compute required for scoring.

References are stored in contiguous blocks (pages or erase blocks) to amortize I/O latency. We define the total library size (footprint) as
\begin{equation}
    S = N \times F = N \times \left\lceil \frac{D \cdot b}{8} \right\rceil .
\end{equation}
This exposes the direct impact of representation precision: standard pipelines typically use FP32 ($b=32$), quantized approaches (e.g., HOMS-TC) use INT8 ($b=8$), and HyperOMS uses binary representations ($b=1$). Unlike targeted search, OMS often operates under wide precursor tolerances, so the candidate sets $C_q$ can span a substantial fraction of the library; in the worst case, the staged footprint approaches a full linear scan.

The system's operating regime is determined by whether the staged working set fits within the resident capacity of the executing device. Let $C_{\mathrm{res}}$ denote the resident capacity (e.g., a GPU's HBM/GDDR or a device-side buffer), and let $C_{\mathrm{dev}}$ denote the usable capacity of a provisioned persistent substrate (e.g., DIMM/SSD package or a capacity-normalized tile budget). If we provision a persistent substrate to store the entire library in-place, the minimum number of device packages is $P = \left\lceil S / C_{\mathrm{dev}} \right\rceil$. In contrast, commodity accelerators typically execute with a limited resident working set. When the staged footprint $S$ exceeds $C_{\mathrm{res}}$, the workload enters a \textit{transient staging regime}: reference blocks must be repeatedly streamed over the external interface, and throughput becomes bounded by the effective external bandwidth $\mathrm{BW}_{\mathrm{ext}}$ (e.g., PCIe/NVLink or a storage link) rather than by on-device compute. In this regime, each pass over the staged working set incurs $\Theta(S / \mathrm{BW}_{\mathrm{ext}})$ data movement, which quickly dominates per-batch execution time as $S$ scales. This model links representation choices $(b, D)$ to staging cost via $S$, and we use it as the normalization basis for cross-platform evaluation.






%==============================================================%



% \begin{table}[t]
% \caption{Notation for OMS Computational Model}
% \label{tab:oms-notation}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabularx}{\columnwidth}{@{}lX lX@{}}
% \toprule
% \textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
% \midrule
% $Q_b$ & Query batch set & $b$ & Precision (bits/element) \\
% $q$ & Single query ($q \in Q_b$) & $N$ & Total reference count \\
% $C_q$ & Candidate reference set & $F$ & Per-reference footprint (B) \\
% $D$ & Vector dimensionality & $S$ & Total library size ($N \cdot F$) \\
% $W_{\mathrm{calc}}$ & Arithmetic workload & $P$ & Device packages required \\
% $C_{\mathrm{dev}}$ & resident capacity per device & $\mathrm{BW}_{\mathrm{ext}}$ & External I/O bandwidth \\
% \bottomrule
% \end{tabularx}
% \end{table}


% \subsection{Primary Computational Challenges}
% At repository scale, the dominant cost in OMS lies in data movement rather than in the comparison operations themselves. Each query must touch a substantial portion of the library. Once the library exceeds device memory, the system spends most of its time moving pages between storage, host DRAM, and the accelerator. Even when the library fits, repeatedly moving multi-gigabyte batches through the hierarchy often dominates kernel time. Therefore, Capacity limits become performance limits: tens of GB of HBM or GDDR are small relative to multi-terabyte libraries, which forces partitioning and streaming that erode locality and keep the I/O fabric saturated.
% %
% Computation remains consequential because shifted-cosine and Hamming similarity aggregate over high-dimensional representations. The total work scales with both the candidate set size and the feature dimension, so naive scoring grows quadratically with the effective problem size. Indexing and filtering (approximate nearest neighbor (ANN), fragment ion, tag-based filters) can reduce candidates, but OMS deliberately widens the precursor window, weakening the most effective early filter. At scale, the recall versus speed trade-off becomes sensitive. Aggressive pruning saves time but drops identifications, while conservative pruning preserves quality but pushes the workload back toward exhaustive scoring.
% %
% Consequently, OMS is fundamentally bandwidth and capacity bound, which motivates architectures that place scoring close to where the data resides, inside memory arrays or storage devices, so the primary limiter is addressed while the similarity primitive remains simple enough to execute at scale.
% %
% %
% \subsection{Moving Compute to the Data: IMP, NMP, and ISP Approach}
% OMS is bandwidth bound, so we place computation near where the references are stored. \emph{In-Memory Processing (IMP)} executes inside the array (for example, DRAM row operations with near-bank Hamming engines, or ReRAM/PCM crossbars that realize small vector operations). \emph{Near-Memory Processing (NMP)} adds lightweight logic at banks, subarrays, or the controller to exploit internal parallelism without disturbing array regularity. \emph{In-Storage Processing (ISP)} performs similarity directly inside storage devices such as 3D NAND and FeNAND by pairing array tiles with simple mixed-signal or digital reduction logic.
% %
% Across these substrates the OMS kernel is intentionally simple: XOR + population count for binary hypervectors, or a small dot product that reduces to the same decision. Queries are injected once per device and fanned out internally; only compact results (top-$k$ indices and scores) leave the device. DRAM-class designs exploit bank and subarray parallelism, ReRAM/PCM leverage crossbar concurrency, and 3D NAND/FeNAND use page-, plane-, and die-level parallelism. FeNAND further reduces vertical serialization through multi-row activation, improving throughput while preserving identification quality. The common goal is to collapse host-device traffic and make terabyte-scale OMS feasible by executing scoring where the references reside.
% %
% \subsection{A Normalized Cross-Device Framework}
% Directly comparing prior results is unreliable because implementations differ in process node, capacity and I/O limits, peripheral circuits (sense amplifiers, DAC/ADCs, controllers), datasets, and accuracy targets. A 5~nm GPU, a 7~nm FPGA, and a 40--130~nm PIM prototype will show very different raw numbers even if the architecture-level idea is similar.
% %
% We therefore adopt a normalized framework: a fixed per-package reference capacity of 1.67~Tb, a common external interface for memory and storage devices (64-bit at 200~MHz), inclusion of peripheral overheads in performance and energy, and mapping each design to a representative process node. Accuracy is held to a common baseline; for PIM/ISP devices we explicitly account for memory non-idealities. This lets us attribute gains to architecture and data-movement reduction rather than process scaling and sets up a fair, single-workload comparison in the evaluation that follows.


% \section{Background and Challenges}
% \subsection{Mass Spectrometry Database Search}
% % - Workload characteristics: large-scale DB (TB-scale), query patterns, matching requirements

% The HyperOMS algorithm, which combines HDC encoding with Hamming-distance search, is inherently processor-agnostic and well suited to in-memory computing. Its reliance on simple primitives (XOR, population count) and resilience to noise make it particularly attractive for direct integration within memory devices. Several prototypes have demonstrated this portability across in-memory processing (IMP) substrates. For instance, Kang et al.~\cite{dramoms} describe a DRAM accelerator where spectral libraries are stored in compute-enabled DRAM arrays, and each bank is augmented with logic to perform bit-wise XNOR and intra-bank reductions. A query hypervector can then be broadcast across banks (or placed near-memory), with partial Hamming distances evaluated in parallel to exploit the DRAM internal bandwidth. Similar efforts have mapped HyperOMS onto non-volatile memory crossbar arrays such as resistive RAM and phase-change memory, leveraging their analog matrix--vector multiplication capabilities to approximate Hamming similarity, thereby transforming the device into an associative spectral search engine.

% Across these implementations, HyperOMS functions as a unifying algorithmic layer. It is important to note that all these accelerators – GPU HOMS-TC\cite{homstc}, RapidOMS FPGA\cite{pinge2024rapidoms}, DRAM \cite{dramoms}, ReRAM\cite{RRAM}, PCM\cite{Fan2024SpecPCM}, designs all yield consistent search outcomes, since they execute the same HDC-based matching procedure. Benchmark comparisons (e.g., the iPRG2012 dataset) confirm that hypervector-based searches recover a comparable spectrum range to conventional methods. In the following section, we analyze these architectures in greater detail, with emphasis on their design principles and the mechanisms by which they implement HDC search at the device level.




% \subsection{Search Algorithms}
% \subsubsection{ANN-SoLo}
% % - GPU-based cosine similarity search, high accuracy but computation-heavy

% \subsubsection{HOMS-TC}
% % - GPU HDC-based search, leverages INT8/INT4 tensor cores for acceleration

% \subsubsection{HyperOMS}
% % - HDC-based, simple XOR + popcount, noise-tolerant, naturally IMP-friendly

% \subsection{Challenges of Fair Comparison between Devices}
% % - Different technology nodes, device interfaces, peripheral overhead
% % - Need for assumptions (DB size, precision, bus frequency) to ensure fairness

% \subsection{Hyperdimensional Computing (HDC)}
% Hyperdimensional computing (HDC) has emerged as a promising abstraction for OMS. In HDC, spectra are encoded into high-dimensional binary hypervectors that capture both fragment indices and intensities. Similarity reduces to lightweight XOR and population count operations, replacing floating-point arithmetic with Boolean logic. HDC offers three critical advantages: (i) robustness to noise and PTM-induced peak shifts, (ii) suitability for highly parallel hardware through bitwise operations, and (iii) portability across diverse accelerators. Algorithms such as HOMS-TC and HyperOMS leverage these properties to unify OMS across GPUs, FPGAs, and diverse devices that implement IMP and NMP platforms.


% \subsubsection{Primary Computational Challenges}
% \begin{itemize}
%   \item \textbf{Data movement.} Each query touches a very large portion of the library. When the library does not fit in main memory, repeated transfers between storage and host memory dominate latency and energy. Even when it fits, shuffling multi gigabyte batches through the memory hierarchy is often the largest cost.
%   \item \textbf{Memory capacity.} Tens of gigabytes of device memory are not enough for multi terabyte OMS libraries. This forces partitioning and streaming, introduces scheduling overheads, and reduces temporal locality.
%   \item \textbf{Similarity computation at scale.} Shifted cosine and Hamming style distances require billions of reductions over high dimensional vectors. Sparsity helps but does not eliminate the total work once candidate sets are large.
%   \item \textbf{Indexing and pruning limits.} Approximate nearest neighbor search, fragment ion indexing, and tag based filters reduce the candidate pool, but wide precursor windows weaken precursor mass pruning and make recall versus speed trade offs more sensitive at large scale.
%   \item \textbf{Irregularity and sparsity.} Spectra differ in peak counts and intensity distributions. This leads to irregular memory access, poor cache reuse, and suboptimal SIMD or SIMT utilization in batched kernels.
%   \item \textbf{Precision and numerical stability.} High quality shifted cosine often relies on FP32 accumulation. Mixed precision or integer encodings must preserve ranking fidelity and stable tie breaking across billions of comparisons.
%   \item \textbf{Throughput versus quality.} Tuning candidate set sizes, similarity kernels, and post filters affects both runtime and identification rates. Maintaining controlled false discovery rate while sustaining high throughput remains a central tension.
%   \item \textbf{Orchestration overheads.} Managing partitions, batching, and top $k$ aggregation across many queries and shards adds nontrivial CPU and I/O coordination overhead.
% \end{itemize}



% \subsubsection{Problem Abstraction}
% Let there be $Q$ queries, $N$ references, and feature dimension $D$ after preprocessing or encoding. OMS computes a similarity $s(\mathbf{q}, \mathbf{r}_i)$ for many $i \in [1, N]$, then selects top $k$ per query. Practical cost scales with the number of scored pairs and the reductions over $D$. In current pipelines, the dominant costs are (i) moving candidate data to where it is scored and (ii) executing a very large number of high dimensional similarity reductions. At repository scale, OMS is fundamentally bandwidth and capacity bound.

==> TEX/backup_Data_Mapping.tex.tex <==
% \section{Data Mapping and Scalability}

% The way OMS data is mapped directly impacts scalability and efficiency. Here we analyze how different accelerators handle reference database layout, parallelism, and long-term scalability.

% \subsection{Conventional Accelerators}
% On GPUs, references must fit within limited HBM capacity (≤80~GB). Multi-terabyte OMS libraries require partitioning across multiple GPUs or streaming from host memory, introducing heavy interconnect overhead. FPGAs colocated with SSDs reduce host traffic, but logic and BRAM/URAM resources limit the size of cached reference blocks and query width.

% \subsection{Memory-Centric Accelerators}
% In DRAM IMP, references are spread across banks and subarrays. Query broadcast exploits high internal bandwidth, but filtering by $m/z$ or charge can cause bank underutilization. ReRAM and PCM exploit multi-level cells to pack 2–3× more references per array, offering higher density. However, endurance limits (ReRAM) and resistance drift (PCM) constrain scalability, and ADC overhead grows with array size. These technologies scale in capacity but face challenges in long-term stability.

% \subsection{Storage-Centric Accelerators}
% 3D NAND achieves terabyte-per-package density through vertical stacking, but similarity search is limited by sequential multi-level sensing. Scaling to thousands of layers improves raw capacity but not query throughput. FeNAND addresses this by enabling multi-WL activation and DBAM filtering, which reduces the number of sequential reads per query. With stacking beyond 1000 layers and low-voltage ferroelectric cells, FeNAND offers unmatched scalability while alleviating NAND’s inherent sequential bottleneck.


% Overall, GPUs and FPGAs provide limited scalability due to device memory and resource constraints. DRAM IMP offers moderate scalability but is bounded by package capacity and bank balance. ReRAM and PCM scale through MLC density but face device reliability concerns. 3D NAND and FeNAND scale to storage-class datasets, with FeNAND offering improved latency and efficiency through DBAM. These mapping and scalability differences define the trade-offs evaluated in Section~6.





\section{Data Mapping and Scalability}

% \subsection{GPUs (NVIDIA RTX 4090, H100)}

% GPU scalability is governed by how the reference library is partitioned and staged into device memory. If the library size $S$ is less than or equal to $C_{\mathrm{HBM}}$ (or $C_{\mathrm{GDDR}}$ on RTX~4090), references remain resident in device memory and query batches reuse them directly. If $S$ is greater than $C_{\mathrm{HBM}}$, the dataset is divided into shards that fit in device memory. If using a single GPU, each batch of queries is processed against one shard at a time, per-shard top-$k$ is produced, and results are merged across shards. In multi-GPU settings, full library shards can be distributed across devices for query-level parallelism, and final results are merged by the host.

% At terabyte scale, scalability is determined by two factors: (1) the ratio $S/C_{\mathrm{HBM}}$, which dictates how much sharding and movement is required, and (2) the efficiency of data movement and overlap across the storage to device fabric. Report both warm runs, search-only with data already in device memory, and cold runs, including the one-time library load, to capture the true end-to-end trade-off.

% \subsection{FPGAs (SmartSSD-class, VP1902-class)}

% FPGA scalability is governed by how the reference library is partitioned on SSD and staged into device DRAM. References are stored as block-aligned partitions with the metadata needed for open-search filtering. The orchestrator prefetches the next block into device DRAM, refills on-chip buffers, and launches the bitwise kernel on the active block. Per-query top-$k$ is produced on device and only indices and scores are written back. Overlap of SSD reads, device-DRAM refill, and kernel execution is essential. Strengths are reduced host traffic and good energy per query. Limits are on-chip memory sizes and device DRAM capacity, which bound the reusable hotset and partial-score buffers.

% At terabyte scale, scalability is determined by two factors: (1) the ratio of library size to effective on-device memory for caching, which dictates block reuse and prefetch depth, and (2) the efficiency of the overlap among SSD reads, device-DRAM buffering, and fabric compute.



% \subsection{DRAM-Centric Accelerator (HyperOMS PIM, search only)}

% References are interleaved by precursor charge and $m/z$ range so every bank holds candidates for every query, ensuring that all banks are active and avoiding skew. The dispatcher consults the mapping table to derive row ranges for the query and broadcasts identical commands to all banks. Each bank searches independently, then reports its local best (row, offset, similarity). The dispatcher reconstructs the global reference ID from the bank and row indices, and selects the overall top match or builds a top-$k$ set.

% Scaling is primarily driven by the number of banks. Doubling banks from 64 to 128 increases throughput by about $1.9\times$, nearly linear but not perfect since only the in-bank search benefits directly. The interleaved layout plus broadcast dispatch avoids underutilization, giving more than $3\times$ improvement compared to a naive scheme that groups references by charge per bank. Because search occurs inside the memory, only the small query vector and compact results cross the external bus. This unlocks far higher effective bandwidth than host-side scanning. Combined with early exit via folding, the DRAM PIM design significantly improves throughput and energy efficiency at repository scale while preserving identification accuracy.





% \subsection{Storage-Centric Accelerators (3D NAND and FeNAND)}

% Hypervector bits are placed so that the page width matches the dimension $D$, allowing each page read to correspond to one vector slice without extra partial-sum passes. References are organized into tiles aligned with page, plane, and die geometry; queries are broadcast to the active tiles; local reduction yields per-tile top-$k$; only indices and scores traverse the device interface. For each query, the controller schedules a sequence of page activations, senses and digitizes per-page overlaps, and accumulates across the required layers to form complete scores. Because computation occurs in place, host traffic is minimal and largely independent of library size. Effective scale depends on tile count per package, page scheduling across planes and dies, and the efficiency of local accumulation; FeNAND follows the same scheduling and mapping model while operating at different device conditions.

